Cellular automata on a $G$-set

We extend the usual definition of cellular automaton on a group in order to deal with a new kind of cellular automata, like cellular automata in the hyperbolic plane and we explore some properties of these cellular automata. This definition also allows to deal with maps, intuitively considered as cellular automata, even if they did not match the usual definition, like the Margolus billiard-ball. One of the main results is an extension of Hedlund's theorem for these cellular automata.

==> fig1-0dr.tex <==
\psarccircP 3 ; 1.189207 [1,2]
\psarccircP 13 ; 1.189207 [11,12]
\psarccircP 23 ; 1.189207 [21,22]
\psarccircP 33 ; 1.189207 [31,32]
\psarccircP 43 ; 1.189207 [41,42]
\psarccircP 53 ; 1.189207 [51,52]
\psarccircP 63 ; 1.189207 [61,62]
\psarccircP 73 ; 1.189207 [71,72]
\psarccircP 83 ; 1.189207 [81,82]
\psline[91,92]
\psarccircP 103 ; 0.492586 [101,102]
\psarccircP 113 ; 0.246293 [111,112]
\psarccircP 123 ; 0.204036 [121,122]
\psarccircP 133 ; 0.246293 [131,132]
\psarccircP 143 ; 0.492586 [141,142]
\psline[151,152]
\psarccircP 163 ; 1.189207 [161,162]
\psline[171,172]
\psarccircP 183 ; 0.492586 [181,182]
\psarccircP 193 ; 0.246293 [191,192]
\psarccircP 203 ; 0.204036 [201,202]
\psarccircP 213 ; 0.246293 [211,212]
\psarccircP 223 ; 0.492586 [221,222]
\psline[231,232]
\psarccircP 243 ; 1.189207 [241,242]
\psline[251,252]
\psarccircP 263 ; 0.492586 [261,262]
\psarccircP 273 ; 0.246293 [271,272]
\psarccircP 283 ; 0.204036 [281,282]
\psarccircP 293 ; 0.246293 [291,292]
\psarccircP 303 ; 0.492586 [301,302]
\psline[311,312]
\psarccircP 323 ; 1.189207 [321,322]
\psline[331,332]
\psarccircP 343 ; 0.492586 [341,342]
\psarccircP 353 ; 0.246293 [351,352]
\psarccircP 363 ; 0.204036 [361,362]
\psarccircP 373 ; 0.246293 [371,372]
\psarccircP 383 ; 0.492586 [381,382]
\psline[391,392]
\psarccircP 403 ; 1.189207 [401,402]
\psline[411,412]
\psarccircP 423 ; 0.492586 [421,422]
\psarccircP 433 ; 0.246293 [431,432]
\psarccircP 443 ; 0.204036 [441,442]
\psarccircP 453 ; 0.246293 [451,452]
\psarccircP 463 ; 0.492586 [461,462]
\psline[471,472]
\psarccircP 483 ; 1.189207 [481,482]
\psline[491,492]
\psarccircP 503 ; 0.492586 [501,502]
\psarccircP 513 ; 0.246293 [511,512]
\psarccircP 523 ; 0.204036 [521,522]
\psarccircP 533 ; 0.246293 [531,532]
\psarccircP 543 ; 0.492586 [541,542]
\psline[551,552]
\psarccircP 563 ; 1.189207 [561,562]
\psline[571,572]
\psarccircP 583 ; 0.492586 [581,582]
\psarccircP 593 ; 0.246293 [591,592]
\psarccircP 603 ; 0.204036 [601,602]
\psarccircP 613 ; 0.246293 [611,612]
\psarccircP 623 ; 0.492586 [621,622]
\psline[631,632]
\psarccircP 643 ; 1.189207 [641,642]
\psline[651,652]
\psarccircP 663 ; 0.492586 [661,662]
\psarccircP 673 ; 0.246293 [671,672]
\psarccircP 683 ; 0.204036 [681,682]
\psarccircP 693 ; 0.246293 [691,692]
\psarccircP 703 ; 0.492586 [701,702]
\psline[711,712]
\psarccircP 723 ; 0.492586 [721,722]
\psarccircP 733 ; 0.492586 [731,732]
\psarccircP 743 ; 0.492586 [741,742]
\psarccircP 753 ; 0.128665 [751,752]
\psarccircP 763 ; 0.084514 [761,762]
\psarccircP 773 ; 0.084514 [771,772]
\psarccircP 783 ; 0.128665 [781,782]
\psarccircP 793 ; 0.492586 [791,792]
\psarccircP 803 ; 0.246293 [801,802]
\psarccircP 813 ; 0.492586 [811,812]
\psarccircP 823 ; 0.174155 [821,822]
\psarccircP 833 ; 0.068012 [831,832]
\psarccircP 843 ; 0.051009 [841,842]
\psarccircP 853 ; 0.056901 [851,852]
\psarccircP 863 ; 0.102018 [861,862]
\psarccircP 873 ; 1.189207 [871,872]
\psarccircP 883 ; 0.204036 [881,882]
\psarccircP 893 ; 1.189207 [891,892]
\psarccircP 903 ; 0.111591 [901,902]
\psarccircP 913 ; 0.053295 [911,912]
\psarccircP 923 ; 0.043814 [921,922]
\psarccircP 933 ; 0.053295 [931,932]
\psarccircP 943 ; 0.111591 [941,942]
\psarccircP 953 ; 1.189207 [951,952]
\psarccircP 963 ; 0.246293 [961,962]
\psarccircP 973 ; 1.189207 [971,972]
\psarccircP 983 ; 0.102018 [981,982]
\psarccircP 993 ; 0.056901 [991,992]
\psarccircP 1003 ; 0.051009 [1001,1002]
\psarccircP 1013 ; 0.068012 [1011,1012]
\psarccircP 1023 ; 0.174155 [1021,1022]
\psarccircP 1033 ; 0.492586 [1031,1032]
\psarccircP 1043 ; 0.492586 [1041,1042]
\psarccircP 1053 ; 0.492586 [1051,1052]
\psarccircP 1063 ; 0.492586 [1061,1062]
\psarccircP 1073 ; 0.128665 [1071,1072]
\psarccircP 1083 ; 0.084514 [1081,1082]
\psarccircP 1093 ; 0.084514 [1091,1092]
\psarccircP 1103 ; 0.128665 [1101,1102]
\psarccircP 1113 ; 0.492586 [1111,1112]
\psarccircP 1123 ; 0.246293 [1121,1122]
\psarccircP 1133 ; 0.492586 [1131,1132]
\psarccircP 1143 ; 0.174155 [1141,1142]
\psarccircP 1153 ; 0.068012 [1151,1152]
\psarccircP 1163 ; 0.051009 [1161,1162]
\psarccircP 1173 ; 0.056901 [1171,1172]
\psarccircP 1183 ; 0.102018 [1181,1182]
\psarccircP 1193 ; 1.189207 [1191,1192]
\psarccircP 1203 ; 0.204036 [1201,1202]
\psarccircP 1213 ; 1.189207 [1211,1212]
\psarccircP 1223 ; 0.111591 [1221,1222]
\psarccircP 1233 ; 0.053295 [1231,1232]
\psarccircP 1243 ; 0.043814 [1241,1242]
\psarccircP 1253 ; 0.053295 [1251,1252]
\psarccircP 1263 ; 0.111591 [1261,1262]
\psarccircP 1273 ; 1.189207 [1271,1272]
\psarccircP 1283 ; 0.246293 [1281,1282]
\psarccircP 1293 ; 1.189207 [1291,1292]
\psarccircP 1303 ; 0.102018 [1301,1302]
\psarccircP 1313 ; 0.056901 [1311,1312]
\psarccircP 1323 ; 0.051009 [1321,1322]
\psarccircP 1333 ; 0.068012 [1331,1332]
\psarccircP 1343 ; 0.174155 [1341,1342]
\psarccircP 1353 ; 0.492586 [1351,1352]
\psarccircP 1363 ; 0.492586 [1361,1362]
\psarccircP 1373 ; 0.492586 [1371,1372]
\psarccircP 1383 ; 0.492586 [1381,1382]
\psarccircP 1393 ; 0.128665 [1391,1392]
\psarccircP 1403 ; 0.084514 [1401,1402]
\psarccircP 1413 ; 0.084514 [1411,1412]
\psarccircP 1423 ; 0.128665 [1421,1422]
\psarccircP 1433 ; 0.492586 [1431,1432]
\psarccircP 1443 ; 0.246293 [1441,1442]
\psarccircP 1453 ; 0.492586 [1451,1452]
\psarccircP 1463 ; 0.174155 [1461,1462]
\psarccircP 1473 ; 0.068012 [1471,1472]
\psarccircP 1483 ; 0.051009 [1481,1482]
\psarccircP 1493 ; 0.056901 [1491,1492]
\psarccircP 1503 ; 0.102018 [1501,1502]
\psarccircP 1513 ; 1.189207 [1511,1512]
\psarccircP 1523 ; 0.204036 [1521,1522]
\psarccircP 1533 ; 1.189207 [1531,1532]
\psarccircP 1543 ; 0.111591 [1541,1542]
\psarccircP 1553 ; 0.053295 [1551,1552]
\psarccircP 1563 ; 0.043814 [1561,1562]
\psarccircP 1573 ; 0.053295 [1571,1572]
\psarccircP 1583 ; 0.111591 [1581,1582]
\psarccircP 1593 ; 1.189207 [1591,1592]
\psarccircP 1603 ; 0.246293 [1601,1602]
\psarccircP 1613 ; 1.189207 [1611,1612]
\psarccircP 1623 ; 0.102018 [1621,1622]
\psarccircP 1633 ; 0.056901 [1631,1632]
\psarccircP 1643 ; 0.051009 [1641,1642]
\psarccircP 1653 ; 0.068012 [1651,1652]
\psarccircP 1663 ; 0.174155 [1661,1662]
\psarccircP 1673 ; 0.492586 [1671,1672]
\psarccircP 1683 ; 0.492586 [1681,1682]
\psarccircP 1693 ; 0.492586 [1691,1692]
\psarccircP 1703 ; 0.492586 [1701,1702]
\psarccircP 1713 ; 0.128665 [1711,1712]
\psarccircP 1723 ; 0.084514 [1721,1722]
\psarccircP 1733 ; 0.084514 [1731,1732]
\psarccircP 1743 ; 0.128665 [1741,1742]
\psarccircP 1753 ; 0.492586 [1751,1752]
\psarccircP 1763 ; 0.246293 [1761,1762]
\psarccircP 1773 ; 0.492586 [1771,1772]
\psarccircP 1783 ; 0.174155 [1781,1782]
\psarccircP 1793 ; 0.068012 [1791,1792]
\psarccircP 1803 ; 0.051009 [1801,1802]
\psarccircP 1813 ; 0.056901 [1811,1812]
\psarccircP 1823 ; 0.102018 [1821,1822]
\psarccircP 1833 ; 1.189207 [1831,1832]
\psarccircP 1843 ; 0.204036 [1841,1842]
\psarccircP 1853 ; 1.189207 [1851,1852]
\psarccircP 1863 ; 0.111591 [1861,1862]
\psarccircP 1873 ; 0.053295 [1871,1872]
\psarccircP 1883 ; 0.043814 [1881,1882]
\psarccircP 1893 ; 0.053295 [1891,1892]
\psarccircP 1903 ; 0.111591 [1901,1902]
\psarccircP 1913 ; 1.189207 [1911,1912]
\psarccircP 1923 ; 0.246293 [1921,1922]
\psarccircP 1933 ; 1.189207 [1931,1932]
\psarccircP 1943 ; 0.102018 [1941,1942]
\psarccircP 1953 ; 0.056901 [1951,1952]
\psarccircP 1963 ; 0.051009 [1961,1962]
\psarccircP 1973 ; 0.068012 [1971,1972]
\psarccircP 1983 ; 0.174155 [1981,1982]
\psarccircP 1993 ; 0.492586 [1991,1992]
\psarccircP 2003 ; 0.492586 [2001,2002]
\psarccircP 2013 ; 0.492586 [2011,2012]
\psarccircP 2023 ; 0.492586 [2021,2022]
\psarccircP 2033 ; 0.128665 [2031,2032]
\psarccircP 2043 ; 0.084514 [2041,2042]
\psarccircP 2053 ; 0.084514 [2051,2052]
\psarccircP 2063 ; 0.128665 [2061,2062]
\psarccircP 2073 ; 0.492586 [2071,2072]
\psarccircP 2083 ; 0.246293 [2081,2082]
\psarccircP 2093 ; 0.492586 [2091,2092]
\psarccircP 2103 ; 0.174155 [2101,2102]
\psarccircP 2113 ; 0.068012 [2111,2112]
\psarccircP 2123 ; 0.051009 [2121,2122]
\psarccircP 2133 ; 0.056901 [2131,2132]
\psarccircP 2143 ; 0.102018 [2141,2142]
\psarccircP 2153 ; 1.189207 [2151,2152]
\psarccircP 2163 ; 0.204036 [2161,2162]
\psarccircP 2173 ; 1.189207 [2171,2172]
\psarccircP 2183 ; 0.111591 [2181,2182]
\psarccircP 2193 ; 0.053295 [2191,2192]
\psarccircP 2203 ; 0.043814 [2201,2202]
\psarccircP 2213 ; 0.053295 [2211,2212]
\psarccircP 2223 ; 0.111591 [2221,2222]
\psarccircP 2233 ; 1.189207 [2231,2232]
\psarccircP 2243 ; 0.246293 [2241,2242]
\psarccircP 2253 ; 1.189207 [2251,2252]
\psarccircP 2263 ; 0.102018 [2261,2262]
\psarccircP 2273 ; 0.056901 [2271,2272]
\psarccircP 2283 ; 0.051009 [2281,2282]
\psarccircP 2293 ; 0.068012 [2291,2292]
\psarccircP 2303 ; 0.174155 [2301,2302]
\psarccircP 2313 ; 0.492586 [2311,2312]
\psarccircP 2323 ; 0.492586 [2321,2322]
\psarccircP 2333 ; 0.492586 [2331,2332]
\psarccircP 2343 ; 0.492586 [2341,2342]
\psarccircP 2353 ; 0.128665 [2351,2352]
\psarccircP 2363 ; 0.084514 [2361,2362]
\psarccircP 2373 ; 0.084514 [2371,2372]
\psarccircP 2383 ; 0.128665 [2381,2382]
\psarccircP 2393 ; 0.492586 [2391,2392]
\psarccircP 2403 ; 0.246293 [2401,2402]
\psarccircP 2413 ; 0.492586 [2411,2412]
\psarccircP 2423 ; 0.174155 [2421,2422]
\psarccircP 2433 ; 0.068012 [2431,2432]
\psarccircP 2443 ; 0.051009 [2441,2442]
\psarccircP 2453 ; 0.056901 [2451,2452]
\psarccircP 2463 ; 0.102018 [2461,2462]
\psarccircP 2473 ; 1.189207 [2471,2472]
\psarccircP 2483 ; 0.204036 [2481,2482]
\psarccircP 2493 ; 1.189207 [2491,2492]
\psarccircP 2503 ; 0.111591 [2501,2502]
\psarccircP 2513 ; 0.053295 [2511,2512]
\psarccircP 2523 ; 0.043814 [2521,2522]
\psarccircP 2533 ; 0.053295 [2531,2532]
\psarccircP 2543 ; 0.111591 [2541,2542]
\psarccircP 2553 ; 1.189207 [2551,2552]
\psarccircP 2563 ; 0.246293 [2561,2562]
\psarccircP 2573 ; 1.189207 [2571,2572]
\psarccircP 2583 ; 0.102018 [2581,2582]
\psarccircP 2593 ; 0.056901 [2591,2592]
\psarccircP 2603 ; 0.051009 [2601,2602]
\psarccircP 2613 ; 0.068012 [2611,2612]
\psarccircP 2623 ; 0.174155 [2621,2622]
\psarccircP 2633 ; 0.492586 [2631,2632]
\psarccircP 2643 ; 0.492586 [2641,2642]
\psarccircP 2653 ; 0.492586 [2651,2652]
\psarccircP 2663 ; 0.492586 [2661,2662]
\psarccircP 2673 ; 0.128665 [2671,2672]
\psarccircP 2683 ; 0.084514 [2681,2682]
\psarccircP 2693 ; 0.084514 [2691,2692]
\psarccircP 2703 ; 0.128665 [2701,2702]
\psarccircP 2713 ; 0.492586 [2711,2712]
\psarccircP 2723 ; 0.246293 [2721,2722]
\psarccircP 2733 ; 0.492586 [2731,2732]
\psarccircP 2743 ; 0.174155 [2741,2742]
\psarccircP 2753 ; 0.068012 [2751,2752]
\psarccircP 2763 ; 0.051009 [2761,2762]
\psarccircP 2773 ; 0.056901 [2771,2772]
\psarccircP 2783 ; 0.102018 [2781,2782]
\psarccircP 2793 ; 1.189207 [2791,2792]
\psarccircP 2803 ; 0.204036 [2801,2802]
\psarccircP 2813 ; 1.189207 [2811,2812]
\psarccircP 2823 ; 0.111591 [2821,2822]
\psarccircP 2833 ; 0.053295 [2831,2832]
\psarccircP 2843 ; 0.043814 [2841,2842]
\psarccircP 2853 ; 0.053295 [2851,2852]
\psarccircP 2863 ; 0.111591 [2861,2862]
\psarccircP 2873 ; 1.189207 [2871,2872]
\psarccircP 2883 ; 0.246293 [2881,2882]
\psarccircP 2893 ; 1.189207 [2891,2892]
\psarccircP 2903 ; 0.102018 [2901,2902]
\psarccircP 2913 ; 0.056901 [2911,2912]
\psarccircP 2923 ; 0.051009 [2921,2922]
\psarccircP 2933 ; 0.068012 [2931,2932]
\psarccircP 2943 ; 0.174155 [2941,2942]
\psarccircP 2953 ; 0.492586 [2951,2952]
\psarccircP 2963 ; 0.492586 [2961,2962]
\psarccircP 2973 ; 0.492586 [2971,2972]
\psarccircP 2983 ; 0.492586 [2981,2982]
\psarccircP 2993 ; 0.128665 [2991,2992]
\psarccircP 3003 ; 0.084514 [3001,3002]
\psarccircP 3013 ; 0.084514 [3011,3012]
\psarccircP 3023 ; 0.128665 [3021,3022]
\psarccircP 3033 ; 0.492586 [3031,3032]
\psarccircP 3043 ; 0.246293 [3041,3042]
\psarccircP 3053 ; 0.492586 [3051,3052]
\psarccircP 3063 ; 0.174155 [3061,3062]
\psarccircP 3073 ; 0.068012 [3071,3072]
\psarccircP 3083 ; 0.051009 [3081,3082]
\psarccircP 3093 ; 0.056901 [3091,3092]
\psarccircP 3103 ; 0.102018 [3101,3102]
\psarccircP 3113 ; 1.189207 [3111,3112]
\psarccircP 3123 ; 0.204036 [3121,3122]
\psarccircP 3133 ; 1.189207 [3131,3132]
\psarccircP 3143 ; 0.111591 [3141,3142]
\psarccircP 3153 ; 0.053295 [3151,3152]
\psarccircP 3163 ; 0.043814 [3161,3162]
\psarccircP 3173 ; 0.053295 [3171,3172]
\psarccircP 3183 ; 0.111591 [3181,3182]
\psarccircP 3193 ; 1.189207 [3191,3192]
\psarccircP 3203 ; 0.246293 [3201,3202]
\psarccircP 3213 ; 1.189207 [3211,3212]
\psarccircP 3223 ; 0.102018 [3221,3222]
\psarccircP 3233 ; 0.056901 [3231,3232]
\psarccircP 3243 ; 0.051009 [3241,3242]
\psarccircP 3253 ; 0.068012 [3251,3252]
\psarccircP 3263 ; 0.174155 [3261,3262]
\psarccircP 3273 ; 0.492586 [3271,3272]
\psarccircP 3283 ; 0.128665 [3281,3282]
\psarccircP 3293 ; 0.174155 [3291,3292]
\psarccircP 3303 ; 0.111591 [3301,3302]
\psarccircP 3313 ; 0.036069 [3311,3312]
\psarccircP 3323 ; 0.025280 [3321,3322]
\psarccircP 3333 ; 0.026647 [3331,3332]
\psarccircP 3343 ; 0.043814 [3341,3342]
\psarccircP 3353 ; 0.246293 [3351,3352]
\psarccircP 3363 ; 0.084514 [3361,3362]
\psarccircP 3373 ; 0.246293 [3371,3372]
\psarccircP 3383 ; 0.053295 [3381,3382]
\psarccircP 3393 ; 0.023111 [3391,3392]
\psarccircP 3403 ; 0.018148 [3401,3402]
\psarccircP 3413 ; 0.021129 [3411,3412]
\psarccircP 3423 ; 0.040807 [3421,3422]
\psline[3431,3432]
\psarccircP 3443 ; 0.084514 [3441,3442]
\psline[3451,3452]
\psarccircP 3463 ; 0.040807 [3461,3462]
\psarccircP 3473 ; 0.021129 [3471,3472]
\psarccircP 3483 ; 0.018148 [3481,3482]
\psarccircP 3493 ; 0.023111 [3491,3492]
\psarccircP 3503 ; 0.053295 [3501,3502]
\psarccircP 3513 ; 0.246293 [3511,3512]
\psarccircP 3523 ; 0.174155 [3521,3522]
\psarccircP 3533 ; 0.128665 [3531,3532]
\psarccircP 3543 ; 0.246293 [3541,3542]
\psarccircP 3553 ; 0.043814 [3551,3552]
\psarccircP 3563 ; 0.026647 [3561,3562]
\psarccircP 3573 ; 0.025280 [3571,3572]
\psarccircP 3583 ; 0.036069 [3581,3582]
\psarccircP 3593 ; 0.111591 [3591,3592]
\psarccircP 3603 ; 0.068012 [3601,3602]
\psarccircP 3613 ; 0.111591 [3611,3612]
\psarccircP 3623 ; 0.053295 [3621,3622]
\psarccircP 3633 ; 0.019146 [3631,3632]
\psarccircP 3643 ; 0.013921 [3641,3642]
\psarccircP 3653 ; 0.015130 [3651,3652]
\psarccircP 3663 ; 0.026063 [3661,3662]
\psarccircP 3673 ; 0.204036 [3671,3672]
\psarccircP 3683 ; 0.051009 [3681,3682]
\psarccircP 3693 ; 0.204036 [3691,3692]
\psarccircP 3703 ; 0.029880 [3701,3702]
\psarccircP 3713 ; 0.013694 [3711,3712]
\psarccircP 3723 ; 0.011038 [3721,3722]
\psarccircP 3733 ; 0.013176 [3731,3732]
\psarccircP 3743 ; 0.026647 [3741,3742]
\psarccircP 3753 ; 0.492586 [3751,3752]
\psarccircP 3763 ; 0.056901 [3761,3762]
\psarccircP 3773 ; 0.492586 [3771,3772]
\psarccircP 3783 ; 0.025280 [3781,3782]
\psarccircP 3793 ; 0.013694 [3791,3792]
\psarccircP 3803 ; 0.012073 [3801,3802]
\psarccircP 3813 ; 0.015817 [3811,3812]
\psarccircP 3823 ; 0.038918 [3821,3822]
\psarccircP 3833 ; 0.128665 [3831,3832]
\psarccircP 3843 ; 0.111591 [3841,3842]
\psarccircP 3853 ; 0.102018 [3851,3852]
\psarccircP 3863 ; 0.128665 [3861,3862]
\psarccircP 3873 ; 0.029880 [3871,3872]
\psarccircP 3883 ; 0.019146 [3881,3882]
\psarccircP 3893 ; 0.018843 [3891,3892]
\psarccircP 3903 ; 0.028171 [3901,3902]
\psarccircP 3913 ; 0.102018 [3911,3912]
\psarccircP 3923 ; 0.053295 [3921,3922]
\psarccircP 3933 ; 0.102018 [3931,3932]
\psarccircP 3943 ; 0.038918 [3941,3942]
\psarccircP 3953 ; 0.014940 [3951,3952]
\psarccircP 3963 ; 0.011141 [3961,3962]
\psarccircP 3973 ; 0.012377 [3971,3972]
\psarccircP 3983 ; 0.022075 [3981,3982]
\psarccircP 3993 ; 0.246293 [3991,3992]
\psarccircP 4003 ; 0.043814 [4001,4002]
\psarccircP 4013 ; 0.246293 [4011,4012]
\psarccircP 4023 ; 0.024249 [4021,4022]
\psarccircP 4033 ; 0.011556 [4031,4032]
\psarccircP 4043 ; 0.009497 [4041,4042]
\psarccircP 4053 ; 0.011556 [4051,4052]
\psarccircP 4063 ; 0.024249 [4061,4062]
\psarccircP 4073 ; 0.246293 [4071,4072]
\psarccircP 4083 ; 0.053295 [4081,4082]
\psarccircP 4093 ; 0.246293 [4091,4092]
\psarccircP 4103 ; 0.022075 [4101,4102]
\psarccircP 4113 ; 0.012377 [4111,4112]
\psarccircP 4123 ; 0.011141 [4121,4122]
\psarccircP 4133 ; 0.014940 [4131,4132]
\psarccircP 4143 ; 0.038918 [4141,4142]
\psarccircP 4153 ; 0.102018 [4151,4152]
\psarccircP 4163 ; 0.102018 [4161,4162]
\psarccircP 4173 ; 0.111591 [4171,4172]
\psarccircP 4183 ; 0.102018 [4181,4182]
\psarccircP 4193 ; 0.028171 [4191,4192]
\psarccircP 4203 ; 0.018843 [4201,4202]
\psarccircP 4213 ; 0.019146 [4211,4212]
\psarccircP 4223 ; 0.029880 [4221,4222]
\psarccircP 4233 ; 0.128665 [4231,4232]
\psarccircP 4243 ; 0.056901 [4241,4242]
\psarccircP 4253 ; 0.128665 [4251,4252]
\psarccircP 4263 ; 0.038918 [4261,4262]
\psarccircP 4273 ; 0.015817 [4271,4272]
\psarccircP 4283 ; 0.012073 [4281,4282]
\psarccircP 4293 ; 0.013694 [4291,4292]
\psarccircP 4303 ; 0.025280 [4301,4302]
\psarccircP 4313 ; 0.492586 [4311,4312]
\psarccircP 4323 ; 0.051009 [4321,4322]
\psarccircP 4333 ; 0.492586 [4331,4332]
\psarccircP 4343 ; 0.026647 [4341,4342]
\psarccircP 4353 ; 0.013176 [4351,4352]
\psarccircP 4363 ; 0.011038 [4361,4362]
\psarccircP 4373 ; 0.013694 [4371,4372]
\psarccircP 4383 ; 0.029880 [4381,4382]
\psarccircP 4393 ; 0.204036 [4391,4392]
\psarccircP 4403 ; 0.068012 [4401,4402]
\psarccircP 4413 ; 0.204036 [4411,4412]
\psarccircP 4423 ; 0.026063 [4421,4422]
\psarccircP 4433 ; 0.015130 [4431,4432]
\psarccircP 4443 ; 0.013921 [4441,4442]
\psarccircP 4453 ; 0.019146 [4451,4452]
\psarccircP 4463 ; 0.053295 [4461,4462]
\psarccircP 4473 ; 0.111591 [4471,4472]
\psarccircP 4483 ; 0.128665 [4481,4482]
\psarccircP 4493 ; 0.174155 [4491,4492]
\psarccircP 4503 ; 0.111591 [4501,4502]
\psarccircP 4513 ; 0.036069 [4511,4512]
\psarccircP 4523 ; 0.025280 [4521,4522]
\psarccircP 4533 ; 0.026647 [4531,4532]
\psarccircP 4543 ; 0.043814 [4541,4542]
\psarccircP 4553 ; 0.246293 [4551,4552]
\psarccircP 4563 ; 0.084514 [4561,4562]
\psarccircP 4573 ; 0.246293 [4571,4572]
\psarccircP 4583 ; 0.053295 [4581,4582]
\psarccircP 4593 ; 0.023111 [4591,4592]
\psarccircP 4603 ; 0.018148 [4601,4602]
\psarccircP 4613 ; 0.021129 [4611,4612]
\psarccircP 4623 ; 0.040807 [4621,4622]
\psline[4631,4632]
\psarccircP 4643 ; 0.084514 [4641,4642]
\psline[4651,4652]
\psarccircP 4663 ; 0.040807 [4661,4662]
\psarccircP 4673 ; 0.021129 [4671,4672]
\psarccircP 4683 ; 0.018148 [4681,4682]
\psarccircP 4693 ; 0.023111 [4691,4692]
\psarccircP 4703 ; 0.053295 [4701,4702]
\psarccircP 4713 ; 0.246293 [4711,4712]
\psarccircP 4723 ; 0.174155 [4721,4722]
\psarccircP 4733 ; 0.128665 [4731,4732]
\psarccircP 4743 ; 0.246293 [4741,4742]
\psarccircP 4753 ; 0.043814 [4751,4752]
\psarccircP 4763 ; 0.026647 [4761,4762]
\psarccircP 4773 ; 0.025280 [4771,4772]
\psarccircP 4783 ; 0.036069 [4781,4782]
\psarccircP 4793 ; 0.111591 [4791,4792]
\psarccircP 4803 ; 0.068012 [4801,4802]
\psarccircP 4813 ; 0.111591 [4811,4812]
\psarccircP 4823 ; 0.053295 [4821,4822]
\psarccircP 4833 ; 0.019146 [4831,4832]
\psarccircP 4843 ; 0.013921 [4841,4842]
\psarccircP 4853 ; 0.015130 [4851,4852]
\psarccircP 4863 ; 0.026063 [4861,4862]
\psarccircP 4873 ; 0.204036 [4871,4872]
\psarccircP 4883 ; 0.051009 [4881,4882]
\psarccircP 4893 ; 0.204036 [4891,4892]
\psarccircP 4903 ; 0.029880 [4901,4902]
\psarccircP 4913 ; 0.013694 [4911,4912]
\psarccircP 4923 ; 0.011038 [4921,4922]
\psarccircP 4933 ; 0.013176 [4931,4932]
\psarccircP 4943 ; 0.026647 [4941,4942]
\psarccircP 4953 ; 0.492586 [4951,4952]
\psarccircP 4963 ; 0.056901 [4961,4962]
\psarccircP 4973 ; 0.492586 [4971,4972]
\psarccircP 4983 ; 0.025280 [4981,4982]
\psarccircP 4993 ; 0.013694 [4991,4992]
\psarccircP 5003 ; 0.012073 [5001,5002]
\psarccircP 5013 ; 0.015817 [5011,5012]
\psarccircP 5023 ; 0.038918 [5021,5022]
\psarccircP 5033 ; 0.128665 [5031,5032]
\psarccircP 5043 ; 0.111591 [5041,5042]
\psarccircP 5053 ; 0.102018 [5051,5052]
\psarccircP 5063 ; 0.128665 [5061,5062]
\psarccircP 5073 ; 0.029880 [5071,5072]
\psarccircP 5083 ; 0.019146 [5081,5082]
\psarccircP 5093 ; 0.018843 [5091,5092]
\psarccircP 5103 ; 0.028171 [5101,5102]
\psarccircP 5113 ; 0.102018 [5111,5112]
\psarccircP 5123 ; 0.053295 [5121,5122]
\psarccircP 5133 ; 0.102018 [5131,5132]
\psarccircP 5143 ; 0.038918 [5141,5142]
\psarccircP 5153 ; 0.014940 [5151,5152]
\psarccircP 5163 ; 0.011141 [5161,5162]
\psarccircP 5173 ; 0.012377 [5171,5172]
\psarccircP 5183 ; 0.022075 [5181,5182]
\psarccircP 5193 ; 0.246293 [5191,5192]
\psarccircP 5203 ; 0.043814 [5201,5202]
\psarccircP 5213 ; 0.246293 [5211,5212]
\psarccircP 5223 ; 0.024249 [5221,5222]
\psarccircP 5233 ; 0.011556 [5231,5232]
\psarccircP 5243 ; 0.009497 [5241,5242]
\psarccircP 5253 ; 0.011556 [5251,5252]
\psarccircP 5263 ; 0.024249 [5261,5262]
\psarccircP 5273 ; 0.246293 [5271,5272]
\psarccircP 5283 ; 0.053295 [5281,5282]
\psarccircP 5293 ; 0.246293 [5291,5292]
\psarccircP 5303 ; 0.022075 [5301,5302]
\psarccircP 5313 ; 0.012377 [5311,5312]
\psarccircP 5323 ; 0.011141 [5321,5322]
\psarccircP 5333 ; 0.014940 [5331,5332]
\psarccircP 5343 ; 0.038918 [5341,5342]
\psarccircP 5353 ; 0.102018 [5351,5352]
\psarccircP 5363 ; 0.102018 [5361,5362]
\psarccircP 5373 ; 0.111591 [5371,5372]
\psarccircP 5383 ; 0.102018 [5381,5382]
\psarccircP 5393 ; 0.028171 [5391,5392]
\psarccircP 5403 ; 0.018843 [5401,5402]
\psarccircP 5413 ; 0.019146 [5411,5412]
\psarccircP 5423 ; 0.029880 [5421,5422]
\psarccircP 5433 ; 0.128665 [5431,5432]
\psarccircP 5443 ; 0.056901 [5441,5442]
\psarccircP 5453 ; 0.128665 [5451,5452]
\psarccircP 5463 ; 0.038918 [5461,5462]
\psarccircP 5473 ; 0.015817 [5471,5472]
\psarccircP 5483 ; 0.012073 [5481,5482]
\psarccircP 5493 ; 0.013694 [5491,5492]
\psarccircP 5503 ; 0.025280 [5501,5502]
\psarccircP 5513 ; 0.492586 [5511,5512]
\psarccircP 5523 ; 0.051009 [5521,5522]
\psarccircP 5533 ; 0.492586 [5531,5532]
\psarccircP 5543 ; 0.026647 [5541,5542]
\psarccircP 5553 ; 0.013176 [5551,5552]
\psarccircP 5563 ; 0.011038 [5561,5562]
\psarccircP 5573 ; 0.013694 [5571,5572]
\psarccircP 5583 ; 0.029880 [5581,5582]
\psarccircP 5593 ; 0.204036 [5591,5592]
\psarccircP 5603 ; 0.068012 [5601,5602]
\psarccircP 5613 ; 0.204036 [5611,5612]
\psarccircP 5623 ; 0.026063 [5621,5622]
\psarccircP 5633 ; 0.015130 [5631,5632]
\psarccircP 5643 ; 0.013921 [5641,5642]
\psarccircP 5653 ; 0.019146 [5651,5652]
\psarccircP 5663 ; 0.053295 [5661,5662]
\psarccircP 5673 ; 0.111591 [5671,5672]
\psarccircP 5683 ; 0.128665 [5681,5682]
\psarccircP 5693 ; 0.174155 [5691,5692]
\psarccircP 5703 ; 0.111591 [5701,5702]
\psarccircP 5713 ; 0.036069 [5711,5712]
\psarccircP 5723 ; 0.025280 [5721,5722]
\psarccircP 5733 ; 0.026647 [5731,5732]
\psarccircP 5743 ; 0.043814 [5741,5742]
\psarccircP 5753 ; 0.246293 [5751,5752]
\psarccircP 5763 ; 0.084514 [5761,5762]
\psarccircP 5773 ; 0.246293 [5771,5772]
\psarccircP 5783 ; 0.053295 [5781,5782]
\psarccircP 5793 ; 0.023111 [5791,5792]
\psarccircP 5803 ; 0.018148 [5801,5802]
\psarccircP 5813 ; 0.021129 [5811,5812]
\psarccircP 5823 ; 0.040807 [5821,5822]
\psline[5831,5832]
\psarccircP 5843 ; 0.084514 [5841,5842]
\psline[5851,5852]
\psarccircP 5863 ; 0.040807 [5861,5862]
\psarccircP 5873 ; 0.021129 [5871,5872]
\psarccircP 5883 ; 0.018148 [5881,5882]
\psarccircP 5893 ; 0.023111 [5891,5892]
\psarccircP 5903 ; 0.053295 [5901,5902]
\psarccircP 5913 ; 0.246293 [5911,5912]
\psarccircP 5923 ; 0.174155 [5921,5922]
\psarccircP 5933 ; 0.128665 [5931,5932]
\psarccircP 5943 ; 0.246293 [5941,5942]
\psarccircP 5953 ; 0.043814 [5951,5952]
\psarccircP 5963 ; 0.026647 [5961,5962]
\psarccircP 5973 ; 0.025280 [5971,5972]
\psarccircP 5983 ; 0.036069 [5981,5982]
\psarccircP 5993 ; 0.111591 [5991,5992]
\psarccircP 6003 ; 0.068012 [6001,6002]
\psarccircP 6013 ; 0.111591 [6011,6012]
\psarccircP 6023 ; 0.053295 [6021,6022]
\psarccircP 6033 ; 0.019146 [6031,6032]
\psarccircP 6043 ; 0.013921 [6041,6042]
\psarccircP 6053 ; 0.015130 [6051,6052]
\psarccircP 6063 ; 0.026063 [6061,6062]
\psarccircP 6073 ; 0.204036 [6071,6072]
\psarccircP 6083 ; 0.051009 [6081,6082]
\psarccircP 6093 ; 0.204036 [6091,6092]
\psarccircP 6103 ; 0.029880 [6101,6102]
\psarccircP 6113 ; 0.013694 [6111,6112]
\psarccircP 6123 ; 0.011038 [6121,6122]
\psarccircP 6133 ; 0.013176 [6131,6132]
\psarccircP 6143 ; 0.026647 [6141,6142]
\psarccircP 6153 ; 0.492586 [6151,6152]
\psarccircP 6163 ; 0.056901 [6161,6162]
\psarccircP 6173 ; 0.492586 [6171,6172]
\psarccircP 6183 ; 0.025280 [6181,6182]
\psarccircP 6193 ; 0.013694 [6191,6192]
\psarccircP 6203 ; 0.012073 [6201,6202]
\psarccircP 6213 ; 0.015817 [6211,6212]
\psarccircP 6223 ; 0.038918 [6221,6222]
\psarccircP 6233 ; 0.128665 [6231,6232]
\psarccircP 6243 ; 0.111591 [6241,6242]
\psarccircP 6253 ; 0.102018 [6251,6252]
\psarccircP 6263 ; 0.128665 [6261,6262]
\psarccircP 6273 ; 0.029880 [6271,6272]
\psarccircP 6283 ; 0.019146 [6281,6282]
\psarccircP 6293 ; 0.018843 [6291,6292]
\psarccircP 6303 ; 0.028171 [6301,6302]
\psarccircP 6313 ; 0.102018 [6311,6312]
\psarccircP 6323 ; 0.053295 [6321,6322]
\psarccircP 6333 ; 0.102018 [6331,6332]
\psarccircP 6343 ; 0.038918 [6341,6342]
\psarccircP 6353 ; 0.014940 [6351,6352]
\psarccircP 6363 ; 0.011141 [6361,6362]
\psarccircP 6373 ; 0.012377 [6371,6372]
\psarccircP 6383 ; 0.022075 [6381,6382]
\psarccircP 6393 ; 0.246293 [6391,6392]
\psarccircP 6403 ; 0.043814 [6401,6402]
\psarccircP 6413 ; 0.246293 [6411,6412]
\psarccircP 6423 ; 0.024249 [6421,6422]
\psarccircP 6433 ; 0.011556 [6431,6432]
\psarccircP 6443 ; 0.009497 [6441,6442]
\psarccircP 6453 ; 0.011556 [6451,6452]
\psarccircP 6463 ; 0.024249 [6461,6462]
\psarccircP 6473 ; 0.246293 [6471,6472]
\psarccircP 6483 ; 0.053295 [6481,6482]
\psarccircP 6493 ; 0.246293 [6491,6492]
\psarccircP 6503 ; 0.022075 [6501,6502]
\psarccircP 6513 ; 0.012377 [6511,6512]
\psarccircP 6523 ; 0.011141 [6521,6522]
\psarccircP 6533 ; 0.014940 [6531,6532]
\psarccircP 6543 ; 0.038918 [6541,6542]
\psarccircP 6553 ; 0.102018 [6551,6552]
\psarccircP 6563 ; 0.102018 [6561,6562]
\psarccircP 6573 ; 0.111591 [6571,6572]
\psarccircP 6583 ; 0.102018 [6581,6582]
\psarccircP 6593 ; 0.028171 [6591,6592]
\psarccircP 6603 ; 0.018843 [6601,6602]
\psarccircP 6613 ; 0.019146 [6611,6612]
\psarccircP 6623 ; 0.029880 [6621,6622]
\psarccircP 6633 ; 0.128665 [6631,6632]
\psarccircP 6643 ; 0.056901 [6641,6642]
\psarccircP 6653 ; 0.128665 [6651,6652]
\psarccircP 6663 ; 0.038918 [6661,6662]
\psarccircP 6673 ; 0.015817 [6671,6672]
\psarccircP 6683 ; 0.012073 [6681,6682]
\psarccircP 6693 ; 0.013694 [6691,6692]
\psarccircP 6703 ; 0.025280 [6701,6702]
\psarccircP 6713 ; 0.492586 [6711,6712]
\psarccircP 6723 ; 0.051009 [6721,6722]
\psarccircP 6733 ; 0.492586 [6731,6732]
\psarccircP 6743 ; 0.026647 [6741,6742]
\psarccircP 6753 ; 0.013176 [6751,6752]
\psarccircP 6763 ; 0.011038 [6761,6762]
\psarccircP 6773 ; 0.013694 [6771,6772]
\psarccircP 6783 ; 0.029880 [6781,6782]
\psarccircP 6793 ; 0.204036 [6791,6792]
\psarccircP 6803 ; 0.068012 [6801,6802]
\psarccircP 6813 ; 0.204036 [6811,6812]
\psarccircP 6823 ; 0.026063 [6821,6822]
\psarccircP 6833 ; 0.015130 [6831,6832]
\psarccircP 6843 ; 0.013921 [6841,6842]
\psarccircP 6853 ; 0.019146 [6851,6852]
\psarccircP 6863 ; 0.053295 [6861,6862]
\psarccircP 6873 ; 0.111591 [6871,6872]
\psarccircP 6883 ; 0.128665 [6881,6882]
\psarccircP 6893 ; 0.174155 [6891,6892]
\psarccircP 6903 ; 0.111591 [6901,6902]
\psarccircP 6913 ; 0.036069 [6911,6912]
\psarccircP 6923 ; 0.025280 [6921,6922]
\psarccircP 6933 ; 0.026647 [6931,6932]
\psarccircP 6943 ; 0.043814 [6941,6942]
\psarccircP 6953 ; 0.246293 [6951,6952]
\psarccircP 6963 ; 0.084514 [6961,6962]
\psarccircP 6973 ; 0.246293 [6971,6972]
\psarccircP 6983 ; 0.053295 [6981,6982]
\psarccircP 6993 ; 0.023111 [6991,6992]
\psarccircP 7003 ; 0.018148 [7001,7002]
\psarccircP 7013 ; 0.021129 [7011,7012]
\psarccircP 7023 ; 0.040807 [7021,7022]
\psline[7031,7032]
\psarccircP 7043 ; 0.084514 [7041,7042]
\psline[7051,7052]
\psarccircP 7063 ; 0.040807 [7061,7062]
\psarccircP 7073 ; 0.021129 [7071,7072]
\psarccircP 7083 ; 0.018148 [7081,7082]
\psarccircP 7093 ; 0.023111 [7091,7092]
\psarccircP 7103 ; 0.053295 [7101,7102]
\psarccircP 7113 ; 0.246293 [7111,7112]
\psarccircP 7123 ; 0.174155 [7121,7122]
\psarccircP 7133 ; 0.128665 [7131,7132]
\psarccircP 7143 ; 0.246293 [7141,7142]
\psarccircP 7153 ; 0.043814 [7151,7152]
\psarccircP 7163 ; 0.026647 [7161,7162]
\psarccircP 7173 ; 0.025280 [7171,7172]
\psarccircP 7183 ; 0.036069 [7181,7182]
\psarccircP 7193 ; 0.111591 [7191,7192]
\psarccircP 7203 ; 0.068012 [7201,7202]
\psarccircP 7213 ; 0.111591 [7211,7212]
\psarccircP 7223 ; 0.053295 [7221,7222]
\psarccircP 7233 ; 0.019146 [7231,7232]
\psarccircP 7243 ; 0.013921 [7241,7242]
\psarccircP 7253 ; 0.015130 [7251,7252]
\psarccircP 7263 ; 0.026063 [7261,7262]
\psarccircP 7273 ; 0.204036 [7271,7272]
\psarccircP 7283 ; 0.051009 [7281,7282]
\psarccircP 7293 ; 0.204036 [7291,7292]
\psarccircP 7303 ; 0.029880 [7301,7302]
\psarccircP 7313 ; 0.013694 [7311,7312]
\psarccircP 7323 ; 0.011038 [7321,7322]
\psarccircP 7333 ; 0.013176 [7331,7332]
\psarccircP 7343 ; 0.026647 [7341,7342]
\psarccircP 7353 ; 0.492586 [7351,7352]
\psarccircP 7363 ; 0.056901 [7361,7362]
\psarccircP 7373 ; 0.492586 [7371,7372]
\psarccircP 7383 ; 0.025280 [7381,7382]
\psarccircP 7393 ; 0.013694 [7391,7392]
\psarccircP 7403 ; 0.012073 [7401,7402]
\psarccircP 7413 ; 0.015817 [7411,7412]
\psarccircP 7423 ; 0.038918 [7421,7422]
\psarccircP 7433 ; 0.128665 [7431,7432]
\psarccircP 7443 ; 0.111591 [7441,7442]
\psarccircP 7453 ; 0.102018 [7451,7452]
\psarccircP 7463 ; 0.128665 [7461,7462]
\psarccircP 7473 ; 0.029880 [7471,7472]
\psarccircP 7483 ; 0.019146 [7481,7482]
\psarccircP 7493 ; 0.018843 [7491,7492]
\psarccircP 7503 ; 0.028171 [7501,7502]
\psarccircP 7513 ; 0.102018 [7511,7512]
\psarccircP 7523 ; 0.053295 [7521,7522]
\psarccircP 7533 ; 0.102018 [7531,7532]
\psarccircP 7543 ; 0.038918 [7541,7542]
\psarccircP 7553 ; 0.014940 [7551,7552]
\psarccircP 7563 ; 0.011141 [7561,7562]
\psarccircP 7573 ; 0.012377 [7571,7572]
\psarccircP 7583 ; 0.022075 [7581,7582]
\psarccircP 7593 ; 0.246293 [7591,7592]
\psarccircP 7603 ; 0.043814 [7601,7602]
\psarccircP 7613 ; 0.246293 [7611,7612]
\psarccircP 7623 ; 0.024249 [7621,7622]
\psarccircP 7633 ; 0.011556 [7631,7632]
\psarccircP 7643 ; 0.009497 [7641,7642]
\psarccircP 7653 ; 0.011556 [7651,7652]
\psarccircP 7663 ; 0.024249 [7661,7662]
\psarccircP 7673 ; 0.246293 [7671,7672]
\psarccircP 7683 ; 0.053295 [7681,7682]
\psarccircP 7693 ; 0.246293 [7691,7692]
\psarccircP 7703 ; 0.022075 [7701,7702]
\psarccircP 7713 ; 0.012377 [7711,7712]
\psarccircP 7723 ; 0.011141 [7721,7722]
\psarccircP 7733 ; 0.014940 [7731,7732]
\psarccircP 7743 ; 0.038918 [7741,7742]
\psarccircP 7753 ; 0.102018 [7751,7752]
\psarccircP 7763 ; 0.102018 [7761,7762]
\psarccircP 7773 ; 0.111591 [7771,7772]
\psarccircP 7783 ; 0.102018 [7781,7782]
\psarccircP 7793 ; 0.028171 [7791,7792]
\psarccircP 7803 ; 0.018843 [7801,7802]
\psarccircP 7813 ; 0.019146 [7811,7812]
\psarccircP 7823 ; 0.029880 [7821,7822]
\psarccircP 7833 ; 0.128665 [7831,7832]
\psarccircP 7843 ; 0.056901 [7841,7842]
\psarccircP 7853 ; 0.128665 [7851,7852]
\psarccircP 7863 ; 0.038918 [7861,7862]
\psarccircP 7873 ; 0.015817 [7871,7872]
\psarccircP 7883 ; 0.012073 [7881,7882]
\psarccircP 7893 ; 0.013694 [7891,7892]
\psarccircP 7903 ; 0.025280 [7901,7902]
\psarccircP 7913 ; 0.492586 [7911,7912]
\psarccircP 7923 ; 0.051009 [7921,7922]
\psarccircP 7933 ; 0.492586 [7931,7932]
\psarccircP 7943 ; 0.026647 [7941,7942]
\psarccircP 7953 ; 0.013176 [7951,7952]
\psarccircP 7963 ; 0.011038 [7961,7962]
\psarccircP 7973 ; 0.013694 [7971,7972]
\psarccircP 7983 ; 0.029880 [7981,7982]
\psarccircP 7993 ; 0.204036 [7991,7992]
\psarccircP 8003 ; 0.068012 [8001,8002]
\psarccircP 8013 ; 0.204036 [8011,8012]
\psarccircP 8023 ; 0.026063 [8021,8022]
\psarccircP 8033 ; 0.015130 [8031,8032]
\psarccircP 8043 ; 0.013921 [8041,8042]
\psarccircP 8053 ; 0.019146 [8051,8052]
\psarccircP 8063 ; 0.053295 [8061,8062]
\psarccircP 8073 ; 0.111591 [8071,8072]
\psarccircP 8083 ; 0.128665 [8081,8082]
\psarccircP 8093 ; 0.174155 [8091,8092]
\psarccircP 8103 ; 0.111591 [8101,8102]
\psarccircP 8113 ; 0.036069 [8111,8112]
\psarccircP 8123 ; 0.025280 [8121,8122]
\psarccircP 8133 ; 0.026647 [8131,8132]
\psarccircP 8143 ; 0.043814 [8141,8142]
\psarccircP 8153 ; 0.246293 [8151,8152]
\psarccircP 8163 ; 0.084514 [8161,8162]
\psarccircP 8173 ; 0.246293 [8171,8172]
\psarccircP 8183 ; 0.053295 [8181,8182]
\psarccircP 8193 ; 0.023111 [8191,8192]
\psarccircP 8203 ; 0.018148 [8201,8202]
\psarccircP 8213 ; 0.021129 [8211,8212]
\psarccircP 8223 ; 0.040807 [8221,8222]
\psline[8231,8232]
\psarccircP 8243 ; 0.084514 [8241,8242]
\psline[8251,8252]
\psarccircP 8263 ; 0.040807 [8261,8262]
\psarccircP 8273 ; 0.021129 [8271,8272]
\psarccircP 8283 ; 0.018148 [8281,8282]
\psarccircP 8293 ; 0.023111 [8291,8292]
\psarccircP 8303 ; 0.053295 [8301,8302]
\psarccircP 8313 ; 0.246293 [8311,8312]
\psarccircP 8323 ; 0.174155 [8321,8322]
\psarccircP 8333 ; 0.128665 [8331,8332]
\psarccircP 8343 ; 0.246293 [8341,8342]
\psarccircP 8353 ; 0.043814 [8351,8352]
\psarccircP 8363 ; 0.026647 [8361,8362]
\psarccircP 8373 ; 0.025280 [8371,8372]
\psarccircP 8383 ; 0.036069 [8381,8382]
\psarccircP 8393 ; 0.111591 [8391,8392]
\psarccircP 8403 ; 0.068012 [8401,8402]
\psarccircP 8413 ; 0.111591 [8411,8412]
\psarccircP 8423 ; 0.053295 [8421,8422]
\psarccircP 8433 ; 0.019146 [8431,8432]
\psarccircP 8443 ; 0.013921 [8441,8442]
\psarccircP 8453 ; 0.015130 [8451,8452]
\psarccircP 8463 ; 0.026063 [8461,8462]
\psarccircP 8473 ; 0.204036 [8471,8472]
\psarccircP 8483 ; 0.051009 [8481,8482]
\psarccircP 8493 ; 0.204036 [8491,8492]
\psarccircP 8503 ; 0.029880 [8501,8502]
\psarccircP 8513 ; 0.013694 [8511,8512]
\psarccircP 8523 ; 0.011038 [8521,8522]
\psarccircP 8533 ; 0.013176 [8531,8532]
\psarccircP 8543 ; 0.026647 [8541,8542]
\psarccircP 8553 ; 0.492586 [8551,8552]
\psarccircP 8563 ; 0.056901 [8561,8562]
\psarccircP 8573 ; 0.492586 [8571,8572]
\psarccircP 8583 ; 0.025280 [8581,8582]
\psarccircP 8593 ; 0.013694 [8591,8592]
\psarccircP 8603 ; 0.012073 [8601,8602]
\psarccircP 8613 ; 0.015817 [8611,8612]
\psarccircP 8623 ; 0.038918 [8621,8622]
\psarccircP 8633 ; 0.128665 [8631,8632]
\psarccircP 8643 ; 0.111591 [8641,8642]
\psarccircP 8653 ; 0.102018 [8651,8652]
\psarccircP 8663 ; 0.128665 [8661,8662]
\psarccircP 8673 ; 0.029880 [8671,8672]
\psarccircP 8683 ; 0.019146 [8681,8682]
\psarccircP 8693 ; 0.018843 [8691,8692]
\psarccircP 8703 ; 0.028171 [8701,8702]
\psarccircP 8713 ; 0.102018 [8711,8712]
\psarccircP 8723 ; 0.053295 [8721,8722]
\psarccircP 8733 ; 0.102018 [8731,8732]
\psarccircP 8743 ; 0.038918 [8741,8742]
\psarccircP 8753 ; 0.014940 [8751,8752]
\psarccircP 8763 ; 0.011141 [8761,8762]
\psarccircP 8773 ; 0.012377 [8771,8772]
\psarccircP 8783 ; 0.022075 [8781,8782]
\psarccircP 8793 ; 0.246293 [8791,8792]
\psarccircP 8803 ; 0.043814 [8801,8802]
\psarccircP 8813 ; 0.246293 [8811,8812]
\psarccircP 8823 ; 0.024249 [8821,8822]
\psarccircP 8833 ; 0.011556 [8831,8832]
\psarccircP 8843 ; 0.009497 [8841,8842]
\psarccircP 8853 ; 0.011556 [8851,8852]
\psarccircP 8863 ; 0.024249 [8861,8862]
\psarccircP 8873 ; 0.246293 [8871,8872]
\psarccircP 8883 ; 0.053295 [8881,8882]
\psarccircP 8893 ; 0.246293 [8891,8892]
\psarccircP 8903 ; 0.022075 [8901,8902]
\psarccircP 8913 ; 0.012377 [8911,8912]
\psarccircP 8923 ; 0.011141 [8921,8922]
\psarccircP 8933 ; 0.014940 [8931,8932]
\psarccircP 8943 ; 0.038918 [8941,8942]
\psarccircP 8953 ; 0.102018 [8951,8952]
\psarccircP 8963 ; 0.102018 [8961,8962]
\psarccircP 8973 ; 0.111591 [8971,8972]
\psarccircP 8983 ; 0.102018 [8981,8982]
\psarccircP 8993 ; 0.028171 [8991,8992]
\psarccircP 9003 ; 0.018843 [9001,9002]
\psarccircP 9013 ; 0.019146 [9011,9012]
\psarccircP 9023 ; 0.029880 [9021,9022]
\psarccircP 9033 ; 0.128665 [9031,9032]
\psarccircP 9043 ; 0.056901 [9041,9042]
\psarccircP 9053 ; 0.128665 [9051,9052]
\psarccircP 9063 ; 0.038918 [9061,9062]
\psarccircP 9073 ; 0.015817 [9071,9072]
\psarccircP 9083 ; 0.012073 [9081,9082]
\psarccircP 9093 ; 0.013694 [9091,9092]
\psarccircP 9103 ; 0.025280 [9101,9102]
\psarccircP 9113 ; 0.492586 [9111,9112]
\psarccircP 9123 ; 0.051009 [9121,9122]
\psarccircP 9133 ; 0.492586 [9131,9132]
\psarccircP 9143 ; 0.026647 [9141,9142]
\psarccircP 9153 ; 0.013176 [9151,9152]
\psarccircP 9163 ; 0.011038 [9161,9162]
\psarccircP 9173 ; 0.013694 [9171,9172]
\psarccircP 9183 ; 0.029880 [9181,9182]
\psarccircP 9193 ; 0.204036 [9191,9192]
\psarccircP 9203 ; 0.068012 [9201,9202]
\psarccircP 9213 ; 0.204036 [9211,9212]
\psarccircP 9223 ; 0.026063 [9221,9222]
\psarccircP 9233 ; 0.015130 [9231,9232]
\psarccircP 9243 ; 0.013921 [9241,9242]
\psarccircP 9253 ; 0.019146 [9251,9252]
\psarccircP 9263 ; 0.053295 [9261,9262]
\psarccircP 9273 ; 0.111591 [9271,9272]
\psarccircP 9283 ; 0.128665 [9281,9282]
\psarccircP 9293 ; 0.174155 [9291,9292]
\psarccircP 9303 ; 0.111591 [9301,9302]
\psarccircP 9313 ; 0.036069 [9311,9312]
\psarccircP 9323 ; 0.025280 [9321,9322]
\psarccircP 9333 ; 0.026647 [9331,9332]
\psarccircP 9343 ; 0.043814 [9341,9342]
\psarccircP 9353 ; 0.246293 [9351,9352]
\psarccircP 9363 ; 0.084514 [9361,9362]
\psarccircP 9373 ; 0.246293 [9371,9372]
\psarccircP 9383 ; 0.053295 [9381,9382]
\psarccircP 9393 ; 0.023111 [9391,9392]
\psarccircP 9403 ; 0.018148 [9401,9402]
\psarccircP 9413 ; 0.021129 [9411,9412]
\psarccircP 9423 ; 0.040807 [9421,9422]
\psline[9431,9432]
\psarccircP 9443 ; 0.084514 [9441,9442]
\psline[9451,9452]
\psarccircP 9463 ; 0.040807 [9461,9462]
\psarccircP 9473 ; 0.021129 [9471,9472]
\psarccircP 9483 ; 0.018148 [9481,9482]
\psarccircP 9493 ; 0.023111 [9491,9492]
\psarccircP 9503 ; 0.053295 [9501,9502]
\psarccircP 9513 ; 0.246293 [9511,9512]
\psarccircP 9523 ; 0.174155 [9521,9522]
\psarccircP 9533 ; 0.128665 [9531,9532]
\psarccircP 9543 ; 0.246293 [9541,9542]
\psarccircP 9553 ; 0.043814 [9551,9552]
\psarccircP 9563 ; 0.026647 [9561,9562]
\psarccircP 9573 ; 0.025280 [9571,9572]
\psarccircP 9583 ; 0.036069 [9581,9582]
\psarccircP 9593 ; 0.111591 [9591,9592]
\psarccircP 9603 ; 0.068012 [9601,9602]
\psarccircP 9613 ; 0.111591 [9611,9612]
\psarccircP 9623 ; 0.053295 [9621,9622]
\psarccircP 9633 ; 0.019146 [9631,9632]
\psarccircP 9643 ; 0.013921 [9641,9642]
\psarccircP 9653 ; 0.015130 [9651,9652]
\psarccircP 9663 ; 0.026063 [9661,9662]
\psarccircP 9673 ; 0.204036 [9671,9672]
\psarccircP 9683 ; 0.051009 [9681,9682]
\psarccircP 9693 ; 0.204036 [9691,9692]
\psarccircP 9703 ; 0.029880 [9701,9702]
\psarccircP 9713 ; 0.013694 [9711,9712]
\psarccircP 9723 ; 0.011038 [9721,9722]
\psarccircP 9733 ; 0.013176 [9731,9732]
\psarccircP 9743 ; 0.026647 [9741,9742]
\psarccircP 9753 ; 0.492586 [9751,9752]
\psarccircP 9763 ; 0.056901 [9761,9762]
\psarccircP 9773 ; 0.492586 [9771,9772]
\psarccircP 9783 ; 0.025280 [9781,9782]
\psarccircP 9793 ; 0.013694 [9791,9792]
\psarccircP 9803 ; 0.012073 [9801,9802]
\psarccircP 9813 ; 0.015817 [9811,9812]
\psarccircP 9823 ; 0.038918 [9821,9822]
\psarccircP 9833 ; 0.128665 [9831,9832]
\psarccircP 9843 ; 0.111591 [9841,9842]
\psarccircP 9853 ; 0.102018 [9851,9852]
\psarccircP 9863 ; 0.128665 [9861,9862]
\psarccircP 9873 ; 0.029880 [9871,9872]
\psarccircP 9883 ; 0.019146 [9881,9882]
\psarccircP 9893 ; 0.018843 [9891,9892]
\psarccircP 9903 ; 0.028171 [9901,9902]
\psarccircP 9913 ; 0.102018 [9911,9912]
\psarccircP 9923 ; 0.053295 [9921,9922]
\psarccircP 9933 ; 0.102018 [9931,9932]
\psarccircP 9943 ; 0.038918 [9941,9942]
\psarccircP 9953 ; 0.014940 [9951,9952]
\psarccircP 9963 ; 0.011141 [9961,9962]
\psarccircP 9973 ; 0.012377 [9971,9972]
\psarccircP 9983 ; 0.022075 [9981,9982]
\psarccircP 9993 ; 0.246293 [9991,9992]
\psarccircP 10003 ; 0.043814 [10001,10002]
\psarccircP 10013 ; 0.246293 [10011,10012]
\psarccircP 10023 ; 0.024249 [10021,10022]
\psarccircP 10033 ; 0.011556 [10031,10032]
\psarccircP 10043 ; 0.009497 [10041,10042]
\psarccircP 10053 ; 0.011556 [10051,10052]
\psarccircP 10063 ; 0.024249 [10061,10062]
\psarccircP 10073 ; 0.246293 [10071,10072]
\psarccircP 10083 ; 0.053295 [10081,10082]
\psarccircP 10093 ; 0.246293 [10091,10092]
\psarccircP 10103 ; 0.022075 [10101,10102]
\psarccircP 10113 ; 0.012377 [10111,10112]
\psarccircP 10123 ; 0.011141 [10121,10122]
\psarccircP 10133 ; 0.014940 [10131,10132]
\psarccircP 10143 ; 0.038918 [10141,10142]
\psarccircP 10153 ; 0.102018 [10151,10152]
\psarccircP 10163 ; 0.102018 [10161,10162]
\psarccircP 10173 ; 0.111591 [10171,10172]
\psarccircP 10183 ; 0.102018 [10181,10182]
\psarccircP 10193 ; 0.028171 [10191,10192]
\psarccircP 10203 ; 0.018843 [10201,10202]
\psarccircP 10213 ; 0.019146 [10211,10212]
\psarccircP 10223 ; 0.029880 [10221,10222]
\psarccircP 10233 ; 0.128665 [10231,10232]
\psarccircP 10243 ; 0.056901 [10241,10242]
\psarccircP 10253 ; 0.128665 [10251,10252]
\psarccircP 10263 ; 0.038918 [10261,10262]
\psarccircP 10273 ; 0.015817 [10271,10272]
\psarccircP 10283 ; 0.012073 [10281,10282]
\psarccircP 10293 ; 0.013694 [10291,10292]
\psarccircP 10303 ; 0.025280 [10301,10302]
\psarccircP 10313 ; 0.492586 [10311,10312]
\psarccircP 10323 ; 0.051009 [10321,10322]
\psarccircP 10333 ; 0.492586 [10331,10332]
\psarccircP 10343 ; 0.026647 [10341,10342]
\psarccircP 10353 ; 0.013176 [10351,10352]
\psarccircP 10363 ; 0.011038 [10361,10362]
\psarccircP 10373 ; 0.013694 [10371,10372]
\psarccircP 10383 ; 0.029880 [10381,10382]
\psarccircP 10393 ; 0.204036 [10391,10392]
\psarccircP 10403 ; 0.068012 [10401,10402]
\psarccircP 10413 ; 0.204036 [10411,10412]
\psarccircP 10423 ; 0.026063 [10421,10422]
\psarccircP 10433 ; 0.015130 [10431,10432]
\psarccircP 10443 ; 0.013921 [10441,10442]
\psarccircP 10453 ; 0.019146 [10451,10452]
\psarccircP 10463 ; 0.053295 [10461,10462]
\psarccircP 10473 ; 0.111591 [10471,10472]
\psarccircP 10483 ; 0.128665 [10481,10482]
\psarccircP 10493 ; 0.174155 [10491,10492]
\psarccircP 10503 ; 0.111591 [10501,10502]
\psarccircP 10513 ; 0.036069 [10511,10512]
\psarccircP 10523 ; 0.025280 [10521,10522]
\psarccircP 10533 ; 0.026647 [10531,10532]
\psarccircP 10543 ; 0.043814 [10541,10542]
\psarccircP 10553 ; 0.246293 [10551,10552]
\psarccircP 10563 ; 0.084514 [10561,10562]
\psarccircP 10573 ; 0.246293 [10571,10572]
\psarccircP 10583 ; 0.053295 [10581,10582]
\psarccircP 10593 ; 0.023111 [10591,10592]
\psarccircP 10603 ; 0.018148 [10601,10602]
\psarccircP 10613 ; 0.021129 [10611,10612]
\psarccircP 10623 ; 0.040807 [10621,10622]
\psline[10631,10632]
\psarccircP 10643 ; 0.084514 [10641,10642]
\psline[10651,10652]
\psarccircP 10663 ; 0.040807 [10661,10662]
\psarccircP 10673 ; 0.021129 [10671,10672]
\psarccircP 10683 ; 0.018148 [10681,10682]
\psarccircP 10693 ; 0.023111 [10691,10692]
\psarccircP 10703 ; 0.053295 [10701,10702]
\psarccircP 10713 ; 0.246293 [10711,10712]
\psarccircP 10723 ; 0.174155 [10721,10722]
\psarccircP 10733 ; 0.128665 [10731,10732]
\psarccircP 10743 ; 0.246293 [10741,10742]
\psarccircP 10753 ; 0.043814 [10751,10752]
\psarccircP 10763 ; 0.026647 [10761,10762]
\psarccircP 10773 ; 0.025280 [10771,10772]
\psarccircP 10783 ; 0.036069 [10781,10782]
\psarccircP 10793 ; 0.111591 [10791,10792]
\psarccircP 10803 ; 0.068012 [10801,10802]
\psarccircP 10813 ; 0.111591 [10811,10812]
\psarccircP 10823 ; 0.053295 [10821,10822]
\psarccircP 10833 ; 0.019146 [10831,10832]
\psarccircP 10843 ; 0.013921 [10841,10842]
\psarccircP 10853 ; 0.015130 [10851,10852]
\psarccircP 10863 ; 0.026063 [10861,10862]
\psarccircP 10873 ; 0.204036 [10871,10872]
\psarccircP 10883 ; 0.051009 [10881,10882]
\psarccircP 10893 ; 0.204036 [10891,10892]
\psarccircP 10903 ; 0.029880 [10901,10902]
\psarccircP 10913 ; 0.013694 [10911,10912]
\psarccircP 10923 ; 0.011038 [10921,10922]
\psarccircP 10933 ; 0.013176 [10931,10932]
\psarccircP 10943 ; 0.026647 [10941,10942]
\psarccircP 10953 ; 0.492586 [10951,10952]
\psarccircP 10963 ; 0.056901 [10961,10962]
\psarccircP 10973 ; 0.492586 [10971,10972]
\psarccircP 10983 ; 0.025280 [10981,10982]
\psarccircP 10993 ; 0.013694 [10991,10992]
\psarccircP 11003 ; 0.012073 [11001,11002]
\psarccircP 11013 ; 0.015817 [11011,11012]
\psarccircP 11023 ; 0.038918 [11021,11022]
\psarccircP 11033 ; 0.128665 [11031,11032]
\psarccircP 11043 ; 0.111591 [11041,11042]
\psarccircP 11053 ; 0.102018 [11051,11052]
\psarccircP 11063 ; 0.128665 [11061,11062]
\psarccircP 11073 ; 0.029880 [11071,11072]
\psarccircP 11083 ; 0.019146 [11081,11082]
\psarccircP 11093 ; 0.018843 [11091,11092]
\psarccircP 11103 ; 0.028171 [11101,11102]
\psarccircP 11113 ; 0.102018 [11111,11112]
\psarccircP 11123 ; 0.053295 [11121,11122]
\psarccircP 11133 ; 0.102018 [11131,11132]
\psarccircP 11143 ; 0.038918 [11141,11142]
\psarccircP 11153 ; 0.014940 [11151,11152]
\psarccircP 11163 ; 0.011141 [11161,11162]
\psarccircP 11173 ; 0.012377 [11171,11172]
\psarccircP 11183 ; 0.022075 [11181,11182]
\psarccircP 11193 ; 0.246293 [11191,11192]
\psarccircP 11203 ; 0.043814 [11201,11202]
\psarccircP 11213 ; 0.246293 [11211,11212]
\psarccircP 11223 ; 0.024249 [11221,11222]
\psarccircP 11233 ; 0.011556 [11231,11232]
\psarccircP 11243 ; 0.009497 [11241,11242]
\psarccircP 11253 ; 0.011556 [11251,11252]
\psarccircP 11263 ; 0.024249 [11261,11262]
\psarccircP 11273 ; 0.246293 [11271,11272]
\psarccircP 11283 ; 0.053295 [11281,11282]
\psarccircP 11293 ; 0.246293 [11291,11292]
\psarccircP 11303 ; 0.022075 [11301,11302]
\psarccircP 11313 ; 0.012377 [11311,11312]
\psarccircP 11323 ; 0.011141 [11321,11322]
\psarccircP 11333 ; 0.014940 [11331,11332]
\psarccircP 11343 ; 0.038918 [11341,11342]
\psarccircP 11353 ; 0.102018 [11351,11352]
\psarccircP 11363 ; 0.102018 [11361,11362]
\psarccircP 11373 ; 0.111591 [11371,11372]
\psarccircP 11383 ; 0.102018 [11381,11382]
\psarccircP 11393 ; 0.028171 [11391,11392]
\psarccircP 11403 ; 0.018843 [11401,11402]
\psarccircP 11413 ; 0.019146 [11411,11412]
\psarccircP 11423 ; 0.029880 [11421,11422]
\psarccircP 11433 ; 0.128665 [11431,11432]
\psarccircP 11443 ; 0.056901 [11441,11442]
\psarccircP 11453 ; 0.128665 [11451,11452]
\psarccircP 11463 ; 0.038918 [11461,11462]
\psarccircP 11473 ; 0.015817 [11471,11472]
\psarccircP 11483 ; 0.012073 [11481,11482]
\psarccircP 11493 ; 0.013694 [11491,11492]
\psarccircP 11503 ; 0.025280 [11501,11502]
\psarccircP 11513 ; 0.492586 [11511,11512]
\psarccircP 11523 ; 0.051009 [11521,11522]
\psarccircP 11533 ; 0.492586 [11531,11532]
\psarccircP 11543 ; 0.026647 [11541,11542]
\psarccircP 11553 ; 0.013176 [11551,11552]
\psarccircP 11563 ; 0.011038 [11561,11562]
\psarccircP 11573 ; 0.013694 [11571,11572]
\psarccircP 11583 ; 0.029880 [11581,11582]
\psarccircP 11593 ; 0.204036 [11591,11592]
\psarccircP 11603 ; 0.068012 [11601,11602]
\psarccircP 11613 ; 0.204036 [11611,11612]
\psarccircP 11623 ; 0.026063 [11621,11622]
\psarccircP 11633 ; 0.015130 [11631,11632]
\psarccircP 11643 ; 0.013921 [11641,11642]
\psarccircP 11653 ; 0.019146 [11651,11652]
\psarccircP 11663 ; 0.053295 [11661,11662]
\psarccircP 11673 ; 0.111591 [11671,11672]
\psarccircP 11683 ; 0.128665 [11681,11682]
\psarccircP 11693 ; 0.174155 [11691,11692]
\psarccircP 11703 ; 0.111591 [11701,11702]
\psarccircP 11713 ; 0.036069 [11711,11712]
\psarccircP 11723 ; 0.025280 [11721,11722]
\psarccircP 11733 ; 0.026647 [11731,11732]
\psarccircP 11743 ; 0.043814 [11741,11742]
\psarccircP 11753 ; 0.246293 [11751,11752]
\psarccircP 11763 ; 0.084514 [11761,11762]
\psarccircP 11773 ; 0.246293 [11771,11772]
\psarccircP 11783 ; 0.053295 [11781,11782]
\psarccircP 11793 ; 0.023111 [11791,11792]
\psarccircP 11803 ; 0.018148 [11801,11802]
\psarccircP 11813 ; 0.021129 [11811,11812]
\psarccircP 11823 ; 0.040807 [11821,11822]
\psline[11831,11832]
\psarccircP 11843 ; 0.084514 [11841,11842]
\psline[11851,11852]
\psarccircP 11863 ; 0.040807 [11861,11862]
\psarccircP 11873 ; 0.021129 [11871,11872]
\psarccircP 11883 ; 0.018148 [11881,11882]
\psarccircP 11893 ; 0.023111 [11891,11892]
\psarccircP 11903 ; 0.053295 [11901,11902]
\psarccircP 11913 ; 0.246293 [11911,11912]
\psarccircP 11923 ; 0.174155 [11921,11922]
\psarccircP 11933 ; 0.128665 [11931,11932]
\psarccircP 11943 ; 0.246293 [11941,11942]
\psarccircP 11953 ; 0.043814 [11951,11952]
\psarccircP 11963 ; 0.026647 [11961,11962]
\psarccircP 11973 ; 0.025280 [11971,11972]
\psarccircP 11983 ; 0.036069 [11981,11982]
\psarccircP 11993 ; 0.111591 [11991,11992]
\psarccircP 12003 ; 0.068012 [12001,12002]
\psarccircP 12013 ; 0.111591 [12011,12012]
\psarccircP 12023 ; 0.053295 [12021,12022]
\psarccircP 12033 ; 0.019146 [12031,12032]
\psarccircP 12043 ; 0.013921 [12041,12042]
\psarccircP 12053 ; 0.015130 [12051,12052]
\psarccircP 12063 ; 0.026063 [12061,12062]
\psarccircP 12073 ; 0.204036 [12071,12072]
\psarccircP 12083 ; 0.051009 [12081,12082]
\psarccircP 12093 ; 0.204036 [12091,12092]
\psarccircP 12103 ; 0.029880 [12101,12102]
\psarccircP 12113 ; 0.013694 [12111,12112]
\psarccircP 12123 ; 0.011038 [12121,12122]
\psarccircP 12133 ; 0.013176 [12131,12132]
\psarccircP 12143 ; 0.026647 [12141,12142]
\psarccircP 12153 ; 0.492586 [12151,12152]
\psarccircP 12163 ; 0.056901 [12161,12162]
\psarccircP 12173 ; 0.492586 [12171,12172]
\psarccircP 12183 ; 0.025280 [12181,12182]
\psarccircP 12193 ; 0.013694 [12191,12192]
\psarccircP 12203 ; 0.012073 [12201,12202]
\psarccircP 12213 ; 0.015817 [12211,12212]
\psarccircP 12223 ; 0.038918 [12221,12222]
\psarccircP 12233 ; 0.128665 [12231,12232]
\psarccircP 12243 ; 0.111591 [12241,12242]
\psarccircP 12253 ; 0.102018 [12251,12252]
\psarccircP 12263 ; 0.128665 [12261,12262]
\psarccircP 12273 ; 0.029880 [12271,12272]
\psarccircP 12283 ; 0.019146 [12281,12282]
\psarccircP 12293 ; 0.018843 [12291,12292]
\psarccircP 12303 ; 0.028171 [12301,12302]
\psarccircP 12313 ; 0.102018 [12311,12312]
\psarccircP 12323 ; 0.053295 [12321,12322]
\psarccircP 12333 ; 0.102018 [12331,12332]
\psarccircP 12343 ; 0.038918 [12341,12342]
\psarccircP 12353 ; 0.014940 [12351,12352]
\psarccircP 12363 ; 0.011141 [12361,12362]
\psarccircP 12373 ; 0.012377 [12371,12372]
\psarccircP 12383 ; 0.022075 [12381,12382]
\psarccircP 12393 ; 0.246293 [12391,12392]
\psarccircP 12403 ; 0.043814 [12401,12402]
\psarccircP 12413 ; 0.246293 [12411,12412]
\psarccircP 12423 ; 0.024249 [12421,12422]
\psarccircP 12433 ; 0.011556 [12431,12432]
\psarccircP 12443 ; 0.009497 [12441,12442]
\psarccircP 12453 ; 0.011556 [12451,12452]
\psarccircP 12463 ; 0.024249 [12461,12462]
\psarccircP 12473 ; 0.246293 [12471,12472]
\psarccircP 12483 ; 0.053295 [12481,12482]
\psarccircP 12493 ; 0.246293 [12491,12492]
\psarccircP 12503 ; 0.022075 [12501,12502]
\psarccircP 12513 ; 0.012377 [12511,12512]
\psarccircP 12523 ; 0.011141 [12521,12522]
\psarccircP 12533 ; 0.014940 [12531,12532]
\psarccircP 12543 ; 0.038918 [12541,12542]
\psarccircP 12553 ; 0.102018 [12551,12552]
\psarccircP 12563 ; 0.102018 [12561,12562]
\psarccircP 12573 ; 0.111591 [12571,12572]
\psarccircP 12583 ; 0.102018 [12581,12582]
\psarccircP 12593 ; 0.028171 [12591,12592]
\psarccircP 12603 ; 0.018843 [12601,12602]
\psarccircP 12613 ; 0.019146 [12611,12612]
\psarccircP 12623 ; 0.029880 [12621,12622]
\psarccircP 12633 ; 0.128665 [12631,12632]
\psarccircP 12643 ; 0.056901 [12641,12642]
\psarccircP 12653 ; 0.128665 [12651,12652]
\psarccircP 12663 ; 0.038918 [12661,12662]
\psarccircP 12673 ; 0.015817 [12671,12672]
\psarccircP 12683 ; 0.012073 [12681,12682]
\psarccircP 12693 ; 0.013694 [12691,12692]
\psarccircP 12703 ; 0.025280 [12701,12702]
\psarccircP 12713 ; 0.492586 [12711,12712]
\psarccircP 12723 ; 0.051009 [12721,12722]
\psarccircP 12733 ; 0.492586 [12731,12732]
\psarccircP 12743 ; 0.026647 [12741,12742]
\psarccircP 12753 ; 0.013176 [12751,12752]
\psarccircP 12763 ; 0.011038 [12761,12762]
\psarccircP 12773 ; 0.013694 [12771,12772]
\psarccircP 12783 ; 0.029880 [12781,12782]
\psarccircP 12793 ; 0.204036 [12791,12792]
\psarccircP 12803 ; 0.068012 [12801,12802]
\psarccircP 12813 ; 0.204036 [12811,12812]
\psarccircP 12823 ; 0.026063 [12821,12822]
\psarccircP 12833 ; 0.015130 [12831,12832]
\psarccircP 12843 ; 0.013921 [12841,12842]
\psarccircP 12853 ; 0.019146 [12851,12852]
\psarccircP 12863 ; 0.053295 [12861,12862]
\psarccircP 12873 ; 0.111591 [12871,12872]


==> fig1-0pt.tex <==
\figpt 1:(-0.155223,0.374741)
\figpt 2:(0.155223,0.374741)
\figpt 3:(-0.000000,1.553774)
\figpt 11:(-0.374741,0.155223)
\figpt 12:(-0.155223,0.374741)
\figpt 13:(-1.098684,1.098684)
\figpt 21:(-0.374741,-0.155223)
\figpt 22:(-0.374741,0.155223)
\figpt 23:(-1.553774,-0.000000)
\figpt 31:(-0.155223,-0.374741)
\figpt 32:(-0.374741,-0.155223)
\figpt 33:(-1.098684,-1.098684)
\figpt 41:(0.155223,-0.374741)
\figpt 42:(-0.155223,-0.374741)
\figpt 43:(-0.000000,-1.553774)
\figpt 51:(0.374741,-0.155223)
\figpt 52:(0.155223,-0.374741)
\figpt 53:(1.098684,-1.098684)
\figpt 61:(0.374741,0.155223)
\figpt 62:(0.374741,-0.155223)
\figpt 63:(1.553774,-0.000000)
\figpt 71:(0.155223,0.374741)
\figpt 72:(0.374741,0.155223)
\figpt 73:(1.098684,1.098684)
\figpt 81:(-0.374741,-0.155223)
\figpt 82:(-0.374741,0.155223)
\figpt 83:(-1.553774,-0.000000)
\figpt 91:(-0.610313,0.252800)
\figpt 92:(-0.374741,0.155223)
\figpt 101:(-0.764226,0.173128)
\figpt 102:(-0.610313,0.252800)
\figpt 103:(-0.910180,0.643594)
\figpt 111:(-0.825177,0.058643)
\figpt 112:(-0.764226,0.173128)
\figpt 113:(-1.004432,0.227545)
\figpt 121:(-0.825177,-0.058643)
\figpt 122:(-0.825177,0.058643)
\figpt 123:(-1.020603,-0.000000)
\figpt 131:(-0.764226,-0.173128)
\figpt 132:(-0.825177,-0.058643)
\figpt 133:(-1.004432,-0.227545)
\figpt 141:(-0.610313,-0.252800)
\figpt 142:(-0.764226,-0.173128)
\figpt 143:(-0.910180,-0.643594)
\figpt 151:(-0.610313,-0.252800)
\figpt 152:(-0.374741,-0.155223)
\figpt 161:(-0.155223,-0.374741)
\figpt 162:(-0.374741,-0.155223)
\figpt 163:(-1.098684,-1.098684)
\figpt 171:(-0.374741,-0.155223)
\figpt 172:(-0.610313,-0.252800)
\figpt 181:(-0.662809,-0.417969)
\figpt 182:(-0.610313,-0.252800)
\figpt 183:(-1.098684,-0.188504)
\figpt 191:(-0.624955,-0.542021)
\figpt 192:(-0.662809,-0.417969)
\figpt 193:(-0.871139,-0.549342)
\figpt 201:(-0.542021,-0.624955)
\figpt 202:(-0.624955,-0.542021)
\figpt 203:(-0.721675,-0.721675)
\figpt 211:(-0.417969,-0.662809)
\figpt 212:(-0.542021,-0.624955)
\figpt 213:(-0.549342,-0.871139)
\figpt 221:(-0.252800,-0.610313)
\figpt 222:(-0.417969,-0.662809)
\figpt 223:(-0.188504,-1.098684)
\figpt 231:(-0.155223,-0.374741)
\figpt 232:(-0.252800,-0.610313)
\figpt 241:(0.155223,-0.374741)
\figpt 242:(-0.155223,-0.374741)
\figpt 243:(-0.000000,-1.553774)
\figpt 251:(-0.252800,-0.610313)
\figpt 252:(-0.155223,-0.374741)
\figpt 261:(-0.173128,-0.764226)
\figpt 262:(-0.252800,-0.610313)
\figpt 263:(-0.643594,-0.910180)
\figpt 271:(-0.058643,-0.825177)
\figpt 272:(-0.173128,-0.764226)
\figpt 273:(-0.227545,-1.004432)
\figpt 281:(0.058643,-0.825177)
\figpt 282:(-0.058643,-0.825177)
\figpt 283:(-0.000000,-1.020603)
\figpt 291:(0.173128,-0.764226)
\figpt 292:(0.058643,-0.825177)
\figpt 293:(0.227545,-1.004432)
\figpt 301:(0.252800,-0.610313)
\figpt 302:(0.173128,-0.764226)
\figpt 303:(0.643594,-0.910180)
\figpt 311:(0.155223,-0.374741)
\figpt 312:(0.252800,-0.610313)
\figpt 321:(0.374741,-0.155223)
\figpt 322:(0.155223,-0.374741)
\figpt 323:(1.098684,-1.098684)
\figpt 331:(0.155223,-0.374741)
\figpt 332:(0.252800,-0.610313)
\figpt 341:(0.417969,-0.662809)
\figpt 342:(0.252800,-0.610313)
\figpt 343:(0.188504,-1.098684)
\figpt 351:(0.542021,-0.624955)
\figpt 352:(0.417969,-0.662809)
\figpt 353:(0.549342,-0.871139)
\figpt 361:(0.624955,-0.542021)
\figpt 362:(0.542021,-0.624955)
\figpt 363:(0.721675,-0.721675)
\figpt 371:(0.662809,-0.417969)
\figpt 372:(0.624955,-0.542021)
\figpt 373:(0.871139,-0.549342)
\figpt 381:(0.610313,-0.252800)
\figpt 382:(0.662809,-0.417969)
\figpt 383:(1.098684,-0.188504)
\figpt 391:(0.610313,-0.252800)
\figpt 392:(0.374741,-0.155223)
\figpt 401:(0.374741,0.155223)
\figpt 402:(0.374741,-0.155223)
\figpt 403:(1.553774,-0.000000)
\figpt 411:(0.374741,-0.155223)
\figpt 412:(0.610313,-0.252800)
\figpt 421:(0.764226,-0.173128)
\figpt 422:(0.610313,-0.252800)
\figpt 423:(0.910180,-0.643594)
\figpt 431:(0.825177,-0.058643)
\figpt 432:(0.764226,-0.173128)
\figpt 433:(1.004432,-0.227545)
\figpt 441:(0.825177,0.058643)
\figpt 442:(0.825177,-0.058643)
\figpt 443:(1.020603,-0.000000)
\figpt 451:(0.764226,0.173128)
\figpt 452:(0.825177,0.058643)
\figpt 453:(1.004432,0.227545)
\figpt 461:(0.610313,0.252800)
\figpt 462:(0.764226,0.173128)
\figpt 463:(0.910180,0.643594)
\figpt 471:(0.374741,0.155223)
\figpt 472:(0.610313,0.252800)
\figpt 481:(0.155223,0.374741)
\figpt 482:(0.374741,0.155223)
\figpt 483:(1.098684,1.098684)
\figpt 491:(0.610313,0.252800)
\figpt 492:(0.374741,0.155223)
\figpt 501:(0.662809,0.417969)
\figpt 502:(0.610313,0.252800)
\figpt 503:(1.098684,0.188504)
\figpt 511:(0.624955,0.542021)
\figpt 512:(0.662809,0.417969)
\figpt 513:(0.871139,0.549342)
\figpt 521:(0.542021,0.624955)
\figpt 522:(0.624955,0.542021)
\figpt 523:(0.721675,0.721675)
\figpt 531:(0.417969,0.662809)
\figpt 532:(0.542021,0.624955)
\figpt 533:(0.549342,0.871139)
\figpt 541:(0.252800,0.610313)
\figpt 542:(0.417969,0.662809)
\figpt 543:(0.188504,1.098684)
\figpt 551:(0.252800,0.610313)
\figpt 552:(0.155223,0.374741)
\figpt 561:(-0.155223,0.374741)
\figpt 562:(0.155223,0.374741)
\figpt 563:(-0.000000,1.553774)
\figpt 571:(0.155223,0.374741)
\figpt 572:(0.252800,0.610313)
\figpt 581:(0.173128,0.764226)
\figpt 582:(0.252800,0.610313)
\figpt 583:(0.643594,0.910180)
\figpt 591:(0.058643,0.825177)
\figpt 592:(0.173128,0.764226)
\figpt 593:(0.227545,1.004432)
\figpt 601:(-0.058643,0.825177)
\figpt 602:(0.058643,0.825177)
\figpt 603:(-0.000000,1.020603)
\figpt 611:(-0.173128,0.764226)
\figpt 612:(-0.058643,0.825177)
\figpt 613:(-0.227545,1.004432)
\figpt 621:(-0.252800,0.610313)
\figpt 622:(-0.173128,0.764226)
\figpt 623:(-0.643594,0.910180)
\figpt 631:(-0.252800,0.610313)
\figpt 632:(-0.155223,0.374741)
\figpt 641:(-0.374741,0.155223)
\figpt 642:(-0.155223,0.374741)
\figpt 643:(-1.098684,1.098684)
\figpt 651:(-0.155223,0.374741)
\figpt 652:(-0.252800,0.610313)
\figpt 661:(-0.417969,0.662809)
\figpt 662:(-0.252800,0.610313)
\figpt 663:(-0.188504,1.098684)
\figpt 671:(-0.542021,0.624955)
\figpt 672:(-0.417969,0.662809)
\figpt 673:(-0.549342,0.871139)
\figpt 681:(-0.624955,0.542021)
\figpt 682:(-0.542021,0.624955)
\figpt 683:(-0.721675,0.721675)
\figpt 691:(-0.662809,0.417969)
\figpt 692:(-0.624955,0.542021)
\figpt 693:(-0.871139,0.549342)
\figpt 701:(-0.610313,0.252800)
\figpt 702:(-0.662809,0.417969)
\figpt 703:(-1.098684,0.188504)
\figpt 711:(-0.610313,0.252800)
\figpt 712:(-0.374741,0.155223)
\figpt 721:(-0.764226,0.173128)
\figpt 722:(-0.610313,0.252800)
\figpt 723:(-0.910180,0.643594)
\figpt 731:(-0.610313,0.252800)
\figpt 732:(-0.662809,0.417969)
\figpt 733:(-1.098684,0.188504)
\figpt 741:(-0.769697,0.434009)
\figpt 742:(-0.662809,0.417969)
\figpt 743:(-0.643594,0.910180)
\figpt 751:(-0.828742,0.400152)
\figpt 752:(-0.769697,0.434009)
\figpt 753:(-0.860942,0.524723)
\figpt 761:(-0.858731,0.355698)
\figpt 762:(-0.828742,0.400152)
\figpt 763:(-0.910180,0.422748)
\figpt 771:(-0.868959,0.303059)
\figpt 772:(-0.858731,0.355698)
\figpt 773:(-0.942522,0.344667)
\figpt 781:(-0.851148,0.237367)
\figpt 782:(-0.868959,0.303059)
\figpt 783:(-0.979813,0.237742)
\figpt 791:(-0.764226,0.173128)
\figpt 792:(-0.851148,0.237367)
\figpt 793:(-1.098684,-0.188504)
\figpt 801:(-0.825177,0.058643)
\figpt 802:(-0.764226,0.173128)
\figpt 803:(-1.004432,0.227545)
\figpt 811:(-0.764226,0.173128)
\figpt 812:(-0.851148,0.237367)
\figpt 813:(-1.098684,-0.188504)
\figpt 821:(-0.909353,0.216625)
\figpt 822:(-0.851148,0.237367)
\figpt 823:(-0.937786,0.388443)
\figpt 831:(-0.934090,0.184787)
\figpt 832:(-0.909353,0.216625)
\figpt 833:(-0.973015,0.240558)
\figpt 841:(-0.942506,0.152070)
\figpt 842:(-0.934090,0.184787)
\figpt 843:(-0.984912,0.180419)
\figpt 851:(-0.937666,0.116176)
\figpt 852:(-0.942506,0.152070)
\figpt 853:(-0.993544,0.126915)
\figpt 861:(-0.909079,0.075311)
\figpt 862:(-0.937666,0.116176)
\figpt 863:(-1.004432,0.039041)
\figpt 871:(-0.825177,0.058643)
\figpt 872:(-0.909079,0.075311)
\figpt 873:(-1.098684,-1.098684)
\figpt 881:(-0.825177,-0.058643)
\figpt 882:(-0.825177,0.058643)
\figpt 883:(-1.020603,0.000000)
\figpt 891:(-0.825177,0.058643)
\figpt 892:(-0.909079,0.075311)
\figpt 893:(-1.098684,-1.098684)
\figpt 901:(-0.947058,0.045315)
\figpt 902:(-0.909079,0.075311)
\figpt 903:(-0.995588,0.145800)
\figpt 911:(-0.959665,0.014645)
\figpt 912:(-0.947058,0.045315)
\figpt 913:(-1.000208,0.049238)
\figpt 921:(-0.959665,-0.014645)
\figpt 922:(-0.959665,0.014645)
\figpt 923:(-1.000959,-0.000000)
\figpt 931:(-0.947058,-0.045315)
\figpt 932:(-0.959665,-0.014645)
\figpt 933:(-1.000208,-0.049238)
\figpt 941:(-0.909079,-0.075311)
\figpt 942:(-0.947058,-0.045315)
\figpt 943:(-0.995588,-0.145800)
\figpt 951:(-0.909079,-0.075311)
\figpt 952:(-0.825177,-0.058643)
\figpt 953:(-1.098684,1.098684)
\figpt 961:(-0.764226,-0.173128)
\figpt 962:(-0.825177,-0.058643)
\figpt 963:(-1.004432,-0.227545)
\figpt 971:(-0.909079,-0.075311)
\figpt 972:(-0.825177,-0.058643)
\figpt 973:(-1.098684,1.098684)
\figpt 981:(-0.937666,-0.116176)
\figpt 982:(-0.909079,-0.075311)
\figpt 983:(-1.004432,-0.039041)
\figpt 991:(-0.942506,-0.152070)
\figpt 992:(-0.937666,-0.116176)
\figpt 993:(-0.993544,-0.126915)
\figpt 1001:(-0.934090,-0.184787)
\figpt 1002:(-0.942506,-0.152070)
\figpt 1003:(-0.984912,-0.180419)
\figpt 1011:(-0.909353,-0.216625)
\figpt 1012:(-0.934090,-0.184787)
\figpt 1013:(-0.973015,-0.240558)
\figpt 1021:(-0.851148,-0.237367)
\figpt 1022:(-0.909353,-0.216625)
\figpt 1023:(-0.937786,-0.388443)
\figpt 1031:(-0.851148,-0.237367)
\figpt 1032:(-0.764226,-0.173128)
\figpt 1033:(-1.098684,0.188504)
\figpt 1041:(-0.662809,-0.417969)
\figpt 1042:(-0.610313,-0.252800)
\figpt 1043:(-1.098684,-0.188504)
\figpt 1051:(-0.610313,-0.252800)
\figpt 1052:(-0.764226,-0.173128)
\figpt 1053:(-0.910180,-0.643594)
\figpt 1061:(-0.851148,-0.237367)
\figpt 1062:(-0.764226,-0.173128)
\figpt 1063:(-1.098684,0.188504)
\figpt 1071:(-0.868959,-0.303059)
\figpt 1072:(-0.851148,-0.237367)
\figpt 1073:(-0.979813,-0.237742)
\figpt 1081:(-0.858731,-0.355698)
\figpt 1082:(-0.868959,-0.303059)
\figpt 1083:(-0.942522,-0.344667)
\figpt 1091:(-0.828742,-0.400152)
\figpt 1092:(-0.858731,-0.355698)
\figpt 1093:(-0.910180,-0.422748)
\figpt 1101:(-0.769697,-0.434009)
\figpt 1102:(-0.828742,-0.400152)
\figpt 1103:(-0.860942,-0.524723)
\figpt 1111:(-0.662809,-0.417969)
\figpt 1112:(-0.769697,-0.434009)
\figpt 1113:(-0.643594,-0.910180)
\figpt 1121:(-0.624955,-0.542021)
\figpt 1122:(-0.662809,-0.417969)
\figpt 1123:(-0.871139,-0.549342)
\figpt 1131:(-0.662809,-0.417969)
\figpt 1132:(-0.769697,-0.434009)
\figpt 1133:(-0.643594,-0.910180)
\figpt 1141:(-0.796186,-0.489833)
\figpt 1142:(-0.769697,-0.434009)
\figpt 1143:(-0.937786,-0.388443)
\figpt 1151:(-0.791165,-0.529838)
\figpt 1152:(-0.796186,-0.489833)
\figpt 1153:(-0.858126,-0.517925)
\figpt 1161:(-0.773982,-0.558922)
\figpt 1162:(-0.791165,-0.529838)
\figpt 1163:(-0.824013,-0.568862)
\figpt 1171:(-0.745179,-0.580881)
\figpt 1172:(-0.773982,-0.558922)
\figpt 1173:(-0.792284,-0.612800)
\figpt 1181:(-0.696069,-0.589564)
\figpt 1182:(-0.745179,-0.580881)
\figpt 1183:(-0.737846,-0.682635)
\figpt 1191:(-0.624955,-0.542021)
\figpt 1192:(-0.696069,-0.589564)
\figpt 1193:(-0.000000,-1.553774)
\figpt 1201:(-0.542021,-0.624955)
\figpt 1202:(-0.624955,-0.542021)
\figpt 1203:(-0.721675,-0.721675)
\figpt 1211:(-0.624955,-0.542021)
\figpt 1212:(-0.696069,-0.589564)
\figpt 1213:(0.000000,-1.553774)
\figpt 1221:(-0.701713,-0.637628)
\figpt 1222:(-0.696069,-0.589564)
\figpt 1223:(-0.807083,-0.600890)
\figpt 1231:(-0.688942,-0.668230)
\figpt 1232:(-0.701713,-0.637628)
\figpt 1233:(-0.742070,-0.672437)
\figpt 1241:(-0.668230,-0.688942)
\figpt 1242:(-0.688942,-0.668230)
\figpt 1243:(-0.707785,-0.707785)
\figpt 1251:(-0.637628,-0.701713)
\figpt 1252:(-0.668230,-0.688942)
\figpt 1253:(-0.672437,-0.742070)
\figpt 1261:(-0.589564,-0.696069)
\figpt 1262:(-0.637628,-0.701713)
\figpt 1263:(-0.600890,-0.807083)
\figpt 1271:(-0.589564,-0.696069)
\figpt 1272:(-0.542021,-0.624955)
\figpt 1273:(-1.553774,0.000000)
\figpt 1281:(-0.417969,-0.662809)
\figpt 1282:(-0.542021,-0.624955)
\figpt 1283:(-0.549342,-0.871139)
\figpt 1291:(-0.589564,-0.696069)
\figpt 1292:(-0.542021,-0.624955)
\figpt 1293:(-1.553774,0.000000)
\figpt 1301:(-0.580881,-0.745179)
\figpt 1302:(-0.589564,-0.696069)
\figpt 1303:(-0.682635,-0.737846)
\figpt 1311:(-0.558922,-0.773982)
\figpt 1312:(-0.580881,-0.745179)
\figpt 1313:(-0.612800,-0.792284)
\figpt 1321:(-0.529838,-0.791165)
\figpt 1322:(-0.558922,-0.773982)
\figpt 1323:(-0.568862,-0.824013)
\figpt 1331:(-0.489833,-0.796186)
\figpt 1332:(-0.529838,-0.791165)
\figpt 1333:(-0.517925,-0.858126)
\figpt 1341:(-0.434009,-0.769697)
\figpt 1342:(-0.489833,-0.796186)
\figpt 1343:(-0.388443,-0.937786)
\figpt 1351:(-0.434009,-0.769697)
\figpt 1352:(-0.417969,-0.662809)
\figpt 1353:(-0.910180,-0.643594)
\figpt 1361:(-0.173128,-0.764226)
\figpt 1362:(-0.252800,-0.610313)
\figpt 1363:(-0.643594,-0.910180)
\figpt 1371:(-0.252800,-0.610313)
\figpt 1372:(-0.417969,-0.662809)
\figpt 1373:(-0.188504,-1.098684)
\figpt 1381:(-0.434009,-0.769697)
\figpt 1382:(-0.417969,-0.662809)
\figpt 1383:(-0.910180,-0.643594)
\figpt 1391:(-0.400152,-0.828742)
\figpt 1392:(-0.434009,-0.769697)
\figpt 1393:(-0.524723,-0.860942)
\figpt 1401:(-0.355698,-0.858731)
\figpt 1402:(-0.400152,-0.828742)
\figpt 1403:(-0.422748,-0.910180)
\figpt 1411:(-0.303059,-0.868959)
\figpt 1412:(-0.355698,-0.858731)
\figpt 1413:(-0.344667,-0.942522)
\figpt 1421:(-0.237367,-0.851148)
\figpt 1422:(-0.303059,-0.868959)
\figpt 1423:(-0.237742,-0.979813)
\figpt 1431:(-0.173128,-0.764226)
\figpt 1432:(-0.237367,-0.851148)
\figpt 1433:(0.188504,-1.098684)
\figpt 1441:(-0.058643,-0.825177)
\figpt 1442:(-0.173128,-0.764226)
\figpt 1443:(-0.227545,-1.004432)
\figpt 1451:(-0.173128,-0.764226)
\figpt 1452:(-0.237367,-0.851148)
\figpt 1453:(0.188504,-1.098684)
\figpt 1461:(-0.216625,-0.909353)
\figpt 1462:(-0.237367,-0.851148)
\figpt 1463:(-0.388443,-0.937786)
\figpt 1471:(-0.184787,-0.934090)
\figpt 1472:(-0.216625,-0.909353)
\figpt 1473:(-0.240558,-0.973015)
\figpt 1481:(-0.152070,-0.942506)
\figpt 1482:(-0.184787,-0.934090)
\figpt 1483:(-0.180419,-0.984912)
\figpt 1491:(-0.116176,-0.937666)
\figpt 1492:(-0.152070,-0.942506)
\figpt 1493:(-0.126915,-0.993544)
\figpt 1501:(-0.075311,-0.909079)
\figpt 1502:(-0.116176,-0.937666)
\figpt 1503:(-0.039041,-1.004432)
\figpt 1511:(-0.058643,-0.825177)
\figpt 1512:(-0.075311,-0.909079)
\figpt 1513:(1.098684,-1.098684)
\figpt 1521:(0.058643,-0.825177)
\figpt 1522:(-0.058643,-0.825177)
\figpt 1523:(0.000000,-1.020603)
\figpt 1531:(-0.058643,-0.825177)
\figpt 1532:(-0.075311,-0.909079)
\figpt 1533:(1.098684,-1.098684)
\figpt 1541:(-0.045315,-0.947058)
\figpt 1542:(-0.075311,-0.909079)
\figpt 1543:(-0.145800,-0.995588)
\figpt 1551:(-0.014645,-0.959665)
\figpt 1552:(-0.045315,-0.947058)
\figpt 1553:(-0.049238,-1.000208)
\figpt 1561:(0.014645,-0.959665)
\figpt 1562:(-0.014645,-0.959665)
\figpt 1563:(-0.000000,-1.000959)
\figpt 1571:(0.045315,-0.947058)
\figpt 1572:(0.014645,-0.959665)
\figpt 1573:(0.049238,-1.000208)
\figpt 1581:(0.075311,-0.909079)
\figpt 1582:(0.045315,-0.947058)
\figpt 1583:(0.145800,-0.995588)
\figpt 1591:(0.075311,-0.909079)
\figpt 1592:(0.058643,-0.825177)
\figpt 1593:(-1.098684,-1.098684)
\figpt 1601:(0.173128,-0.764226)
\figpt 1602:(0.058643,-0.825177)
\figpt 1603:(0.227545,-1.004432)
\figpt 1611:(0.075311,-0.909079)
\figpt 1612:(0.058643,-0.825177)
\figpt 1613:(-1.098684,-1.098684)
\figpt 1621:(0.116176,-0.937666)
\figpt 1622:(0.075311,-0.909079)
\figpt 1623:(0.039041,-1.004432)
\figpt 1631:(0.152070,-0.942506)
\figpt 1632:(0.116176,-0.937666)
\figpt 1633:(0.126915,-0.993544)
\figpt 1641:(0.184787,-0.934090)
\figpt 1642:(0.152070,-0.942506)
\figpt 1643:(0.180419,-0.984912)
\figpt 1651:(0.216625,-0.909353)
\figpt 1652:(0.184787,-0.934090)
\figpt 1653:(0.240558,-0.973015)
\figpt 1661:(0.237367,-0.851148)
\figpt 1662:(0.216625,-0.909353)
\figpt 1663:(0.388443,-0.937786)
\figpt 1671:(0.237367,-0.851148)
\figpt 1672:(0.173128,-0.764226)
\figpt 1673:(-0.188504,-1.098684)
\figpt 1681:(0.417969,-0.662809)
\figpt 1682:(0.252800,-0.610313)
\figpt 1683:(0.188504,-1.098684)
\figpt 1691:(0.252800,-0.610313)
\figpt 1692:(0.173128,-0.764226)
\figpt 1693:(0.643594,-0.910180)
\figpt 1701:(0.237367,-0.851148)
\figpt 1702:(0.173128,-0.764226)
\figpt 1703:(-0.188504,-1.098684)
\figpt 1711:(0.303059,-0.868959)
\figpt 1712:(0.237367,-0.851148)
\figpt 1713:(0.237742,-0.979813)
\figpt 1721:(0.355698,-0.858731)
\figpt 1722:(0.303059,-0.868959)
\figpt 1723:(0.344667,-0.942522)
\figpt 1731:(0.400152,-0.828742)
\figpt 1732:(0.355698,-0.858731)
\figpt 1733:(0.422748,-0.910180)
\figpt 1741:(0.434009,-0.769697)
\figpt 1742:(0.400152,-0.828742)
\figpt 1743:(0.524723,-0.860942)
\figpt 1751:(0.417969,-0.662809)
\figpt 1752:(0.434009,-0.769697)
\figpt 1753:(0.910180,-0.643594)
\figpt 1761:(0.542021,-0.624955)
\figpt 1762:(0.417969,-0.662809)
\figpt 1763:(0.549342,-0.871139)
\figpt 1771:(0.417969,-0.662809)
\figpt 1772:(0.434009,-0.769697)
\figpt 1773:(0.910180,-0.643594)
\figpt 1781:(0.489833,-0.796186)
\figpt 1782:(0.434009,-0.769697)
\figpt 1783:(0.388443,-0.937786)
\figpt 1791:(0.529838,-0.791165)
\figpt 1792:(0.489833,-0.796186)
\figpt 1793:(0.517925,-0.858126)
\figpt 1801:(0.558922,-0.773982)
\figpt 1802:(0.529838,-0.791165)
\figpt 1803:(0.568862,-0.824013)
\figpt 1811:(0.580881,-0.745179)
\figpt 1812:(0.558922,-0.773982)
\figpt 1813:(0.612800,-0.792284)
\figpt 1821:(0.589564,-0.696069)
\figpt 1822:(0.580881,-0.745179)
\figpt 1823:(0.682635,-0.737846)
\figpt 1831:(0.542021,-0.624955)
\figpt 1832:(0.589564,-0.696069)
\figpt 1833:(1.553774,-0.000000)
\figpt 1841:(0.624955,-0.542021)
\figpt 1842:(0.542021,-0.624955)
\figpt 1843:(0.721675,-0.721675)
\figpt 1851:(0.542021,-0.624955)
\figpt 1852:(0.589564,-0.696069)
\figpt 1853:(1.553774,0.000000)
\figpt 1861:(0.637628,-0.701713)
\figpt 1862:(0.589564,-0.696069)
\figpt 1863:(0.600890,-0.807083)
\figpt 1871:(0.668230,-0.688942)
\figpt 1872:(0.637628,-0.701713)
\figpt 1873:(0.672437,-0.742070)
\figpt 1881:(0.688942,-0.668230)
\figpt 1882:(0.668230,-0.688942)
\figpt 1883:(0.707785,-0.707785)
\figpt 1891:(0.701713,-0.637628)
\figpt 1892:(0.688942,-0.668230)
\figpt 1893:(0.742070,-0.672437)
\figpt 1901:(0.696069,-0.589564)
\figpt 1902:(0.701713,-0.637628)
\figpt 1903:(0.807083,-0.600890)
\figpt 1911:(0.696069,-0.589564)
\figpt 1912:(0.624955,-0.542021)
\figpt 1913:(0.000000,-1.553774)
\figpt 1921:(0.662809,-0.417969)
\figpt 1922:(0.624955,-0.542021)
\figpt 1923:(0.871139,-0.549342)
\figpt 1931:(0.696069,-0.589564)
\figpt 1932:(0.624955,-0.542021)
\figpt 1933:(-0.000000,-1.553774)
\figpt 1941:(0.745179,-0.580881)
\figpt 1942:(0.696069,-0.589564)
\figpt 1943:(0.737846,-0.682635)
\figpt 1951:(0.773982,-0.558922)
\figpt 1952:(0.745179,-0.580881)
\figpt 1953:(0.792284,-0.612800)
\figpt 1961:(0.791165,-0.529838)
\figpt 1962:(0.773982,-0.558922)
\figpt 1963:(0.824013,-0.568862)
\figpt 1971:(0.796186,-0.489833)
\figpt 1972:(0.791165,-0.529838)
\figpt 1973:(0.858126,-0.517925)
\figpt 1981:(0.769697,-0.434009)
\figpt 1982:(0.796186,-0.489833)
\figpt 1983:(0.937786,-0.388443)
\figpt 1991:(0.769697,-0.434009)
\figpt 1992:(0.662809,-0.417969)
\figpt 1993:(0.643594,-0.910180)
\figpt 2001:(0.764226,-0.173128)
\figpt 2002:(0.610313,-0.252800)
\figpt 2003:(0.910180,-0.643594)
\figpt 2011:(0.610313,-0.252800)
\figpt 2012:(0.662809,-0.417969)
\figpt 2013:(1.098684,-0.188504)
\figpt 2021:(0.769697,-0.434009)
\figpt 2022:(0.662809,-0.417969)
\figpt 2023:(0.643594,-0.910180)
\figpt 2031:(0.828742,-0.400152)
\figpt 2032:(0.769697,-0.434009)
\figpt 2033:(0.860942,-0.524723)
\figpt 2041:(0.858731,-0.355698)
\figpt 2042:(0.828742,-0.400152)
\figpt 2043:(0.910180,-0.422748)
\figpt 2051:(0.868959,-0.303059)
\figpt 2052:(0.858731,-0.355698)
\figpt 2053:(0.942522,-0.344667)
\figpt 2061:(0.851148,-0.237367)
\figpt 2062:(0.868959,-0.303059)
\figpt 2063:(0.979813,-0.237742)
\figpt 2071:(0.764226,-0.173128)
\figpt 2072:(0.851148,-0.237367)
\figpt 2073:(1.098684,0.188504)
\figpt 2081:(0.825177,-0.058643)
\figpt 2082:(0.764226,-0.173128)
\figpt 2083:(1.004432,-0.227545)
\figpt 2091:(0.764226,-0.173128)
\figpt 2092:(0.851148,-0.237367)
\figpt 2093:(1.098684,0.188504)
\figpt 2101:(0.909353,-0.216625)
\figpt 2102:(0.851148,-0.237367)
\figpt 2103:(0.937786,-0.388443)
\figpt 2111:(0.934090,-0.184787)
\figpt 2112:(0.909353,-0.216625)
\figpt 2113:(0.973015,-0.240558)
\figpt 2121:(0.942506,-0.152070)
\figpt 2122:(0.934090,-0.184787)
\figpt 2123:(0.984912,-0.180419)
\figpt 2131:(0.937666,-0.116176)
\figpt 2132:(0.942506,-0.152070)
\figpt 2133:(0.993544,-0.126915)
\figpt 2141:(0.909079,-0.075311)
\figpt 2142:(0.937666,-0.116176)
\figpt 2143:(1.004432,-0.039041)
\figpt 2151:(0.825177,-0.058643)
\figpt 2152:(0.909079,-0.075311)
\figpt 2153:(1.098684,1.098684)
\figpt 2161:(0.825177,0.058643)
\figpt 2162:(0.825177,-0.058643)
\figpt 2163:(1.020603,0.000000)
\figpt 2171:(0.825177,-0.058643)
\figpt 2172:(0.909079,-0.075311)
\figpt 2173:(1.098684,1.098684)
\figpt 2181:(0.947058,-0.045315)
\figpt 2182:(0.909079,-0.075311)
\figpt 2183:(0.995588,-0.145800)
\figpt 2191:(0.959665,-0.014645)
\figpt 2192:(0.947058,-0.045315)
\figpt 2193:(1.000208,-0.049238)
\figpt 2201:(0.959665,0.014645)
\figpt 2202:(0.959665,-0.014645)
\figpt 2203:(1.000959,-0.000000)
\figpt 2211:(0.947058,0.045315)
\figpt 2212:(0.959665,0.014645)
\figpt 2213:(1.000208,0.049238)
\figpt 2221:(0.909079,0.075311)
\figpt 2222:(0.947058,0.045315)
\figpt 2223:(0.995588,0.145800)
\figpt 2231:(0.909079,0.075311)
\figpt 2232:(0.825177,0.058643)
\figpt 2233:(1.098684,-1.098684)
\figpt 2241:(0.764226,0.173128)
\figpt 2242:(0.825177,0.058643)
\figpt 2243:(1.004432,0.227545)
\figpt 2251:(0.909079,0.075311)
\figpt 2252:(0.825177,0.058643)
\figpt 2253:(1.098684,-1.098684)
\figpt 2261:(0.937666,0.116176)
\figpt 2262:(0.909079,0.075311)
\figpt 2263:(1.004432,0.039041)
\figpt 2271:(0.942506,0.152070)
\figpt 2272:(0.937666,0.116176)
\figpt 2273:(0.993544,0.126915)
\figpt 2281:(0.934090,0.184787)
\figpt 2282:(0.942506,0.152070)
\figpt 2283:(0.984912,0.180419)
\figpt 2291:(0.909353,0.216625)
\figpt 2292:(0.934090,0.184787)
\figpt 2293:(0.973015,0.240558)
\figpt 2301:(0.851148,0.237367)
\figpt 2302:(0.909353,0.216625)
\figpt 2303:(0.937786,0.388443)
\figpt 2311:(0.851148,0.237367)
\figpt 2312:(0.764226,0.173128)
\figpt 2313:(1.098684,-0.188504)
\figpt 2321:(0.662809,0.417969)
\figpt 2322:(0.610313,0.252800)
\figpt 2323:(1.098684,0.188504)
\figpt 2331:(0.610313,0.252800)
\figpt 2332:(0.764226,0.173128)
\figpt 2333:(0.910180,0.643594)
\figpt 2341:(0.851148,0.237367)
\figpt 2342:(0.764226,0.173128)
\figpt 2343:(1.098684,-0.188504)
\figpt 2351:(0.868959,0.303059)
\figpt 2352:(0.851148,0.237367)
\figpt 2353:(0.979813,0.237742)
\figpt 2361:(0.858731,0.355698)
\figpt 2362:(0.868959,0.303059)
\figpt 2363:(0.942522,0.344667)
\figpt 2371:(0.828742,0.400152)
\figpt 2372:(0.858731,0.355698)
\figpt 2373:(0.910180,0.422748)
\figpt 2381:(0.769697,0.434009)
\figpt 2382:(0.828742,0.400152)
\figpt 2383:(0.860942,0.524723)
\figpt 2391:(0.662809,0.417969)
\figpt 2392:(0.769697,0.434009)
\figpt 2393:(0.643594,0.910180)
\figpt 2401:(0.624955,0.542021)
\figpt 2402:(0.662809,0.417969)
\figpt 2403:(0.871139,0.549342)
\figpt 2411:(0.662809,0.417969)
\figpt 2412:(0.769697,0.434009)
\figpt 2413:(0.643594,0.910180)
\figpt 2421:(0.796186,0.489833)
\figpt 2422:(0.769697,0.434009)
\figpt 2423:(0.937786,0.388443)
\figpt 2431:(0.791165,0.529838)
\figpt 2432:(0.796186,0.489833)
\figpt 2433:(0.858126,0.517925)
\figpt 2441:(0.773982,0.558922)
\figpt 2442:(0.791165,0.529838)
\figpt 2443:(0.824013,0.568862)
\figpt 2451:(0.745179,0.580881)
\figpt 2452:(0.773982,0.558922)
\figpt 2453:(0.792284,0.612800)
\figpt 2461:(0.696069,0.589564)
\figpt 2462:(0.745179,0.580881)
\figpt 2463:(0.737846,0.682635)
\figpt 2471:(0.624955,0.542021)
\figpt 2472:(0.696069,0.589564)
\figpt 2473:(-0.000000,1.553774)
\figpt 2481:(0.542021,0.624955)
\figpt 2482:(0.624955,0.542021)
\figpt 2483:(0.721675,0.721675)
\figpt 2491:(0.624955,0.542021)
\figpt 2492:(0.696069,0.589564)
\figpt 2493:(-0.000000,1.553774)
\figpt 2501:(0.701713,0.637628)
\figpt 2502:(0.696069,0.589564)
\figpt 2503:(0.807083,0.600890)
\figpt 2511:(0.688942,0.668230)
\figpt 2512:(0.701713,0.637628)
\figpt 2513:(0.742070,0.672437)
\figpt 2521:(0.668230,0.688942)
\figpt 2522:(0.688942,0.668230)
\figpt 2523:(0.707785,0.707785)
\figpt 2531:(0.637628,0.701713)
\figpt 2532:(0.668230,0.688942)
\figpt 2533:(0.672437,0.742070)
\figpt 2541:(0.589564,0.696069)
\figpt 2542:(0.637628,0.701713)
\figpt 2543:(0.600890,0.807083)
\figpt 2551:(0.589564,0.696069)
\figpt 2552:(0.542021,0.624955)
\figpt 2553:(1.553774,0.000000)
\figpt 2561:(0.417969,0.662809)
\figpt 2562:(0.542021,0.624955)
\figpt 2563:(0.549342,0.871139)
\figpt 2571:(0.589564,0.696069)
\figpt 2572:(0.542021,0.624955)
\figpt 2573:(1.553774,-0.000000)
\figpt 2581:(0.580881,0.745179)
\figpt 2582:(0.589564,0.696069)
\figpt 2583:(0.682635,0.737846)
\figpt 2591:(0.558922,0.773982)
\figpt 2592:(0.580881,0.745179)
\figpt 2593:(0.612800,0.792284)
\figpt 2601:(0.529838,0.791165)
\figpt 2602:(0.558922,0.773982)
\figpt 2603:(0.568862,0.824013)
\figpt 2611:(0.489833,0.796186)
\figpt 2612:(0.529838,0.791165)
\figpt 2613:(0.517925,0.858126)
\figpt 2621:(0.434009,0.769697)
\figpt 2622:(0.489833,0.796186)
\figpt 2623:(0.388443,0.937786)
\figpt 2631:(0.434009,0.769697)
\figpt 2632:(0.417969,0.662809)
\figpt 2633:(0.910180,0.643594)
\figpt 2641:(0.173128,0.764226)
\figpt 2642:(0.252800,0.610313)
\figpt 2643:(0.643594,0.910180)
\figpt 2651:(0.252800,0.610313)
\figpt 2652:(0.417969,0.662809)
\figpt 2653:(0.188504,1.098684)
\figpt 2661:(0.434009,0.769697)
\figpt 2662:(0.417969,0.662809)
\figpt 2663:(0.910180,0.643594)
\figpt 2671:(0.400152,0.828742)
\figpt 2672:(0.434009,0.769697)
\figpt 2673:(0.524723,0.860942)
\figpt 2681:(0.355698,0.858731)
\figpt 2682:(0.400152,0.828742)
\figpt 2683:(0.422748,0.910180)
\figpt 2691:(0.303059,0.868959)
\figpt 2692:(0.355698,0.858731)
\figpt 2693:(0.344667,0.942522)
\figpt 2701:(0.237367,0.851148)
\figpt 2702:(0.303059,0.868959)
\figpt 2703:(0.237742,0.979813)
\figpt 2711:(0.173128,0.764226)
\figpt 2712:(0.237367,0.851148)
\figpt 2713:(-0.188504,1.098684)
\figpt 2721:(0.058643,0.825177)
\figpt 2722:(0.173128,0.764226)
\figpt 2723:(0.227545,1.004432)
\figpt 2731:(0.173128,0.764226)
\figpt 2732:(0.237367,0.851148)
\figpt 2733:(-0.188504,1.098684)
\figpt 2741:(0.216625,0.909353)
\figpt 2742:(0.237367,0.851148)
\figpt 2743:(0.388443,0.937786)
\figpt 2751:(0.184787,0.934090)
\figpt 2752:(0.216625,0.909353)
\figpt 2753:(0.240558,0.973015)
\figpt 2761:(0.152070,0.942506)
\figpt 2762:(0.184787,0.934090)
\figpt 2763:(0.180419,0.984912)
\figpt 2771:(0.116176,0.937666)
\figpt 2772:(0.152070,0.942506)
\figpt 2773:(0.126915,0.993544)
\figpt 2781:(0.075311,0.909079)
\figpt 2782:(0.116176,0.937666)
\figpt 2783:(0.039041,1.004432)
\figpt 2791:(0.058643,0.825177)
\figpt 2792:(0.075311,0.909079)
\figpt 2793:(-1.098684,1.098684)
\figpt 2801:(-0.058643,0.825177)
\figpt 2802:(0.058643,0.825177)
\figpt 2803:(-0.000000,1.020603)
\figpt 2811:(0.058643,0.825177)
\figpt 2812:(0.075311,0.909079)
\figpt 2813:(-1.098684,1.098684)
\figpt 2821:(0.045315,0.947058)
\figpt 2822:(0.075311,0.909079)
\figpt 2823:(0.145800,0.995588)
\figpt 2831:(0.014645,0.959665)
\figpt 2832:(0.045315,0.947058)
\figpt 2833:(0.049238,1.000208)
\figpt 2841:(-0.014645,0.959665)
\figpt 2842:(0.014645,0.959665)
\figpt 2843:(-0.000000,1.000959)
\figpt 2851:(-0.045315,0.947058)
\figpt 2852:(-0.014645,0.959665)
\figpt 2853:(-0.049238,1.000208)
\figpt 2861:(-0.075311,0.909079)
\figpt 2862:(-0.045315,0.947058)
\figpt 2863:(-0.145800,0.995588)
\figpt 2871:(-0.075311,0.909079)
\figpt 2872:(-0.058643,0.825177)
\figpt 2873:(1.098684,1.098684)
\figpt 2881:(-0.173128,0.764226)
\figpt 2882:(-0.058643,0.825177)
\figpt 2883:(-0.227545,1.004432)
\figpt 2891:(-0.075311,0.909079)
\figpt 2892:(-0.058643,0.825177)
\figpt 2893:(1.098684,1.098684)
\figpt 2901:(-0.116176,0.937666)
\figpt 2902:(-0.075311,0.909079)
\figpt 2903:(-0.039041,1.004432)
\figpt 2911:(-0.152070,0.942506)
\figpt 2912:(-0.116176,0.937666)
\figpt 2913:(-0.126915,0.993544)
\figpt 2921:(-0.184787,0.934090)
\figpt 2922:(-0.152070,0.942506)
\figpt 2923:(-0.180419,0.984912)
\figpt 2931:(-0.216625,0.909353)
\figpt 2932:(-0.184787,0.934090)
\figpt 2933:(-0.240558,0.973015)
\figpt 2941:(-0.237367,0.851148)
\figpt 2942:(-0.216625,0.909353)
\figpt 2943:(-0.388443,0.937786)
\figpt 2951:(-0.237367,0.851148)
\figpt 2952:(-0.173128,0.764226)
\figpt 2953:(0.188504,1.098684)
\figpt 2961:(-0.417969,0.662809)
\figpt 2962:(-0.252800,0.610313)
\figpt 2963:(-0.188504,1.098684)
\figpt 2971:(-0.252800,0.610313)
\figpt 2972:(-0.173128,0.764226)
\figpt 2973:(-0.643594,0.910180)
\figpt 2981:(-0.237367,0.851148)
\figpt 2982:(-0.173128,0.764226)
\figpt 2983:(0.188504,1.098684)
\figpt 2991:(-0.303059,0.868959)
\figpt 2992:(-0.237367,0.851148)
\figpt 2993:(-0.237742,0.979813)
\figpt 3001:(-0.355698,0.858731)
\figpt 3002:(-0.303059,0.868959)
\figpt 3003:(-0.344667,0.942522)
\figpt 3011:(-0.400152,0.828742)
\figpt 3012:(-0.355698,0.858731)
\figpt 3013:(-0.422748,0.910180)
\figpt 3021:(-0.434009,0.769697)
\figpt 3022:(-0.400152,0.828742)
\figpt 3023:(-0.524723,0.860942)
\figpt 3031:(-0.417969,0.662809)
\figpt 3032:(-0.434009,0.769697)
\figpt 3033:(-0.910180,0.643594)
\figpt 3041:(-0.542021,0.624955)
\figpt 3042:(-0.417969,0.662809)
\figpt 3043:(-0.549342,0.871139)
\figpt 3051:(-0.417969,0.662809)
\figpt 3052:(-0.434009,0.769697)
\figpt 3053:(-0.910180,0.643594)
\figpt 3061:(-0.489833,0.796186)
\figpt 3062:(-0.434009,0.769697)
\figpt 3063:(-0.388443,0.937786)
\figpt 3071:(-0.529838,0.791165)
\figpt 3072:(-0.489833,0.796186)
\figpt 3073:(-0.517925,0.858126)
\figpt 3081:(-0.558922,0.773982)
\figpt 3082:(-0.529838,0.791165)
\figpt 3083:(-0.568862,0.824013)
\figpt 3091:(-0.580881,0.745179)
\figpt 3092:(-0.558922,0.773982)
\figpt 3093:(-0.612800,0.792284)
\figpt 3101:(-0.589564,0.696069)
\figpt 3102:(-0.580881,0.745179)
\figpt 3103:(-0.682635,0.737846)
\figpt 3111:(-0.542021,0.624955)
\figpt 3112:(-0.589564,0.696069)
\figpt 3113:(-1.553774,-0.000000)
\figpt 3121:(-0.624955,0.542021)
\figpt 3122:(-0.542021,0.624955)
\figpt 3123:(-0.721675,0.721675)
\figpt 3131:(-0.542021,0.624955)
\figpt 3132:(-0.589564,0.696069)
\figpt 3133:(-1.553774,0.000000)
\figpt 3141:(-0.637628,0.701713)
\figpt 3142:(-0.589564,0.696069)
\figpt 3143:(-0.600890,0.807083)
\figpt 3151:(-0.668230,0.688942)
\figpt 3152:(-0.637628,0.701713)
\figpt 3153:(-0.672437,0.742070)
\figpt 3161:(-0.688942,0.668230)
\figpt 3162:(-0.668230,0.688942)
\figpt 3163:(-0.707785,0.707785)
\figpt 3171:(-0.701713,0.637628)
\figpt 3172:(-0.688942,0.668230)
\figpt 3173:(-0.742070,0.672437)
\figpt 3181:(-0.696069,0.589564)
\figpt 3182:(-0.701713,0.637628)
\figpt 3183:(-0.807083,0.600890)
\figpt 3191:(-0.696069,0.589564)
\figpt 3192:(-0.624955,0.542021)
\figpt 3193:(0.000000,1.553774)
\figpt 3201:(-0.662809,0.417969)
\figpt 3202:(-0.624955,0.542021)
\figpt 3203:(-0.871139,0.549342)
\figpt 3211:(-0.696069,0.589564)
\figpt 3212:(-0.624955,0.542021)
\figpt 3213:(-0.000000,1.553774)
\figpt 3221:(-0.745179,0.580881)
\figpt 3222:(-0.696069,0.589564)
\figpt 3223:(-0.737846,0.682635)
\figpt 3231:(-0.773982,0.558922)
\figpt 3232:(-0.745179,0.580881)
\figpt 3233:(-0.792284,0.612800)
\figpt 3241:(-0.791165,0.529838)
\figpt 3242:(-0.773982,0.558922)
\figpt 3243:(-0.824013,0.568862)
\figpt 3251:(-0.796186,0.489833)
\figpt 3252:(-0.791165,0.529838)
\figpt 3253:(-0.858126,0.517925)
\figpt 3261:(-0.769697,0.434009)
\figpt 3262:(-0.796186,0.489833)
\figpt 3263:(-0.937786,0.388443)
\figpt 3271:(-0.769697,0.434009)
\figpt 3272:(-0.662809,0.417969)
\figpt 3273:(-0.643594,0.910180)
\figpt 3281:(-0.828742,0.400152)
\figpt 3282:(-0.769697,0.434009)
\figpt 3283:(-0.860942,0.524723)
\figpt 3291:(-0.769697,0.434009)
\figpt 3292:(-0.796186,0.489833)
\figpt 3293:(-0.937786,0.388443)
\figpt 3301:(-0.830602,0.491806)
\figpt 3302:(-0.796186,0.489833)
\figpt 3303:(-0.807083,0.600890)
\figpt 3311:(-0.848901,0.480950)
\figpt 3312:(-0.830602,0.491806)
\figpt 3313:(-0.857336,0.516019)
\figpt 3321:(-0.858980,0.467179)
\figpt 3322:(-0.848901,0.480950)
\figpt 3323:(-0.873143,0.488120)
\figpt 3331:(-0.863639,0.450137)
\figpt 3332:(-0.858980,0.467179)
\figpt 3333:(-0.885561,0.465287)
\figpt 3341:(-0.859661,0.426797)
\figpt 3342:(-0.863639,0.450137)
\figpt 3343:(-0.903235,0.431378)
\figpt 3351:(-0.828742,0.400152)
\figpt 3352:(-0.859661,0.426797)
\figpt 3353:(-1.004432,0.227545)
\figpt 3361:(-0.858731,0.355698)
\figpt 3362:(-0.828742,0.400152)
\figpt 3363:(-0.910180,0.422748)
\figpt 3371:(-0.828742,0.400152)
\figpt 3372:(-0.859661,0.426797)
\figpt 3373:(-1.004432,0.227545)
\figpt 3381:(-0.881316,0.422190)
\figpt 3382:(-0.859661,0.426797)
\figpt 3383:(-0.881337,0.475485)
\figpt 3391:(-0.892151,0.412530)
\figpt 3392:(-0.881316,0.422190)
\figpt 3393:(-0.901335,0.433738)
\figpt 3401:(-0.897711,0.401424)
\figpt 3402:(-0.892151,0.412530)
\figpt 3403:(-0.910180,0.414611)
\figpt 3411:(-0.899040,0.387765)
\figpt 3412:(-0.897711,0.401424)
\figpt 3413:(-0.918265,0.396529)
\figpt 3421:(-0.891806,0.369398)
\figpt 3422:(-0.899040,0.387765)
\figpt 3423:(-0.932264,0.364072)
\figpt 3431:(-0.891806,0.369398)
\figpt 3432:(-0.858731,0.355698)
\figpt 3441:(-0.868959,0.303059)
\figpt 3442:(-0.858731,0.355698)
\figpt 3443:(-0.942522,0.344667)
\figpt 3451:(-0.858731,0.355698)
\figpt 3452:(-0.891806,0.369398)
\figpt 3461:(-0.909909,0.361526)
\figpt 3462:(-0.891806,0.369398)
\figpt 3463:(-0.916648,0.401773)
\figpt 3471:(-0.918627,0.350928)
\figpt 3472:(-0.909909,0.361526)
\figpt 3473:(-0.929700,0.368923)
\figpt 3481:(-0.922549,0.339143)
\figpt 3482:(-0.918627,0.350928)
\figpt 3483:(-0.936768,0.350420)
\figpt 3491:(-0.921718,0.324651)
\figpt 3492:(-0.922549,0.339143)
\figpt 3493:(-0.944039,0.330641)
\figpt 3501:(-0.909663,0.306081)
\figpt 3502:(-0.921718,0.324651)
\figpt 3503:(-0.959418,0.286981)
\figpt 3511:(-0.909663,0.306081)
\figpt 3512:(-0.868959,0.303059)
\figpt 3513:(-0.871139,0.549342)
\figpt 3521:(-0.909353,0.216625)
\figpt 3522:(-0.851148,0.237367)
\figpt 3523:(-0.937786,0.388443)
\figpt 3531:(-0.851148,0.237367)
\figpt 3532:(-0.868959,0.303059)
\figpt 3533:(-0.979813,0.237742)
\figpt 3541:(-0.909663,0.306081)
\figpt 3542:(-0.868959,0.303059)
\figpt 3543:(-0.871139,0.549342)
\figpt 3551:(-0.928980,0.292391)
\figpt 3552:(-0.909663,0.306081)
\figpt 3553:(-0.943714,0.333653)
\figpt 3561:(-0.937736,0.277045)
\figpt 3562:(-0.928980,0.292391)
\figpt 3563:(-0.955194,0.297178)
\figpt 3571:(-0.940347,0.260180)
\figpt 3572:(-0.937736,0.277045)
\figpt 3573:(-0.962558,0.272252)
\figpt 3581:(-0.935084,0.239565)
\figpt 3582:(-0.940347,0.260180)
\figpt 3583:(-0.971109,0.241348)
\figpt 3591:(-0.909353,0.216625)
\figpt 3592:(-0.935084,0.239565)
\figpt 3593:(-0.995588,0.145800)
\figpt 3601:(-0.934090,0.184787)
\figpt 3602:(-0.909353,0.216625)
\figpt 3603:(-0.973015,0.240558)
\figpt 3611:(-0.909353,0.216625)
\figpt 3612:(-0.935084,0.239565)
\figpt 3613:(-0.995588,0.145800)
\figpt 3621:(-0.952952,0.234079)
\figpt 3622:(-0.935084,0.239565)
\figpt 3623:(-0.959418,0.286981)
\figpt 3631:(-0.960570,0.225245)
\figpt 3632:(-0.952952,0.234079)
\figpt 3633:(-0.970572,0.241570)
\figpt 3641:(-0.963594,0.216211)
\figpt 3642:(-0.960570,0.225245)
\figpt 3643:(-0.974486,0.224881)
\figpt 3651:(-0.963235,0.206149)
\figpt 3652:(-0.963594,0.216211)
\figpt 3653:(-0.977674,0.210671)
\figpt 3661:(-0.956906,0.193838)
\figpt 3662:(-0.963235,0.206149)
\figpt 3663:(-0.982418,0.188504)
\figpt 3671:(-0.934090,0.184787)
\figpt 3672:(-0.956906,0.193838)
\figpt 3673:(-1.020603,-0.000000)
\figpt 3681:(-0.942506,0.152070)
\figpt 3682:(-0.934090,0.184787)
\figpt 3683:(-0.984912,0.180419)
\figpt 3691:(-0.934090,0.184787)
\figpt 3692:(-0.956906,0.193838)
\figpt 3693:(-1.020603,0.000000)
\figpt 3701:(-0.968445,0.187429)
\figpt 3702:(-0.956906,0.193838)
\figpt 3703:(-0.976826,0.216110)
\figpt 3711:(-0.973134,0.180030)
\figpt 3712:(-0.968445,0.187429)
\figpt 3713:(-0.981749,0.190675)
\figpt 3721:(-0.974610,0.172565)
\figpt 3722:(-0.973134,0.180030)
\figpt 3723:(-0.984037,0.178307)
\figpt 3731:(-0.973166,0.164138)
\figpt 3732:(-0.974610,0.172565)
\figpt 3733:(-0.986172,0.166247)
\figpt 3741:(-0.965581,0.154134)
\figpt 3742:(-0.973166,0.164138)
\figpt 3743:(-0.990010,0.143490)
\figpt 3751:(-0.965581,0.154134)
\figpt 3752:(-0.942506,0.152070)
\figpt 3753:(-0.910180,0.643594)
\figpt 3761:(-0.937666,0.116176)
\figpt 3762:(-0.942506,0.152070)
\figpt 3763:(-0.993544,0.126915)
\figpt 3771:(-0.965581,0.154134)
\figpt 3772:(-0.942506,0.152070)
\figpt 3773:(-0.910180,0.643594)
\figpt 3781:(-0.975535,0.146105)
\figpt 3782:(-0.965581,0.154134)
\figpt 3783:(-0.985913,0.169156)
\figpt 3791:(-0.979348,0.137927)
\figpt 3792:(-0.975535,0.146105)
\figpt 3793:(-0.989160,0.147479)
\figpt 3801:(-0.979976,0.129649)
\figpt 3802:(-0.979348,0.137927)
\figpt 3803:(-0.990967,0.134646)
\figpt 3811:(-0.977030,0.120218)
\figpt 3812:(-0.979976,0.129649)
\figpt 3813:(-0.992845,0.120452)
\figpt 3821:(-0.965631,0.109861)
\figpt 3822:(-0.977030,0.120218)
\figpt 3823:(-0.996985,0.086805)
\figpt 3831:(-0.965631,0.109861)
\figpt 3832:(-0.937666,0.116176)
\figpt 3833:(-0.979813,0.237742)
\figpt 3841:(-0.947058,0.045315)
\figpt 3842:(-0.909079,0.075311)
\figpt 3843:(-0.995588,0.145800)
\figpt 3851:(-0.909079,0.075311)
\figpt 3852:(-0.937666,0.116176)
\figpt 3853:(-1.004432,0.039041)
\figpt 3861:(-0.965631,0.109861)
\figpt 3862:(-0.937666,0.116176)
\figpt 3863:(-0.979813,0.237742)
\figpt 3871:(-0.976479,0.096959)
\figpt 3872:(-0.965631,0.109861)
\figpt 3873:(-0.992997,0.121858)
\figpt 3881:(-0.980045,0.084590)
\figpt 3882:(-0.976479,0.096959)
\figpt 3883:(-0.995588,0.095770)
\figpt 3891:(-0.979041,0.071893)
\figpt 3892:(-0.980045,0.084590)
\figpt 3893:(-0.997221,0.076844)
\figpt 3901:(-0.971398,0.057481)
\figpt 3902:(-0.979041,0.071893)
\figpt 3903:(-0.999042,0.052054)
\figpt 3911:(-0.947058,0.045315)
\figpt 3912:(-0.971398,0.057481)
\figpt 3913:(-1.004432,-0.039041)
\figpt 3921:(-0.959665,0.014645)
\figpt 3922:(-0.947058,0.045315)
\figpt 3923:(-1.000208,0.049238)
\figpt 3931:(-0.947058,0.045315)
\figpt 3932:(-0.971398,0.057481)
\figpt 3933:(-1.004432,-0.039041)
\figpt 3941:(-0.984027,0.050108)
\figpt 3942:(-0.971398,0.057481)
\figpt 3943:(-0.996985,0.086805)
\figpt 3951:(-0.988448,0.041990)
\figpt 3952:(-0.984027,0.050108)
\figpt 3953:(-0.998715,0.052843)
\figpt 3961:(-0.989340,0.034385)
\figpt 3962:(-0.988448,0.041990)
\figpt 3963:(-0.999285,0.039406)
\figpt 3971:(-0.987376,0.026411)
\figpt 3972:(-0.989340,0.034385)
\figpt 3973:(-0.999696,0.027606)
\figpt 3981:(-0.980093,0.017542)
\figpt 3982:(-0.987376,0.026411)
\figpt 3983:(-1.000208,0.008448)
\figpt 3991:(-0.959665,0.014645)
\figpt 3992:(-0.980093,0.017542)
\figpt 3993:(-1.004432,-0.227545)
\figpt 4001:(-0.959665,-0.014645)
\figpt 4002:(-0.959665,0.014645)
\figpt 4003:(-1.000959,-0.000000)
\figpt 4011:(-0.959665,0.014645)
\figpt 4012:(-0.980093,0.017542)
\figpt 4013:(-1.004432,-0.227545)
\figpt 4021:(-0.988462,0.010243)
\figpt 4022:(-0.980093,0.017542)
\figpt 4023:(-0.999792,0.031683)
\figpt 4031:(-0.991132,0.003278)
\figpt 4032:(-0.988462,0.010243)
\figpt 4033:(-1.000010,0.010676)
\figpt 4041:(-0.991132,-0.003278)
\figpt 4042:(-0.991132,0.003278)
\figpt 4043:(-1.000045,-0.000000)
\figpt 4051:(-0.988462,-0.010243)
\figpt 4052:(-0.991132,-0.003278)
\figpt 4053:(-1.000010,-0.010676)
\figpt 4061:(-0.980093,-0.017542)
\figpt 4062:(-0.988462,-0.010243)
\figpt 4063:(-0.999792,-0.031683)
\figpt 4071:(-0.980093,-0.017542)
\figpt 4072:(-0.959665,-0.014645)
\figpt 4073:(-1.004432,0.227545)
\figpt 4081:(-0.947058,-0.045315)
\figpt 4082:(-0.959665,-0.014645)
\figpt 4083:(-1.000208,-0.049238)
\figpt 4091:(-0.980093,-0.017542)
\figpt 4092:(-0.959665,-0.014645)
\figpt 4093:(-1.004432,0.227545)
\figpt 4101:(-0.987376,-0.026411)
\figpt 4102:(-0.980093,-0.017542)
\figpt 4103:(-1.000208,-0.008448)
\figpt 4111:(-0.989340,-0.034385)
\figpt 4112:(-0.987376,-0.026411)
\figpt 4113:(-0.999696,-0.027606)
\figpt 4121:(-0.988448,-0.041990)
\figpt 4122:(-0.989340,-0.034385)
\figpt 4123:(-0.999285,-0.039406)
\figpt 4131:(-0.984027,-0.050108)
\figpt 4132:(-0.988448,-0.041990)
\figpt 4133:(-0.998715,-0.052843)
\figpt 4141:(-0.971398,-0.057481)
\figpt 4142:(-0.984027,-0.050108)
\figpt 4143:(-0.996985,-0.086805)
\figpt 4151:(-0.971398,-0.057481)
\figpt 4152:(-0.947058,-0.045315)
\figpt 4153:(-1.004432,0.039041)
\figpt 4161:(-0.937666,-0.116176)
\figpt 4162:(-0.909079,-0.075311)
\figpt 4163:(-1.004432,-0.039041)
\figpt 4171:(-0.909079,-0.075311)
\figpt 4172:(-0.947058,-0.045315)
\figpt 4173:(-0.995588,-0.145800)
\figpt 4181:(-0.971398,-0.057481)
\figpt 4182:(-0.947058,-0.045315)
\figpt 4183:(-1.004432,0.039041)
\figpt 4191:(-0.979041,-0.071893)
\figpt 4192:(-0.971398,-0.057481)
\figpt 4193:(-0.999042,-0.052054)
\figpt 4201:(-0.980045,-0.084590)
\figpt 4202:(-0.979041,-0.071893)
\figpt 4203:(-0.997221,-0.076844)
\figpt 4211:(-0.976479,-0.096959)
\figpt 4212:(-0.980045,-0.084590)
\figpt 4213:(-0.995588,-0.095770)
\figpt 4221:(-0.965631,-0.109861)
\figpt 4222:(-0.976479,-0.096959)
\figpt 4223:(-0.992997,-0.121858)
\figpt 4231:(-0.937666,-0.116176)
\figpt 4232:(-0.965631,-0.109861)
\figpt 4233:(-0.979813,-0.237742)
\figpt 4241:(-0.942506,-0.152070)
\figpt 4242:(-0.937666,-0.116176)
\figpt 4243:(-0.993544,-0.126915)
\figpt 4251:(-0.937666,-0.116176)
\figpt 4252:(-0.965631,-0.109861)
\figpt 4253:(-0.979813,-0.237742)
\figpt 4261:(-0.977030,-0.120218)
\figpt 4262:(-0.965631,-0.109861)
\figpt 4263:(-0.996985,-0.086805)
\figpt 4271:(-0.979976,-0.129649)
\figpt 4272:(-0.977030,-0.120218)
\figpt 4273:(-0.992845,-0.120452)
\figpt 4281:(-0.979348,-0.137927)
\figpt 4282:(-0.979976,-0.129649)
\figpt 4283:(-0.990967,-0.134646)
\figpt 4291:(-0.975535,-0.146105)
\figpt 4292:(-0.979348,-0.137927)
\figpt 4293:(-0.989160,-0.147479)
\figpt 4301:(-0.965581,-0.154134)
\figpt 4302:(-0.975535,-0.146105)
\figpt 4303:(-0.985913,-0.169156)
\figpt 4311:(-0.942506,-0.152070)
\figpt 4312:(-0.965581,-0.154134)
\figpt 4313:(-0.910180,-0.643594)
\figpt 4321:(-0.934090,-0.184787)
\figpt 4322:(-0.942506,-0.152070)
\figpt 4323:(-0.984912,-0.180419)
\figpt 4331:(-0.942506,-0.152070)
\figpt 4332:(-0.965581,-0.154134)
\figpt 4333:(-0.910180,-0.643594)
\figpt 4341:(-0.973166,-0.164138)
\figpt 4342:(-0.965581,-0.154134)
\figpt 4343:(-0.990010,-0.143490)
\figpt 4351:(-0.974610,-0.172565)
\figpt 4352:(-0.973166,-0.164138)
\figpt 4353:(-0.986172,-0.166247)
\figpt 4361:(-0.973134,-0.180030)
\figpt 4362:(-0.974610,-0.172565)
\figpt 4363:(-0.984037,-0.178307)
\figpt 4371:(-0.968445,-0.187429)
\figpt 4372:(-0.973134,-0.180030)
\figpt 4373:(-0.981749,-0.190675)
\figpt 4381:(-0.956906,-0.193838)
\figpt 4382:(-0.968445,-0.187429)
\figpt 4383:(-0.976826,-0.216110)
\figpt 4391:(-0.956906,-0.193838)
\figpt 4392:(-0.934090,-0.184787)
\figpt 4393:(-1.020603,-0.000000)
\figpt 4401:(-0.909353,-0.216625)
\figpt 4402:(-0.934090,-0.184787)
\figpt 4403:(-0.973015,-0.240558)
\figpt 4411:(-0.956906,-0.193838)
\figpt 4412:(-0.934090,-0.184787)
\figpt 4413:(-1.020603,0.000000)
\figpt 4421:(-0.963235,-0.206149)
\figpt 4422:(-0.956906,-0.193838)
\figpt 4423:(-0.982418,-0.188504)
\figpt 4431:(-0.963594,-0.216211)
\figpt 4432:(-0.963235,-0.206149)
\figpt 4433:(-0.977674,-0.210671)
\figpt 4441:(-0.960570,-0.225245)
\figpt 4442:(-0.963594,-0.216211)
\figpt 4443:(-0.974486,-0.224881)
\figpt 4451:(-0.952952,-0.234079)
\figpt 4452:(-0.960570,-0.225245)
\figpt 4453:(-0.970572,-0.241570)
\figpt 4461:(-0.935084,-0.239565)
\figpt 4462:(-0.952952,-0.234079)
\figpt 4463:(-0.959418,-0.286981)
\figpt 4471:(-0.935084,-0.239565)
\figpt 4472:(-0.909353,-0.216625)
\figpt 4473:(-0.995588,-0.145800)
\figpt 4481:(-0.868959,-0.303059)
\figpt 4482:(-0.851148,-0.237367)
\figpt 4483:(-0.979813,-0.237742)
\figpt 4491:(-0.851148,-0.237367)
\figpt 4492:(-0.909353,-0.216625)
\figpt 4493:(-0.937786,-0.388443)
\figpt 4501:(-0.935084,-0.239565)
\figpt 4502:(-0.909353,-0.216625)
\figpt 4503:(-0.995588,-0.145800)
\figpt 4511:(-0.940347,-0.260180)
\figpt 4512:(-0.935084,-0.239565)
\figpt 4513:(-0.971109,-0.241348)
\figpt 4521:(-0.937736,-0.277045)
\figpt 4522:(-0.940347,-0.260180)
\figpt 4523:(-0.962558,-0.272252)
\figpt 4531:(-0.928980,-0.292391)
\figpt 4532:(-0.937736,-0.277045)
\figpt 4533:(-0.955194,-0.297178)
\figpt 4541:(-0.909663,-0.306081)
\figpt 4542:(-0.928980,-0.292391)
\figpt 4543:(-0.943714,-0.333653)
\figpt 4551:(-0.868959,-0.303059)
\figpt 4552:(-0.909663,-0.306081)
\figpt 4553:(-0.871139,-0.549342)
\figpt 4561:(-0.858731,-0.355698)
\figpt 4562:(-0.868959,-0.303059)
\figpt 4563:(-0.942522,-0.344667)
\figpt 4571:(-0.868959,-0.303059)
\figpt 4572:(-0.909663,-0.306081)
\figpt 4573:(-0.871139,-0.549342)
\figpt 4581:(-0.921718,-0.324651)
\figpt 4582:(-0.909663,-0.306081)
\figpt 4583:(-0.959418,-0.286981)
\figpt 4591:(-0.922549,-0.339143)
\figpt 4592:(-0.921718,-0.324651)
\figpt 4593:(-0.944039,-0.330641)
\figpt 4601:(-0.918627,-0.350928)
\figpt 4602:(-0.922549,-0.339143)
\figpt 4603:(-0.936768,-0.350420)
\figpt 4611:(-0.909909,-0.361526)
\figpt 4612:(-0.918627,-0.350928)
\figpt 4613:(-0.929700,-0.368923)
\figpt 4621:(-0.891806,-0.369398)
\figpt 4622:(-0.909909,-0.361526)
\figpt 4623:(-0.916648,-0.401773)
\figpt 4631:(-0.858731,-0.355698)
\figpt 4632:(-0.891806,-0.369398)
\figpt 4641:(-0.828742,-0.400152)
\figpt 4642:(-0.858731,-0.355698)
\figpt 4643:(-0.910180,-0.422748)
\figpt 4651:(-0.891806,-0.369398)
\figpt 4652:(-0.858731,-0.355698)
\figpt 4661:(-0.899040,-0.387765)
\figpt 4662:(-0.891806,-0.369398)
\figpt 4663:(-0.932264,-0.364072)
\figpt 4671:(-0.897711,-0.401424)
\figpt 4672:(-0.899040,-0.387765)
\figpt 4673:(-0.918265,-0.396529)
\figpt 4681:(-0.892151,-0.412530)
\figpt 4682:(-0.897711,-0.401424)
\figpt 4683:(-0.910180,-0.414611)
\figpt 4691:(-0.881316,-0.422190)
\figpt 4692:(-0.892151,-0.412530)
\figpt 4693:(-0.901335,-0.433738)
\figpt 4701:(-0.859661,-0.426797)
\figpt 4702:(-0.881316,-0.422190)
\figpt 4703:(-0.881337,-0.475485)
\figpt 4711:(-0.859661,-0.426797)
\figpt 4712:(-0.828742,-0.400152)
\figpt 4713:(-1.004432,-0.227545)
\figpt 4721:(-0.796186,-0.489833)
\figpt 4722:(-0.769697,-0.434009)
\figpt 4723:(-0.937786,-0.388443)
\figpt 4731:(-0.769697,-0.434009)
\figpt 4732:(-0.828742,-0.400152)
\figpt 4733:(-0.860942,-0.524723)
\figpt 4741:(-0.859661,-0.426797)
\figpt 4742:(-0.828742,-0.400152)
\figpt 4743:(-1.004432,-0.227545)
\figpt 4751:(-0.863639,-0.450137)
\figpt 4752:(-0.859661,-0.426797)
\figpt 4753:(-0.903235,-0.431378)
\figpt 4761:(-0.858980,-0.467179)
\figpt 4762:(-0.863639,-0.450137)
\figpt 4763:(-0.885561,-0.465287)
\figpt 4771:(-0.848901,-0.480950)
\figpt 4772:(-0.858980,-0.467179)
\figpt 4773:(-0.873143,-0.488120)
\figpt 4781:(-0.830602,-0.491806)
\figpt 4782:(-0.848901,-0.480950)
\figpt 4783:(-0.857336,-0.516019)
\figpt 4791:(-0.796186,-0.489833)
\figpt 4792:(-0.830602,-0.491806)
\figpt 4793:(-0.807083,-0.600890)
\figpt 4801:(-0.791165,-0.529838)
\figpt 4802:(-0.796186,-0.489833)
\figpt 4803:(-0.858126,-0.517925)
\figpt 4811:(-0.796186,-0.489833)
\figpt 4812:(-0.830602,-0.491806)
\figpt 4813:(-0.807083,-0.600890)
\figpt 4821:(-0.839358,-0.508320)
\figpt 4822:(-0.830602,-0.491806)
\figpt 4823:(-0.881337,-0.475485)
\figpt 4831:(-0.838497,-0.519953)
\figpt 4832:(-0.839358,-0.508320)
\figpt 4833:(-0.857114,-0.515482)
\figpt 4841:(-0.834249,-0.528480)
\figpt 4842:(-0.838497,-0.519953)
\figpt 4843:(-0.848080,-0.530050)
\figpt 4851:(-0.826880,-0.535341)
\figpt 4852:(-0.834249,-0.528480)
\figpt 4853:(-0.840287,-0.542353)
\figpt 4861:(-0.813699,-0.539571)
\figpt 4862:(-0.826880,-0.535341)
\figpt 4863:(-0.827967,-0.561382)
\figpt 4871:(-0.791165,-0.529838)
\figpt 4872:(-0.813699,-0.539571)
\figpt 4873:(-0.721675,-0.721675)
\figpt 4881:(-0.773982,-0.558922)
\figpt 4882:(-0.791165,-0.529838)
\figpt 4883:(-0.824013,-0.568862)
\figpt 4891:(-0.791165,-0.529838)
\figpt 4892:(-0.813699,-0.539571)
\figpt 4893:(-0.721675,-0.721675)
\figpt 4901:(-0.817326,-0.552261)
\figpt 4902:(-0.813699,-0.539571)
\figpt 4903:(-0.843533,-0.537907)
\figpt 4911:(-0.815410,-0.560810)
\figpt 4912:(-0.817326,-0.552261)
\figpt 4913:(-0.829029,-0.559374)
\figpt 4921:(-0.811175,-0.567131)
\figpt 4922:(-0.815410,-0.560810)
\figpt 4923:(-0.821901,-0.569737)
\figpt 4931:(-0.804196,-0.572069)
\figpt 4932:(-0.811175,-0.567131)
\figpt 4933:(-0.814883,-0.579775)
\figpt 4941:(-0.791758,-0.573780)
\figpt 4942:(-0.804196,-0.572069)
\figpt 4943:(-0.801506,-0.598580)
\figpt 4951:(-0.791758,-0.573780)
\figpt 4952:(-0.773982,-0.558922)
\figpt 4953:(-1.098684,-0.188504)
\figpt 4961:(-0.745179,-0.580881)
\figpt 4962:(-0.773982,-0.558922)
\figpt 4963:(-0.792284,-0.612800)
\figpt 4971:(-0.791758,-0.573780)
\figpt 4972:(-0.773982,-0.558922)
\figpt 4973:(-1.098684,-0.188504)
\figpt 4981:(-0.793119,-0.586496)
\figpt 4982:(-0.791758,-0.573780)
\figpt 4983:(-0.816757,-0.577535)
\figpt 4991:(-0.790032,-0.594975)
\figpt 4992:(-0.793119,-0.586496)
\figpt 4993:(-0.803725,-0.595158)
\figpt 5001:(-0.784624,-0.601272)
\figpt 5002:(-0.790032,-0.594975)
\figpt 5003:(-0.795929,-0.605511)
\figpt 5011:(-0.775871,-0.605857)
\figpt 5012:(-0.784624,-0.601272)
\figpt 5013:(-0.787220,-0.616875)
\figpt 5021:(-0.760488,-0.605121)
\figpt 5022:(-0.775871,-0.605857)
\figpt 5023:(-0.766356,-0.643594)
\figpt 5031:(-0.760488,-0.605121)
\figpt 5032:(-0.745179,-0.580881)
\figpt 5033:(-0.860942,-0.524723)
\figpt 5041:(-0.701713,-0.637628)
\figpt 5042:(-0.696069,-0.589564)
\figpt 5043:(-0.807083,-0.600890)
\figpt 5051:(-0.696069,-0.589564)
\figpt 5052:(-0.745179,-0.580881)
\figpt 5053:(-0.737846,-0.682635)
\figpt 5061:(-0.760488,-0.605121)
\figpt 5062:(-0.745179,-0.580881)
\figpt 5063:(-0.860942,-0.524723)
\figpt 5071:(-0.759035,-0.621914)
\figpt 5072:(-0.760488,-0.605121)
\figpt 5073:(-0.788322,-0.615988)
\figpt 5081:(-0.752810,-0.633182)
\figpt 5082:(-0.759035,-0.621914)
\figpt 5083:(-0.771706,-0.636267)
\figpt 5091:(-0.743122,-0.641450)
\figpt 5092:(-0.752810,-0.633182)
\figpt 5093:(-0.759479,-0.650805)
\figpt 5101:(-0.727527,-0.646237)
\figpt 5102:(-0.743122,-0.641450)
\figpt 5103:(-0.743237,-0.669621)
\figpt 5111:(-0.701713,-0.637628)
\figpt 5112:(-0.727527,-0.646237)
\figpt 5113:(-0.682635,-0.737846)
\figpt 5121:(-0.688942,-0.668230)
\figpt 5122:(-0.701713,-0.637628)
\figpt 5123:(-0.742070,-0.672437)
\figpt 5131:(-0.701713,-0.637628)
\figpt 5132:(-0.727527,-0.646237)
\figpt 5133:(-0.682635,-0.737846)
\figpt 5141:(-0.731244,-0.660381)
\figpt 5142:(-0.727527,-0.646237)
\figpt 5143:(-0.766356,-0.643594)
\figpt 5151:(-0.728629,-0.669247)
\figpt 5152:(-0.731244,-0.660381)
\figpt 5153:(-0.743564,-0.668832)
\figpt 5161:(-0.723883,-0.675256)
\figpt 5162:(-0.728629,-0.669247)
\figpt 5163:(-0.734466,-0.678737)
\figpt 5171:(-0.716856,-0.679505)
\figpt 5172:(-0.723883,-0.675256)
\figpt 5173:(-0.726412,-0.687371)
\figpt 5181:(-0.705435,-0.680626)
\figpt 5182:(-0.716856,-0.679505)
\figpt 5183:(-0.713227,-0.701280)
\figpt 5191:(-0.688942,-0.668230)
\figpt 5192:(-0.705435,-0.680626)
\figpt 5193:(-0.549342,-0.871139)
\figpt 5201:(-0.668230,-0.688942)
\figpt 5202:(-0.688942,-0.668230)
\figpt 5203:(-0.707785,-0.707785)
\figpt 5211:(-0.688942,-0.668230)
\figpt 5212:(-0.705435,-0.680626)
\figpt 5213:(-0.549342,-0.871139)
\figpt 5221:(-0.706192,-0.691705)
\figpt 5222:(-0.705435,-0.680626)
\figpt 5223:(-0.729363,-0.684557)
\figpt 5231:(-0.703155,-0.698518)
\figpt 5232:(-0.706192,-0.691705)
\figpt 5233:(-0.714663,-0.699565)
\figpt 5241:(-0.698518,-0.703155)
\figpt 5242:(-0.703155,-0.698518)
\figpt 5243:(-0.707139,-0.707139)
\figpt 5251:(-0.691705,-0.706192)
\figpt 5252:(-0.698518,-0.703155)
\figpt 5253:(-0.699565,-0.714663)
\figpt 5261:(-0.680626,-0.705435)
\figpt 5262:(-0.691705,-0.706192)
\figpt 5263:(-0.684557,-0.729363)
\figpt 5271:(-0.680626,-0.705435)
\figpt 5272:(-0.668230,-0.688942)
\figpt 5273:(-0.871139,-0.549342)
\figpt 5281:(-0.637628,-0.701713)
\figpt 5282:(-0.668230,-0.688942)
\figpt 5283:(-0.672437,-0.742070)
\figpt 5291:(-0.680626,-0.705435)
\figpt 5292:(-0.668230,-0.688942)
\figpt 5293:(-0.871139,-0.549342)
\figpt 5301:(-0.679505,-0.716856)
\figpt 5302:(-0.680626,-0.705435)
\figpt 5303:(-0.701280,-0.713227)
\figpt 5311:(-0.675256,-0.723883)
\figpt 5312:(-0.679505,-0.716856)
\figpt 5313:(-0.687371,-0.726412)
\figpt 5321:(-0.669247,-0.728629)
\figpt 5322:(-0.675256,-0.723883)
\figpt 5323:(-0.678737,-0.734466)
\figpt 5331:(-0.660381,-0.731244)
\figpt 5332:(-0.669247,-0.728629)
\figpt 5333:(-0.668832,-0.743564)
\figpt 5341:(-0.646237,-0.727527)
\figpt 5342:(-0.660381,-0.731244)
\figpt 5343:(-0.643594,-0.766356)
\figpt 5351:(-0.646237,-0.727527)
\figpt 5352:(-0.637628,-0.701713)
\figpt 5353:(-0.737846,-0.682635)
\figpt 5361:(-0.580881,-0.745179)
\figpt 5362:(-0.589564,-0.696069)
\figpt 5363:(-0.682635,-0.737846)
\figpt 5371:(-0.589564,-0.696069)
\figpt 5372:(-0.637628,-0.701713)
\figpt 5373:(-0.600890,-0.807083)
\figpt 5381:(-0.646237,-0.727527)
\figpt 5382:(-0.637628,-0.701713)
\figpt 5383:(-0.737846,-0.682635)
\figpt 5391:(-0.641450,-0.743122)
\figpt 5392:(-0.646237,-0.727527)
\figpt 5393:(-0.669621,-0.743237)
\figpt 5401:(-0.633182,-0.752810)
\figpt 5402:(-0.641450,-0.743122)
\figpt 5403:(-0.650805,-0.759479)
\figpt 5411:(-0.621914,-0.759035)
\figpt 5412:(-0.633182,-0.752810)
\figpt 5413:(-0.636267,-0.771706)
\figpt 5421:(-0.605121,-0.760488)
\figpt 5422:(-0.621914,-0.759035)
\figpt 5423:(-0.615988,-0.788322)
\figpt 5431:(-0.580881,-0.745179)
\figpt 5432:(-0.605121,-0.760488)
\figpt 5433:(-0.524723,-0.860942)
\figpt 5441:(-0.558922,-0.773982)
\figpt 5442:(-0.580881,-0.745179)
\figpt 5443:(-0.612800,-0.792284)
\figpt 5451:(-0.580881,-0.745179)
\figpt 5452:(-0.605121,-0.760488)
\figpt 5453:(-0.524723,-0.860942)
\figpt 5461:(-0.605857,-0.775871)
\figpt 5462:(-0.605121,-0.760488)
\figpt 5463:(-0.643594,-0.766356)
\figpt 5471:(-0.601272,-0.784624)
\figpt 5472:(-0.605857,-0.775871)
\figpt 5473:(-0.616875,-0.787220)
\figpt 5481:(-0.594975,-0.790032)
\figpt 5482:(-0.601272,-0.784624)
\figpt 5483:(-0.605511,-0.795929)
\figpt 5491:(-0.586496,-0.793119)
\figpt 5492:(-0.594975,-0.790032)
\figpt 5493:(-0.595158,-0.803725)
\figpt 5501:(-0.573780,-0.791758)
\figpt 5502:(-0.586496,-0.793119)
\figpt 5503:(-0.577535,-0.816757)
\figpt 5511:(-0.558922,-0.773982)
\figpt 5512:(-0.573780,-0.791758)
\figpt 5513:(-0.188504,-1.098684)
\figpt 5521:(-0.529838,-0.791165)
\figpt 5522:(-0.558922,-0.773982)
\figpt 5523:(-0.568862,-0.824013)
\figpt 5531:(-0.558922,-0.773982)
\figpt 5532:(-0.573780,-0.791758)
\figpt 5533:(-0.188504,-1.098684)
\figpt 5541:(-0.572069,-0.804196)
\figpt 5542:(-0.573780,-0.791758)
\figpt 5543:(-0.598580,-0.801506)
\figpt 5551:(-0.567131,-0.811175)
\figpt 5552:(-0.572069,-0.804196)
\figpt 5553:(-0.579775,-0.814883)
\figpt 5561:(-0.560810,-0.815410)
\figpt 5562:(-0.567131,-0.811175)
\figpt 5563:(-0.569737,-0.821901)
\figpt 5571:(-0.552261,-0.817326)
\figpt 5572:(-0.560810,-0.815410)
\figpt 5573:(-0.559374,-0.829029)
\figpt 5581:(-0.539571,-0.813699)
\figpt 5582:(-0.552261,-0.817326)
\figpt 5583:(-0.537907,-0.843533)
\figpt 5591:(-0.539571,-0.813699)
\figpt 5592:(-0.529838,-0.791165)
\figpt 5593:(-0.721675,-0.721675)
\figpt 5601:(-0.489833,-0.796186)
\figpt 5602:(-0.529838,-0.791165)
\figpt 5603:(-0.517925,-0.858126)
\figpt 5611:(-0.539571,-0.813699)
\figpt 5612:(-0.529838,-0.791165)
\figpt 5613:(-0.721675,-0.721675)
\figpt 5621:(-0.535341,-0.826880)
\figpt 5622:(-0.539571,-0.813699)
\figpt 5623:(-0.561382,-0.827967)
\figpt 5631:(-0.528480,-0.834249)
\figpt 5632:(-0.535341,-0.826880)
\figpt 5633:(-0.542353,-0.840287)
\figpt 5641:(-0.519953,-0.838497)
\figpt 5642:(-0.528480,-0.834249)
\figpt 5643:(-0.530050,-0.848080)
\figpt 5651:(-0.508320,-0.839358)
\figpt 5652:(-0.519953,-0.838497)
\figpt 5653:(-0.515482,-0.857114)
\figpt 5661:(-0.491806,-0.830602)
\figpt 5662:(-0.508320,-0.839358)
\figpt 5663:(-0.475485,-0.881337)
\figpt 5671:(-0.491806,-0.830602)
\figpt 5672:(-0.489833,-0.796186)
\figpt 5673:(-0.600890,-0.807083)
\figpt 5681:(-0.400152,-0.828742)
\figpt 5682:(-0.434009,-0.769697)
\figpt 5683:(-0.524723,-0.860942)
\figpt 5691:(-0.434009,-0.769697)
\figpt 5692:(-0.489833,-0.796186)
\figpt 5693:(-0.388443,-0.937786)
\figpt 5701:(-0.491806,-0.830602)
\figpt 5702:(-0.489833,-0.796186)
\figpt 5703:(-0.600890,-0.807083)
\figpt 5711:(-0.480950,-0.848901)
\figpt 5712:(-0.491806,-0.830602)
\figpt 5713:(-0.516019,-0.857336)
\figpt 5721:(-0.467179,-0.858980)
\figpt 5722:(-0.480950,-0.848901)
\figpt 5723:(-0.488120,-0.873143)
\figpt 5731:(-0.450137,-0.863639)
\figpt 5732:(-0.467179,-0.858980)
\figpt 5733:(-0.465287,-0.885561)
\figpt 5741:(-0.426797,-0.859661)
\figpt 5742:(-0.450137,-0.863639)
\figpt 5743:(-0.431378,-0.903235)
\figpt 5751:(-0.400152,-0.828742)
\figpt 5752:(-0.426797,-0.859661)
\figpt 5753:(-0.227545,-1.004432)
\figpt 5761:(-0.355698,-0.858731)
\figpt 5762:(-0.400152,-0.828742)
\figpt 5763:(-0.422748,-0.910180)
\figpt 5771:(-0.400152,-0.828742)
\figpt 5772:(-0.426797,-0.859661)
\figpt 5773:(-0.227545,-1.004432)
\figpt 5781:(-0.422190,-0.881316)
\figpt 5782:(-0.426797,-0.859661)
\figpt 5783:(-0.475485,-0.881337)
\figpt 5791:(-0.412530,-0.892151)
\figpt 5792:(-0.422190,-0.881316)
\figpt 5793:(-0.433738,-0.901335)
\figpt 5801:(-0.401424,-0.897711)
\figpt 5802:(-0.412530,-0.892151)
\figpt 5803:(-0.414611,-0.910180)
\figpt 5811:(-0.387765,-0.899040)
\figpt 5812:(-0.401424,-0.897711)
\figpt 5813:(-0.396529,-0.918265)
\figpt 5821:(-0.369398,-0.891806)
\figpt 5822:(-0.387765,-0.899040)
\figpt 5823:(-0.364072,-0.932264)
\figpt 5831:(-0.355698,-0.858731)
\figpt 5832:(-0.369398,-0.891806)
\figpt 5841:(-0.303059,-0.868959)
\figpt 5842:(-0.355698,-0.858731)
\figpt 5843:(-0.344667,-0.942522)
\figpt 5851:(-0.369398,-0.891806)
\figpt 5852:(-0.355698,-0.858731)
\figpt 5861:(-0.361526,-0.909909)
\figpt 5862:(-0.369398,-0.891806)
\figpt 5863:(-0.401773,-0.916648)
\figpt 5871:(-0.350928,-0.918627)
\figpt 5872:(-0.361526,-0.909909)
\figpt 5873:(-0.368923,-0.929700)
\figpt 5881:(-0.339143,-0.922549)
\figpt 5882:(-0.350928,-0.918627)
\figpt 5883:(-0.350420,-0.936768)
\figpt 5891:(-0.324651,-0.921718)
\figpt 5892:(-0.339143,-0.922549)
\figpt 5893:(-0.330641,-0.944039)
\figpt 5901:(-0.306081,-0.909663)
\figpt 5902:(-0.324651,-0.921718)
\figpt 5903:(-0.286981,-0.959418)
\figpt 5911:(-0.306081,-0.909663)
\figpt 5912:(-0.303059,-0.868959)
\figpt 5913:(-0.549342,-0.871139)
\figpt 5921:(-0.216625,-0.909353)
\figpt 5922:(-0.237367,-0.851148)
\figpt 5923:(-0.388443,-0.937786)
\figpt 5931:(-0.237367,-0.851148)
\figpt 5932:(-0.303059,-0.868959)
\figpt 5933:(-0.237742,-0.979813)
\figpt 5941:(-0.306081,-0.909663)
\figpt 5942:(-0.303059,-0.868959)
\figpt 5943:(-0.549342,-0.871139)
\figpt 5951:(-0.292391,-0.928980)
\figpt 5952:(-0.306081,-0.909663)
\figpt 5953:(-0.333653,-0.943714)
\figpt 5961:(-0.277045,-0.937736)
\figpt 5962:(-0.292391,-0.928980)
\figpt 5963:(-0.297178,-0.955194)
\figpt 5971:(-0.260180,-0.940347)
\figpt 5972:(-0.277045,-0.937736)
\figpt 5973:(-0.272252,-0.962558)
\figpt 5981:(-0.239565,-0.935084)
\figpt 5982:(-0.260180,-0.940347)
\figpt 5983:(-0.241348,-0.971109)
\figpt 5991:(-0.216625,-0.909353)
\figpt 5992:(-0.239565,-0.935084)
\figpt 5993:(-0.145800,-0.995588)
\figpt 6001:(-0.184787,-0.934090)
\figpt 6002:(-0.216625,-0.909353)
\figpt 6003:(-0.240558,-0.973015)
\figpt 6011:(-0.216625,-0.909353)
\figpt 6012:(-0.239565,-0.935084)
\figpt 6013:(-0.145800,-0.995588)
\figpt 6021:(-0.234079,-0.952952)
\figpt 6022:(-0.239565,-0.935084)
\figpt 6023:(-0.286981,-0.959418)
\figpt 6031:(-0.225245,-0.960570)
\figpt 6032:(-0.234079,-0.952952)
\figpt 6033:(-0.241570,-0.970572)
\figpt 6041:(-0.216211,-0.963594)
\figpt 6042:(-0.225245,-0.960570)
\figpt 6043:(-0.224881,-0.974486)
\figpt 6051:(-0.206149,-0.963235)
\figpt 6052:(-0.216211,-0.963594)
\figpt 6053:(-0.210671,-0.977674)
\figpt 6061:(-0.193838,-0.956906)
\figpt 6062:(-0.206149,-0.963235)
\figpt 6063:(-0.188504,-0.982418)
\figpt 6071:(-0.184787,-0.934090)
\figpt 6072:(-0.193838,-0.956906)
\figpt 6073:(-0.000000,-1.020603)
\figpt 6081:(-0.152070,-0.942506)
\figpt 6082:(-0.184787,-0.934090)
\figpt 6083:(-0.180419,-0.984912)
\figpt 6091:(-0.184787,-0.934090)
\figpt 6092:(-0.193838,-0.956906)
\figpt 6093:(0.000000,-1.020603)
\figpt 6101:(-0.187429,-0.968445)
\figpt 6102:(-0.193838,-0.956906)
\figpt 6103:(-0.216110,-0.976826)
\figpt 6111:(-0.180030,-0.973134)
\figpt 6112:(-0.187429,-0.968445)
\figpt 6113:(-0.190675,-0.981749)
\figpt 6121:(-0.172565,-0.974610)
\figpt 6122:(-0.180030,-0.973134)
\figpt 6123:(-0.178307,-0.984037)
\figpt 6131:(-0.164138,-0.973166)
\figpt 6132:(-0.172565,-0.974610)
\figpt 6133:(-0.166247,-0.986172)
\figpt 6141:(-0.154134,-0.965581)
\figpt 6142:(-0.164138,-0.973166)
\figpt 6143:(-0.143490,-0.990010)
\figpt 6151:(-0.154134,-0.965581)
\figpt 6152:(-0.152070,-0.942506)
\figpt 6153:(-0.643594,-0.910180)
\figpt 6161:(-0.116176,-0.937666)
\figpt 6162:(-0.152070,-0.942506)
\figpt 6163:(-0.126915,-0.993544)
\figpt 6171:(-0.154134,-0.965581)
\figpt 6172:(-0.152070,-0.942506)
\figpt 6173:(-0.643594,-0.910180)
\figpt 6181:(-0.146105,-0.975535)
\figpt 6182:(-0.154134,-0.965581)
\figpt 6183:(-0.169156,-0.985913)
\figpt 6191:(-0.137927,-0.979348)
\figpt 6192:(-0.146105,-0.975535)
\figpt 6193:(-0.147479,-0.989160)
\figpt 6201:(-0.129649,-0.979976)
\figpt 6202:(-0.137927,-0.979348)
\figpt 6203:(-0.134646,-0.990967)
\figpt 6211:(-0.120218,-0.977030)
\figpt 6212:(-0.129649,-0.979976)
\figpt 6213:(-0.120452,-0.992845)
\figpt 6221:(-0.109861,-0.965631)
\figpt 6222:(-0.120218,-0.977030)
\figpt 6223:(-0.086805,-0.996985)
\figpt 6231:(-0.109861,-0.965631)
\figpt 6232:(-0.116176,-0.937666)
\figpt 6233:(-0.237742,-0.979813)
\figpt 6241:(-0.045315,-0.947058)
\figpt 6242:(-0.075311,-0.909079)
\figpt 6243:(-0.145800,-0.995588)
\figpt 6251:(-0.075311,-0.909079)
\figpt 6252:(-0.116176,-0.937666)
\figpt 6253:(-0.039041,-1.004432)
\figpt 6261:(-0.109861,-0.965631)
\figpt 6262:(-0.116176,-0.937666)
\figpt 6263:(-0.237742,-0.979813)
\figpt 6271:(-0.096959,-0.976479)
\figpt 6272:(-0.109861,-0.965631)
\figpt 6273:(-0.121858,-0.992997)
\figpt 6281:(-0.084590,-0.980045)
\figpt 6282:(-0.096959,-0.976479)
\figpt 6283:(-0.095770,-0.995588)
\figpt 6291:(-0.071893,-0.979041)
\figpt 6292:(-0.084590,-0.980045)
\figpt 6293:(-0.076844,-0.997221)
\figpt 6301:(-0.057481,-0.971398)
\figpt 6302:(-0.071893,-0.979041)
\figpt 6303:(-0.052054,-0.999042)
\figpt 6311:(-0.045315,-0.947058)
\figpt 6312:(-0.057481,-0.971398)
\figpt 6313:(0.039041,-1.004432)
\figpt 6321:(-0.014645,-0.959665)
\figpt 6322:(-0.045315,-0.947058)
\figpt 6323:(-0.049238,-1.000208)
\figpt 6331:(-0.045315,-0.947058)
\figpt 6332:(-0.057481,-0.971398)
\figpt 6333:(0.039041,-1.004432)
\figpt 6341:(-0.050108,-0.984027)
\figpt 6342:(-0.057481,-0.971398)
\figpt 6343:(-0.086805,-0.996985)
\figpt 6351:(-0.041990,-0.988448)
\figpt 6352:(-0.050108,-0.984027)
\figpt 6353:(-0.052843,-0.998715)
\figpt 6361:(-0.034385,-0.989340)
\figpt 6362:(-0.041990,-0.988448)
\figpt 6363:(-0.039406,-0.999285)
\figpt 6371:(-0.026411,-0.987376)
\figpt 6372:(-0.034385,-0.989340)
\figpt 6373:(-0.027606,-0.999696)
\figpt 6381:(-0.017542,-0.980093)
\figpt 6382:(-0.026411,-0.987376)
\figpt 6383:(-0.008448,-1.000208)
\figpt 6391:(-0.014645,-0.959665)
\figpt 6392:(-0.017542,-0.980093)
\figpt 6393:(0.227545,-1.004432)
\figpt 6401:(0.014645,-0.959665)
\figpt 6402:(-0.014645,-0.959665)
\figpt 6403:(0.000000,-1.000959)
\figpt 6411:(-0.014645,-0.959665)
\figpt 6412:(-0.017542,-0.980093)
\figpt 6413:(0.227545,-1.004432)
\figpt 6421:(-0.010243,-0.988462)
\figpt 6422:(-0.017542,-0.980093)
\figpt 6423:(-0.031683,-0.999792)
\figpt 6431:(-0.003278,-0.991132)
\figpt 6432:(-0.010243,-0.988462)
\figpt 6433:(-0.010676,-1.000010)
\figpt 6441:(0.003278,-0.991132)
\figpt 6442:(-0.003278,-0.991132)
\figpt 6443:(-0.000000,-1.000045)
\figpt 6451:(0.010243,-0.988462)
\figpt 6452:(0.003278,-0.991132)
\figpt 6453:(0.010676,-1.000010)
\figpt 6461:(0.017542,-0.980093)
\figpt 6462:(0.010243,-0.988462)
\figpt 6463:(0.031683,-0.999792)
\figpt 6471:(0.017542,-0.980093)
\figpt 6472:(0.014645,-0.959665)
\figpt 6473:(-0.227545,-1.004432)
\figpt 6481:(0.045315,-0.947058)
\figpt 6482:(0.014645,-0.959665)
\figpt 6483:(0.049238,-1.000208)
\figpt 6491:(0.017542,-0.980093)
\figpt 6492:(0.014645,-0.959665)
\figpt 6493:(-0.227545,-1.004432)
\figpt 6501:(0.026411,-0.987376)
\figpt 6502:(0.017542,-0.980093)
\figpt 6503:(0.008448,-1.000208)
\figpt 6511:(0.034385,-0.989340)
\figpt 6512:(0.026411,-0.987376)
\figpt 6513:(0.027606,-0.999696)
\figpt 6521:(0.041990,-0.988448)
\figpt 6522:(0.034385,-0.989340)
\figpt 6523:(0.039406,-0.999285)
\figpt 6531:(0.050108,-0.984027)
\figpt 6532:(0.041990,-0.988448)
\figpt 6533:(0.052843,-0.998715)
\figpt 6541:(0.057481,-0.971398)
\figpt 6542:(0.050108,-0.984027)
\figpt 6543:(0.086805,-0.996985)
\figpt 6551:(0.057481,-0.971398)
\figpt 6552:(0.045315,-0.947058)
\figpt 6553:(-0.039041,-1.004432)
\figpt 6561:(0.116176,-0.937666)
\figpt 6562:(0.075311,-0.909079)
\figpt 6563:(0.039041,-1.004432)
\figpt 6571:(0.075311,-0.909079)
\figpt 6572:(0.045315,-0.947058)
\figpt 6573:(0.145800,-0.995588)
\figpt 6581:(0.057481,-0.971398)
\figpt 6582:(0.045315,-0.947058)
\figpt 6583:(-0.039041,-1.004432)
\figpt 6591:(0.071893,-0.979041)
\figpt 6592:(0.057481,-0.971398)
\figpt 6593:(0.052054,-0.999042)
\figpt 6601:(0.084590,-0.980045)
\figpt 6602:(0.071893,-0.979041)
\figpt 6603:(0.076844,-0.997221)
\figpt 6611:(0.096959,-0.976479)
\figpt 6612:(0.084590,-0.980045)
\figpt 6613:(0.095770,-0.995588)
\figpt 6621:(0.109861,-0.965631)
\figpt 6622:(0.096959,-0.976479)
\figpt 6623:(0.121858,-0.992997)
\figpt 6631:(0.116176,-0.937666)
\figpt 6632:(0.109861,-0.965631)
\figpt 6633:(0.237742,-0.979813)
\figpt 6641:(0.152070,-0.942506)
\figpt 6642:(0.116176,-0.937666)
\figpt 6643:(0.126915,-0.993544)
\figpt 6651:(0.116176,-0.937666)
\figpt 6652:(0.109861,-0.965631)
\figpt 6653:(0.237742,-0.979813)
\figpt 6661:(0.120218,-0.977030)
\figpt 6662:(0.109861,-0.965631)
\figpt 6663:(0.086805,-0.996985)
\figpt 6671:(0.129649,-0.979976)
\figpt 6672:(0.120218,-0.977030)
\figpt 6673:(0.120452,-0.992845)
\figpt 6681:(0.137927,-0.979348)
\figpt 6682:(0.129649,-0.979976)
\figpt 6683:(0.134646,-0.990967)
\figpt 6691:(0.146105,-0.975535)
\figpt 6692:(0.137927,-0.979348)
\figpt 6693:(0.147479,-0.989160)
\figpt 6701:(0.154134,-0.965581)
\figpt 6702:(0.146105,-0.975535)
\figpt 6703:(0.169156,-0.985913)
\figpt 6711:(0.152070,-0.942506)
\figpt 6712:(0.154134,-0.965581)
\figpt 6713:(0.643594,-0.910180)
\figpt 6721:(0.184787,-0.934090)
\figpt 6722:(0.152070,-0.942506)
\figpt 6723:(0.180419,-0.984912)
\figpt 6731:(0.152070,-0.942506)
\figpt 6732:(0.154134,-0.965581)
\figpt 6733:(0.643594,-0.910180)
\figpt 6741:(0.164138,-0.973166)
\figpt 6742:(0.154134,-0.965581)
\figpt 6743:(0.143490,-0.990010)
\figpt 6751:(0.172565,-0.974610)
\figpt 6752:(0.164138,-0.973166)
\figpt 6753:(0.166247,-0.986172)
\figpt 6761:(0.180030,-0.973134)
\figpt 6762:(0.172565,-0.974610)
\figpt 6763:(0.178307,-0.984037)
\figpt 6771:(0.187429,-0.968445)
\figpt 6772:(0.180030,-0.973134)
\figpt 6773:(0.190675,-0.981749)
\figpt 6781:(0.193838,-0.956906)
\figpt 6782:(0.187429,-0.968445)
\figpt 6783:(0.216110,-0.976826)
\figpt 6791:(0.193838,-0.956906)
\figpt 6792:(0.184787,-0.934090)
\figpt 6793:(-0.000000,-1.020603)
\figpt 6801:(0.216625,-0.909353)
\figpt 6802:(0.184787,-0.934090)
\figpt 6803:(0.240558,-0.973015)
\figpt 6811:(0.193838,-0.956906)
\figpt 6812:(0.184787,-0.934090)
\figpt 6813:(-0.000000,-1.020603)
\figpt 6821:(0.206149,-0.963235)
\figpt 6822:(0.193838,-0.956906)
\figpt 6823:(0.188504,-0.982418)
\figpt 6831:(0.216211,-0.963594)
\figpt 6832:(0.206149,-0.963235)
\figpt 6833:(0.210671,-0.977674)
\figpt 6841:(0.225245,-0.960570)
\figpt 6842:(0.216211,-0.963594)
\figpt 6843:(0.224881,-0.974486)
\figpt 6851:(0.234079,-0.952952)
\figpt 6852:(0.225245,-0.960570)
\figpt 6853:(0.241570,-0.970572)
\figpt 6861:(0.239565,-0.935084)
\figpt 6862:(0.234079,-0.952952)
\figpt 6863:(0.286981,-0.959418)
\figpt 6871:(0.239565,-0.935084)
\figpt 6872:(0.216625,-0.909353)
\figpt 6873:(0.145800,-0.995588)
\figpt 6881:(0.303059,-0.868959)
\figpt 6882:(0.237367,-0.851148)
\figpt 6883:(0.237742,-0.979813)
\figpt 6891:(0.237367,-0.851148)
\figpt 6892:(0.216625,-0.909353)
\figpt 6893:(0.388443,-0.937786)
\figpt 6901:(0.239565,-0.935084)
\figpt 6902:(0.216625,-0.909353)
\figpt 6903:(0.145800,-0.995588)
\figpt 6911:(0.260180,-0.940347)
\figpt 6912:(0.239565,-0.935084)
\figpt 6913:(0.241348,-0.971109)
\figpt 6921:(0.277045,-0.937736)
\figpt 6922:(0.260180,-0.940347)
\figpt 6923:(0.272252,-0.962558)
\figpt 6931:(0.292391,-0.928980)
\figpt 6932:(0.277045,-0.937736)
\figpt 6933:(0.297178,-0.955194)
\figpt 6941:(0.306081,-0.909663)
\figpt 6942:(0.292391,-0.928980)
\figpt 6943:(0.333653,-0.943714)
\figpt 6951:(0.303059,-0.868959)
\figpt 6952:(0.306081,-0.909663)
\figpt 6953:(0.549342,-0.871139)
\figpt 6961:(0.355698,-0.858731)
\figpt 6962:(0.303059,-0.868959)
\figpt 6963:(0.344667,-0.942522)
\figpt 6971:(0.303059,-0.868959)
\figpt 6972:(0.306081,-0.909663)
\figpt 6973:(0.549342,-0.871139)
\figpt 6981:(0.324651,-0.921718)
\figpt 6982:(0.306081,-0.909663)
\figpt 6983:(0.286981,-0.959418)
\figpt 6991:(0.339143,-0.922549)
\figpt 6992:(0.324651,-0.921718)
\figpt 6993:(0.330641,-0.944039)
\figpt 7001:(0.350928,-0.918627)
\figpt 7002:(0.339143,-0.922549)
\figpt 7003:(0.350420,-0.936768)
\figpt 7011:(0.361526,-0.909909)
\figpt 7012:(0.350928,-0.918627)
\figpt 7013:(0.368923,-0.929700)
\figpt 7021:(0.369398,-0.891806)
\figpt 7022:(0.361526,-0.909909)
\figpt 7023:(0.401773,-0.916648)
\figpt 7031:(0.369398,-0.891806)
\figpt 7032:(0.355698,-0.858731)
\figpt 7041:(0.400152,-0.828742)
\figpt 7042:(0.355698,-0.858731)
\figpt 7043:(0.422748,-0.910180)
\figpt 7051:(0.369398,-0.891806)
\figpt 7052:(0.355698,-0.858731)
\figpt 7061:(0.387765,-0.899040)
\figpt 7062:(0.369398,-0.891806)
\figpt 7063:(0.364072,-0.932264)
\figpt 7071:(0.401424,-0.897711)
\figpt 7072:(0.387765,-0.899040)
\figpt 7073:(0.396529,-0.918265)
\figpt 7081:(0.412530,-0.892151)
\figpt 7082:(0.401424,-0.897711)
\figpt 7083:(0.414611,-0.910180)
\figpt 7091:(0.422190,-0.881316)
\figpt 7092:(0.412530,-0.892151)
\figpt 7093:(0.433738,-0.901335)
\figpt 7101:(0.426797,-0.859661)
\figpt 7102:(0.422190,-0.881316)
\figpt 7103:(0.475485,-0.881337)
\figpt 7111:(0.426797,-0.859661)
\figpt 7112:(0.400152,-0.828742)
\figpt 7113:(0.227545,-1.004432)
\figpt 7121:(0.489833,-0.796186)
\figpt 7122:(0.434009,-0.769697)
\figpt 7123:(0.388443,-0.937786)
\figpt 7131:(0.434009,-0.769697)
\figpt 7132:(0.400152,-0.828742)
\figpt 7133:(0.524723,-0.860942)
\figpt 7141:(0.426797,-0.859661)
\figpt 7142:(0.400152,-0.828742)
\figpt 7143:(0.227545,-1.004432)
\figpt 7151:(0.450137,-0.863639)
\figpt 7152:(0.426797,-0.859661)
\figpt 7153:(0.431378,-0.903235)
\figpt 7161:(0.467179,-0.858980)
\figpt 7162:(0.450137,-0.863639)
\figpt 7163:(0.465287,-0.885561)
\figpt 7171:(0.480950,-0.848901)
\figpt 7172:(0.467179,-0.858980)
\figpt 7173:(0.488120,-0.873143)
\figpt 7181:(0.491806,-0.830602)
\figpt 7182:(0.480950,-0.848901)
\figpt 7183:(0.516019,-0.857336)
\figpt 7191:(0.489833,-0.796186)
\figpt 7192:(0.491806,-0.830602)
\figpt 7193:(0.600890,-0.807083)
\figpt 7201:(0.529838,-0.791165)
\figpt 7202:(0.489833,-0.796186)
\figpt 7203:(0.517925,-0.858126)
\figpt 7211:(0.489833,-0.796186)
\figpt 7212:(0.491806,-0.830602)
\figpt 7213:(0.600890,-0.807083)
\figpt 7221:(0.508320,-0.839358)
\figpt 7222:(0.491806,-0.830602)
\figpt 7223:(0.475485,-0.881337)
\figpt 7231:(0.519953,-0.838497)
\figpt 7232:(0.508320,-0.839358)
\figpt 7233:(0.515482,-0.857114)
\figpt 7241:(0.528480,-0.834249)
\figpt 7242:(0.519953,-0.838497)
\figpt 7243:(0.530050,-0.848080)
\figpt 7251:(0.535341,-0.826880)
\figpt 7252:(0.528480,-0.834249)
\figpt 7253:(0.542353,-0.840287)
\figpt 7261:(0.539571,-0.813699)
\figpt 7262:(0.535341,-0.826880)
\figpt 7263:(0.561382,-0.827967)
\figpt 7271:(0.529838,-0.791165)
\figpt 7272:(0.539571,-0.813699)
\figpt 7273:(0.721675,-0.721675)
\figpt 7281:(0.558922,-0.773982)
\figpt 7282:(0.529838,-0.791165)
\figpt 7283:(0.568862,-0.824013)
\figpt 7291:(0.529838,-0.791165)
\figpt 7292:(0.539571,-0.813699)
\figpt 7293:(0.721675,-0.721675)
\figpt 7301:(0.552261,-0.817326)
\figpt 7302:(0.539571,-0.813699)
\figpt 7303:(0.537907,-0.843533)
\figpt 7311:(0.560810,-0.815410)
\figpt 7312:(0.552261,-0.817326)
\figpt 7313:(0.559374,-0.829029)
\figpt 7321:(0.567131,-0.811175)
\figpt 7322:(0.560810,-0.815410)
\figpt 7323:(0.569737,-0.821901)
\figpt 7331:(0.572069,-0.804196)
\figpt 7332:(0.567131,-0.811175)
\figpt 7333:(0.579775,-0.814883)
\figpt 7341:(0.573780,-0.791758)
\figpt 7342:(0.572069,-0.804196)
\figpt 7343:(0.598580,-0.801506)
\figpt 7351:(0.573780,-0.791758)
\figpt 7352:(0.558922,-0.773982)
\figpt 7353:(0.188504,-1.098684)
\figpt 7361:(0.580881,-0.745179)
\figpt 7362:(0.558922,-0.773982)
\figpt 7363:(0.612800,-0.792284)
\figpt 7371:(0.573780,-0.791758)
\figpt 7372:(0.558922,-0.773982)
\figpt 7373:(0.188504,-1.098684)
\figpt 7381:(0.586496,-0.793119)
\figpt 7382:(0.573780,-0.791758)
\figpt 7383:(0.577535,-0.816757)
\figpt 7391:(0.594975,-0.790032)
\figpt 7392:(0.586496,-0.793119)
\figpt 7393:(0.595158,-0.803725)
\figpt 7401:(0.601272,-0.784624)
\figpt 7402:(0.594975,-0.790032)
\figpt 7403:(0.605511,-0.795929)
\figpt 7411:(0.605857,-0.775871)
\figpt 7412:(0.601272,-0.784624)
\figpt 7413:(0.616875,-0.787220)
\figpt 7421:(0.605121,-0.760488)
\figpt 7422:(0.605857,-0.775871)
\figpt 7423:(0.643594,-0.766356)
\figpt 7431:(0.605121,-0.760488)
\figpt 7432:(0.580881,-0.745179)
\figpt 7433:(0.524723,-0.860942)
\figpt 7441:(0.637628,-0.701713)
\figpt 7442:(0.589564,-0.696069)
\figpt 7443:(0.600890,-0.807083)
\figpt 7451:(0.589564,-0.696069)
\figpt 7452:(0.580881,-0.745179)
\figpt 7453:(0.682635,-0.737846)
\figpt 7461:(0.605121,-0.760488)
\figpt 7462:(0.580881,-0.745179)
\figpt 7463:(0.524723,-0.860942)
\figpt 7471:(0.621914,-0.759035)
\figpt 7472:(0.605121,-0.760488)
\figpt 7473:(0.615988,-0.788322)
\figpt 7481:(0.633182,-0.752810)
\figpt 7482:(0.621914,-0.759035)
\figpt 7483:(0.636267,-0.771706)
\figpt 7491:(0.641450,-0.743122)
\figpt 7492:(0.633182,-0.752810)
\figpt 7493:(0.650805,-0.759479)
\figpt 7501:(0.646237,-0.727527)
\figpt 7502:(0.641450,-0.743122)
\figpt 7503:(0.669621,-0.743237)
\figpt 7511:(0.637628,-0.701713)
\figpt 7512:(0.646237,-0.727527)
\figpt 7513:(0.737846,-0.682635)
\figpt 7521:(0.668230,-0.688942)
\figpt 7522:(0.637628,-0.701713)
\figpt 7523:(0.672437,-0.742070)
\figpt 7531:(0.637628,-0.701713)
\figpt 7532:(0.646237,-0.727527)
\figpt 7533:(0.737846,-0.682635)
\figpt 7541:(0.660381,-0.731244)
\figpt 7542:(0.646237,-0.727527)
\figpt 7543:(0.643594,-0.766356)
\figpt 7551:(0.669247,-0.728629)
\figpt 7552:(0.660381,-0.731244)
\figpt 7553:(0.668832,-0.743564)
\figpt 7561:(0.675256,-0.723883)
\figpt 7562:(0.669247,-0.728629)
\figpt 7563:(0.678737,-0.734466)
\figpt 7571:(0.679505,-0.716856)
\figpt 7572:(0.675256,-0.723883)
\figpt 7573:(0.687371,-0.726412)
\figpt 7581:(0.680626,-0.705435)
\figpt 7582:(0.679505,-0.716856)
\figpt 7583:(0.701280,-0.713227)
\figpt 7591:(0.668230,-0.688942)
\figpt 7592:(0.680626,-0.705435)
\figpt 7593:(0.871139,-0.549342)
\figpt 7601:(0.688942,-0.668230)
\figpt 7602:(0.668230,-0.688942)
\figpt 7603:(0.707785,-0.707785)
\figpt 7611:(0.668230,-0.688942)
\figpt 7612:(0.680626,-0.705435)
\figpt 7613:(0.871139,-0.549342)
\figpt 7621:(0.691705,-0.706192)
\figpt 7622:(0.680626,-0.705435)
\figpt 7623:(0.684557,-0.729363)
\figpt 7631:(0.698518,-0.703155)
\figpt 7632:(0.691705,-0.706192)
\figpt 7633:(0.699565,-0.714663)
\figpt 7641:(0.703155,-0.698518)
\figpt 7642:(0.698518,-0.703155)
\figpt 7643:(0.707139,-0.707139)
\figpt 7651:(0.706192,-0.691705)
\figpt 7652:(0.703155,-0.698518)
\figpt 7653:(0.714663,-0.699565)
\figpt 7661:(0.705435,-0.680626)
\figpt 7662:(0.706192,-0.691705)
\figpt 7663:(0.729363,-0.684557)
\figpt 7671:(0.705435,-0.680626)
\figpt 7672:(0.688942,-0.668230)
\figpt 7673:(0.549342,-0.871139)
\figpt 7681:(0.701713,-0.637628)
\figpt 7682:(0.688942,-0.668230)
\figpt 7683:(0.742070,-0.672437)
\figpt 7691:(0.705435,-0.680626)
\figpt 7692:(0.688942,-0.668230)
\figpt 7693:(0.549342,-0.871139)
\figpt 7701:(0.716856,-0.679505)
\figpt 7702:(0.705435,-0.680626)
\figpt 7703:(0.713227,-0.701280)
\figpt 7711:(0.723883,-0.675256)
\figpt 7712:(0.716856,-0.679505)
\figpt 7713:(0.726412,-0.687371)
\figpt 7721:(0.728629,-0.669247)
\figpt 7722:(0.723883,-0.675256)
\figpt 7723:(0.734466,-0.678737)
\figpt 7731:(0.731244,-0.660381)
\figpt 7732:(0.728629,-0.669247)
\figpt 7733:(0.743564,-0.668832)
\figpt 7741:(0.727527,-0.646237)
\figpt 7742:(0.731244,-0.660381)
\figpt 7743:(0.766356,-0.643594)
\figpt 7751:(0.727527,-0.646237)
\figpt 7752:(0.701713,-0.637628)
\figpt 7753:(0.682635,-0.737846)
\figpt 7761:(0.745179,-0.580881)
\figpt 7762:(0.696069,-0.589564)
\figpt 7763:(0.737846,-0.682635)
\figpt 7771:(0.696069,-0.589564)
\figpt 7772:(0.701713,-0.637628)
\figpt 7773:(0.807083,-0.600890)
\figpt 7781:(0.727527,-0.646237)
\figpt 7782:(0.701713,-0.637628)
\figpt 7783:(0.682635,-0.737846)
\figpt 7791:(0.743122,-0.641450)
\figpt 7792:(0.727527,-0.646237)
\figpt 7793:(0.743237,-0.669621)
\figpt 7801:(0.752810,-0.633182)
\figpt 7802:(0.743122,-0.641450)
\figpt 7803:(0.759479,-0.650805)
\figpt 7811:(0.759035,-0.621914)
\figpt 7812:(0.752810,-0.633182)
\figpt 7813:(0.771706,-0.636267)
\figpt 7821:(0.760488,-0.605121)
\figpt 7822:(0.759035,-0.621914)
\figpt 7823:(0.788322,-0.615988)
\figpt 7831:(0.745179,-0.580881)
\figpt 7832:(0.760488,-0.605121)
\figpt 7833:(0.860942,-0.524723)
\figpt 7841:(0.773982,-0.558922)
\figpt 7842:(0.745179,-0.580881)
\figpt 7843:(0.792284,-0.612800)
\figpt 7851:(0.745179,-0.580881)
\figpt 7852:(0.760488,-0.605121)
\figpt 7853:(0.860942,-0.524723)
\figpt 7861:(0.775871,-0.605857)
\figpt 7862:(0.760488,-0.605121)
\figpt 7863:(0.766356,-0.643594)
\figpt 7871:(0.784624,-0.601272)
\figpt 7872:(0.775871,-0.605857)
\figpt 7873:(0.787220,-0.616875)
\figpt 7881:(0.790032,-0.594975)
\figpt 7882:(0.784624,-0.601272)
\figpt 7883:(0.795929,-0.605511)
\figpt 7891:(0.793119,-0.586496)
\figpt 7892:(0.790032,-0.594975)
\figpt 7893:(0.803725,-0.595158)
\figpt 7901:(0.791758,-0.573780)
\figpt 7902:(0.793119,-0.586496)
\figpt 7903:(0.816757,-0.577535)
\figpt 7911:(0.773982,-0.558922)
\figpt 7912:(0.791758,-0.573780)
\figpt 7913:(1.098684,-0.188504)
\figpt 7921:(0.791165,-0.529838)
\figpt 7922:(0.773982,-0.558922)
\figpt 7923:(0.824013,-0.568862)
\figpt 7931:(0.773982,-0.558922)
\figpt 7932:(0.791758,-0.573780)
\figpt 7933:(1.098684,-0.188504)
\figpt 7941:(0.804196,-0.572069)
\figpt 7942:(0.791758,-0.573780)
\figpt 7943:(0.801506,-0.598580)
\figpt 7951:(0.811175,-0.567131)
\figpt 7952:(0.804196,-0.572069)
\figpt 7953:(0.814883,-0.579775)
\figpt 7961:(0.815410,-0.560810)
\figpt 7962:(0.811175,-0.567131)
\figpt 7963:(0.821901,-0.569737)
\figpt 7971:(0.817326,-0.552261)
\figpt 7972:(0.815410,-0.560810)
\figpt 7973:(0.829029,-0.559374)
\figpt 7981:(0.813699,-0.539571)
\figpt 7982:(0.817326,-0.552261)
\figpt 7983:(0.843533,-0.537907)
\figpt 7991:(0.813699,-0.539571)
\figpt 7992:(0.791165,-0.529838)
\figpt 7993:(0.721675,-0.721675)
\figpt 8001:(0.796186,-0.489833)
\figpt 8002:(0.791165,-0.529838)
\figpt 8003:(0.858126,-0.517925)
\figpt 8011:(0.813699,-0.539571)
\figpt 8012:(0.791165,-0.529838)
\figpt 8013:(0.721675,-0.721675)
\figpt 8021:(0.826880,-0.535341)
\figpt 8022:(0.813699,-0.539571)
\figpt 8023:(0.827967,-0.561382)
\figpt 8031:(0.834249,-0.528480)
\figpt 8032:(0.826880,-0.535341)
\figpt 8033:(0.840287,-0.542353)
\figpt 8041:(0.838497,-0.519953)
\figpt 8042:(0.834249,-0.528480)
\figpt 8043:(0.848080,-0.530050)
\figpt 8051:(0.839358,-0.508320)
\figpt 8052:(0.838497,-0.519953)
\figpt 8053:(0.857114,-0.515482)
\figpt 8061:(0.830602,-0.491806)
\figpt 8062:(0.839358,-0.508320)
\figpt 8063:(0.881337,-0.475485)
\figpt 8071:(0.830602,-0.491806)
\figpt 8072:(0.796186,-0.489833)
\figpt 8073:(0.807083,-0.600890)
\figpt 8081:(0.828742,-0.400152)
\figpt 8082:(0.769697,-0.434009)
\figpt 8083:(0.860942,-0.524723)
\figpt 8091:(0.769697,-0.434009)
\figpt 8092:(0.796186,-0.489833)
\figpt 8093:(0.937786,-0.388443)
\figpt 8101:(0.830602,-0.491806)
\figpt 8102:(0.796186,-0.489833)
\figpt 8103:(0.807083,-0.600890)
\figpt 8111:(0.848901,-0.480950)
\figpt 8112:(0.830602,-0.491806)
\figpt 8113:(0.857336,-0.516019)
\figpt 8121:(0.858980,-0.467179)
\figpt 8122:(0.848901,-0.480950)
\figpt 8123:(0.873143,-0.488120)
\figpt 8131:(0.863639,-0.450137)
\figpt 8132:(0.858980,-0.467179)
\figpt 8133:(0.885561,-0.465287)
\figpt 8141:(0.859661,-0.426797)
\figpt 8142:(0.863639,-0.450137)
\figpt 8143:(0.903235,-0.431378)
\figpt 8151:(0.828742,-0.400152)
\figpt 8152:(0.859661,-0.426797)
\figpt 8153:(1.004432,-0.227545)
\figpt 8161:(0.858731,-0.355698)
\figpt 8162:(0.828742,-0.400152)
\figpt 8163:(0.910180,-0.422748)
\figpt 8171:(0.828742,-0.400152)
\figpt 8172:(0.859661,-0.426797)
\figpt 8173:(1.004432,-0.227545)
\figpt 8181:(0.881316,-0.422190)
\figpt 8182:(0.859661,-0.426797)
\figpt 8183:(0.881337,-0.475485)
\figpt 8191:(0.892151,-0.412530)
\figpt 8192:(0.881316,-0.422190)
\figpt 8193:(0.901335,-0.433738)
\figpt 8201:(0.897711,-0.401424)
\figpt 8202:(0.892151,-0.412530)
\figpt 8203:(0.910180,-0.414611)
\figpt 8211:(0.899040,-0.387765)
\figpt 8212:(0.897711,-0.401424)
\figpt 8213:(0.918265,-0.396529)
\figpt 8221:(0.891806,-0.369398)
\figpt 8222:(0.899040,-0.387765)
\figpt 8223:(0.932264,-0.364072)
\figpt 8231:(0.891806,-0.369398)
\figpt 8232:(0.858731,-0.355698)
\figpt 8241:(0.868959,-0.303059)
\figpt 8242:(0.858731,-0.355698)
\figpt 8243:(0.942522,-0.344667)
\figpt 8251:(0.858731,-0.355698)
\figpt 8252:(0.891806,-0.369398)
\figpt 8261:(0.909909,-0.361526)
\figpt 8262:(0.891806,-0.369398)
\figpt 8263:(0.916648,-0.401773)
\figpt 8271:(0.918627,-0.350928)
\figpt 8272:(0.909909,-0.361526)
\figpt 8273:(0.929700,-0.368923)
\figpt 8281:(0.922549,-0.339143)
\figpt 8282:(0.918627,-0.350928)
\figpt 8283:(0.936768,-0.350420)
\figpt 8291:(0.921718,-0.324651)
\figpt 8292:(0.922549,-0.339143)
\figpt 8293:(0.944039,-0.330641)
\figpt 8301:(0.909663,-0.306081)
\figpt 8302:(0.921718,-0.324651)
\figpt 8303:(0.959418,-0.286981)
\figpt 8311:(0.909663,-0.306081)
\figpt 8312:(0.868959,-0.303059)
\figpt 8313:(0.871139,-0.549342)
\figpt 8321:(0.909353,-0.216625)
\figpt 8322:(0.851148,-0.237367)
\figpt 8323:(0.937786,-0.388443)
\figpt 8331:(0.851148,-0.237367)
\figpt 8332:(0.868959,-0.303059)
\figpt 8333:(0.979813,-0.237742)
\figpt 8341:(0.909663,-0.306081)
\figpt 8342:(0.868959,-0.303059)
\figpt 8343:(0.871139,-0.549342)
\figpt 8351:(0.928980,-0.292391)
\figpt 8352:(0.909663,-0.306081)
\figpt 8353:(0.943714,-0.333653)
\figpt 8361:(0.937736,-0.277045)
\figpt 8362:(0.928980,-0.292391)
\figpt 8363:(0.955194,-0.297178)
\figpt 8371:(0.940347,-0.260180)
\figpt 8372:(0.937736,-0.277045)
\figpt 8373:(0.962558,-0.272252)
\figpt 8381:(0.935084,-0.239565)
\figpt 8382:(0.940347,-0.260180)
\figpt 8383:(0.971109,-0.241348)
\figpt 8391:(0.909353,-0.216625)
\figpt 8392:(0.935084,-0.239565)
\figpt 8393:(0.995588,-0.145800)
\figpt 8401:(0.934090,-0.184787)
\figpt 8402:(0.909353,-0.216625)
\figpt 8403:(0.973015,-0.240558)
\figpt 8411:(0.909353,-0.216625)
\figpt 8412:(0.935084,-0.239565)
\figpt 8413:(0.995588,-0.145800)
\figpt 8421:(0.952952,-0.234079)
\figpt 8422:(0.935084,-0.239565)
\figpt 8423:(0.959418,-0.286981)
\figpt 8431:(0.960570,-0.225245)
\figpt 8432:(0.952952,-0.234079)
\figpt 8433:(0.970572,-0.241570)
\figpt 8441:(0.963594,-0.216211)
\figpt 8442:(0.960570,-0.225245)
\figpt 8443:(0.974486,-0.224881)
\figpt 8451:(0.963235,-0.206149)
\figpt 8452:(0.963594,-0.216211)
\figpt 8453:(0.977674,-0.210671)
\figpt 8461:(0.956906,-0.193838)
\figpt 8462:(0.963235,-0.206149)
\figpt 8463:(0.982418,-0.188504)
\figpt 8471:(0.934090,-0.184787)
\figpt 8472:(0.956906,-0.193838)
\figpt 8473:(1.020603,-0.000000)
\figpt 8481:(0.942506,-0.152070)
\figpt 8482:(0.934090,-0.184787)
\figpt 8483:(0.984912,-0.180419)
\figpt 8491:(0.934090,-0.184787)
\figpt 8492:(0.956906,-0.193838)
\figpt 8493:(1.020603,-0.000000)
\figpt 8501:(0.968445,-0.187429)
\figpt 8502:(0.956906,-0.193838)
\figpt 8503:(0.976826,-0.216110)
\figpt 8511:(0.973134,-0.180030)
\figpt 8512:(0.968445,-0.187429)
\figpt 8513:(0.981749,-0.190675)
\figpt 8521:(0.974610,-0.172565)
\figpt 8522:(0.973134,-0.180030)
\figpt 8523:(0.984037,-0.178307)
\figpt 8531:(0.973166,-0.164138)
\figpt 8532:(0.974610,-0.172565)
\figpt 8533:(0.986172,-0.166247)
\figpt 8541:(0.965581,-0.154134)
\figpt 8542:(0.973166,-0.164138)
\figpt 8543:(0.990010,-0.143490)
\figpt 8551:(0.965581,-0.154134)
\figpt 8552:(0.942506,-0.152070)
\figpt 8553:(0.910180,-0.643594)
\figpt 8561:(0.937666,-0.116176)
\figpt 8562:(0.942506,-0.152070)
\figpt 8563:(0.993544,-0.126915)
\figpt 8571:(0.965581,-0.154134)
\figpt 8572:(0.942506,-0.152070)
\figpt 8573:(0.910180,-0.643594)
\figpt 8581:(0.975535,-0.146105)
\figpt 8582:(0.965581,-0.154134)
\figpt 8583:(0.985913,-0.169156)
\figpt 8591:(0.979348,-0.137927)
\figpt 8592:(0.975535,-0.146105)
\figpt 8593:(0.989160,-0.147479)
\figpt 8601:(0.979976,-0.129649)
\figpt 8602:(0.979348,-0.137927)
\figpt 8603:(0.990967,-0.134646)
\figpt 8611:(0.977030,-0.120218)
\figpt 8612:(0.979976,-0.129649)
\figpt 8613:(0.992845,-0.120452)
\figpt 8621:(0.965631,-0.109861)
\figpt 8622:(0.977030,-0.120218)
\figpt 8623:(0.996985,-0.086805)
\figpt 8631:(0.965631,-0.109861)
\figpt 8632:(0.937666,-0.116176)
\figpt 8633:(0.979813,-0.237742)
\figpt 8641:(0.947058,-0.045315)
\figpt 8642:(0.909079,-0.075311)
\figpt 8643:(0.995588,-0.145800)
\figpt 8651:(0.909079,-0.075311)
\figpt 8652:(0.937666,-0.116176)
\figpt 8653:(1.004432,-0.039041)
\figpt 8661:(0.965631,-0.109861)
\figpt 8662:(0.937666,-0.116176)
\figpt 8663:(0.979813,-0.237742)
\figpt 8671:(0.976479,-0.096959)
\figpt 8672:(0.965631,-0.109861)
\figpt 8673:(0.992997,-0.121858)
\figpt 8681:(0.980045,-0.084590)
\figpt 8682:(0.976479,-0.096959)
\figpt 8683:(0.995588,-0.095770)
\figpt 8691:(0.979041,-0.071893)
\figpt 8692:(0.980045,-0.084590)
\figpt 8693:(0.997221,-0.076844)
\figpt 8701:(0.971398,-0.057481)
\figpt 8702:(0.979041,-0.071893)
\figpt 8703:(0.999042,-0.052054)
\figpt 8711:(0.947058,-0.045315)
\figpt 8712:(0.971398,-0.057481)
\figpt 8713:(1.004432,0.039041)
\figpt 8721:(0.959665,-0.014645)
\figpt 8722:(0.947058,-0.045315)
\figpt 8723:(1.000208,-0.049238)
\figpt 8731:(0.947058,-0.045315)
\figpt 8732:(0.971398,-0.057481)
\figpt 8733:(1.004432,0.039041)
\figpt 8741:(0.984027,-0.050108)
\figpt 8742:(0.971398,-0.057481)
\figpt 8743:(0.996985,-0.086805)
\figpt 8751:(0.988448,-0.041990)
\figpt 8752:(0.984027,-0.050108)
\figpt 8753:(0.998715,-0.052843)
\figpt 8761:(0.989340,-0.034385)
\figpt 8762:(0.988448,-0.041990)
\figpt 8763:(0.999285,-0.039406)
\figpt 8771:(0.987376,-0.026411)
\figpt 8772:(0.989340,-0.034385)
\figpt 8773:(0.999696,-0.027606)
\figpt 8781:(0.980093,-0.017542)
\figpt 8782:(0.987376,-0.026411)
\figpt 8783:(1.000208,-0.008448)
\figpt 8791:(0.959665,-0.014645)
\figpt 8792:(0.980093,-0.017542)
\figpt 8793:(1.004432,0.227545)
\figpt 8801:(0.959665,0.014645)
\figpt 8802:(0.959665,-0.014645)
\figpt 8803:(1.000959,0.000000)
\figpt 8811:(0.959665,-0.014645)
\figpt 8812:(0.980093,-0.017542)
\figpt 8813:(1.004432,0.227545)
\figpt 8821:(0.988462,-0.010243)
\figpt 8822:(0.980093,-0.017542)
\figpt 8823:(0.999792,-0.031683)
\figpt 8831:(0.991132,-0.003278)
\figpt 8832:(0.988462,-0.010243)
\figpt 8833:(1.000010,-0.010676)
\figpt 8841:(0.991132,0.003278)
\figpt 8842:(0.991132,-0.003278)
\figpt 8843:(1.000045,-0.000000)
\figpt 8851:(0.988462,0.010243)
\figpt 8852:(0.991132,0.003278)
\figpt 8853:(1.000010,0.010676)
\figpt 8861:(0.980093,0.017542)
\figpt 8862:(0.988462,0.010243)
\figpt 8863:(0.999792,0.031683)
\figpt 8871:(0.980093,0.017542)
\figpt 8872:(0.959665,0.014645)
\figpt 8873:(1.004432,-0.227545)
\figpt 8881:(0.947058,0.045315)
\figpt 8882:(0.959665,0.014645)
\figpt 8883:(1.000208,0.049238)
\figpt 8891:(0.980093,0.017542)
\figpt 8892:(0.959665,0.014645)
\figpt 8893:(1.004432,-0.227545)
\figpt 8901:(0.987376,0.026411)
\figpt 8902:(0.980093,0.017542)
\figpt 8903:(1.000208,0.008448)
\figpt 8911:(0.989340,0.034385)
\figpt 8912:(0.987376,0.026411)
\figpt 8913:(0.999696,0.027606)
\figpt 8921:(0.988448,0.041990)
\figpt 8922:(0.989340,0.034385)
\figpt 8923:(0.999285,0.039406)
\figpt 8931:(0.984027,0.050108)
\figpt 8932:(0.988448,0.041990)
\figpt 8933:(0.998715,0.052843)
\figpt 8941:(0.971398,0.057481)
\figpt 8942:(0.984027,0.050108)
\figpt 8943:(0.996985,0.086805)
\figpt 8951:(0.971398,0.057481)
\figpt 8952:(0.947058,0.045315)
\figpt 8953:(1.004432,-0.039041)
\figpt 8961:(0.937666,0.116176)
\figpt 8962:(0.909079,0.075311)
\figpt 8963:(1.004432,0.039041)
\figpt 8971:(0.909079,0.075311)
\figpt 8972:(0.947058,0.045315)
\figpt 8973:(0.995588,0.145800)
\figpt 8981:(0.971398,0.057481)
\figpt 8982:(0.947058,0.045315)
\figpt 8983:(1.004432,-0.039041)
\figpt 8991:(0.979041,0.071893)
\figpt 8992:(0.971398,0.057481)
\figpt 8993:(0.999042,0.052054)
\figpt 9001:(0.980045,0.084590)
\figpt 9002:(0.979041,0.071893)
\figpt 9003:(0.997221,0.076844)
\figpt 9011:(0.976479,0.096959)
\figpt 9012:(0.980045,0.084590)
\figpt 9013:(0.995588,0.095770)
\figpt 9021:(0.965631,0.109861)
\figpt 9022:(0.976479,0.096959)
\figpt 9023:(0.992997,0.121858)
\figpt 9031:(0.937666,0.116176)
\figpt 9032:(0.965631,0.109861)
\figpt 9033:(0.979813,0.237742)
\figpt 9041:(0.942506,0.152070)
\figpt 9042:(0.937666,0.116176)
\figpt 9043:(0.993544,0.126915)
\figpt 9051:(0.937666,0.116176)
\figpt 9052:(0.965631,0.109861)
\figpt 9053:(0.979813,0.237742)
\figpt 9061:(0.977030,0.120218)
\figpt 9062:(0.965631,0.109861)
\figpt 9063:(0.996985,0.086805)
\figpt 9071:(0.979976,0.129649)
\figpt 9072:(0.977030,0.120218)
\figpt 9073:(0.992845,0.120452)
\figpt 9081:(0.979348,0.137927)
\figpt 9082:(0.979976,0.129649)
\figpt 9083:(0.990967,0.134646)
\figpt 9091:(0.975535,0.146105)
\figpt 9092:(0.979348,0.137927)
\figpt 9093:(0.989160,0.147479)
\figpt 9101:(0.965581,0.154134)
\figpt 9102:(0.975535,0.146105)
\figpt 9103:(0.985913,0.169156)
\figpt 9111:(0.942506,0.152070)
\figpt 9112:(0.965581,0.154134)
\figpt 9113:(0.910180,0.643594)
\figpt 9121:(0.934090,0.184787)
\figpt 9122:(0.942506,0.152070)
\figpt 9123:(0.984912,0.180419)
\figpt 9131:(0.942506,0.152070)
\figpt 9132:(0.965581,0.154134)
\figpt 9133:(0.910180,0.643594)
\figpt 9141:(0.973166,0.164138)
\figpt 9142:(0.965581,0.154134)
\figpt 9143:(0.990010,0.143490)
\figpt 9151:(0.974610,0.172565)
\figpt 9152:(0.973166,0.164138)
\figpt 9153:(0.986172,0.166247)
\figpt 9161:(0.973134,0.180030)
\figpt 9162:(0.974610,0.172565)
\figpt 9163:(0.984037,0.178307)
\figpt 9171:(0.968445,0.187429)
\figpt 9172:(0.973134,0.180030)
\figpt 9173:(0.981749,0.190675)
\figpt 9181:(0.956906,0.193838)
\figpt 9182:(0.968445,0.187429)
\figpt 9183:(0.976826,0.216110)
\figpt 9191:(0.956906,0.193838)
\figpt 9192:(0.934090,0.184787)
\figpt 9193:(1.020603,-0.000000)
\figpt 9201:(0.909353,0.216625)
\figpt 9202:(0.934090,0.184787)
\figpt 9203:(0.973015,0.240558)
\figpt 9211:(0.956906,0.193838)
\figpt 9212:(0.934090,0.184787)
\figpt 9213:(1.020603,-0.000000)
\figpt 9221:(0.963235,0.206149)
\figpt 9222:(0.956906,0.193838)
\figpt 9223:(0.982418,0.188504)
\figpt 9231:(0.963594,0.216211)
\figpt 9232:(0.963235,0.206149)
\figpt 9233:(0.977674,0.210671)
\figpt 9241:(0.960570,0.225245)
\figpt 9242:(0.963594,0.216211)
\figpt 9243:(0.974486,0.224881)
\figpt 9251:(0.952952,0.234079)
\figpt 9252:(0.960570,0.225245)
\figpt 9253:(0.970572,0.241570)
\figpt 9261:(0.935084,0.239565)
\figpt 9262:(0.952952,0.234079)
\figpt 9263:(0.959418,0.286981)
\figpt 9271:(0.935084,0.239565)
\figpt 9272:(0.909353,0.216625)
\figpt 9273:(0.995588,0.145800)
\figpt 9281:(0.868959,0.303059)
\figpt 9282:(0.851148,0.237367)
\figpt 9283:(0.979813,0.237742)
\figpt 9291:(0.851148,0.237367)
\figpt 9292:(0.909353,0.216625)
\figpt 9293:(0.937786,0.388443)
\figpt 9301:(0.935084,0.239565)
\figpt 9302:(0.909353,0.216625)
\figpt 9303:(0.995588,0.145800)
\figpt 9311:(0.940347,0.260180)
\figpt 9312:(0.935084,0.239565)
\figpt 9313:(0.971109,0.241348)
\figpt 9321:(0.937736,0.277045)
\figpt 9322:(0.940347,0.260180)
\figpt 9323:(0.962558,0.272252)
\figpt 9331:(0.928980,0.292391)
\figpt 9332:(0.937736,0.277045)
\figpt 9333:(0.955194,0.297178)
\figpt 9341:(0.909663,0.306081)
\figpt 9342:(0.928980,0.292391)
\figpt 9343:(0.943714,0.333653)
\figpt 9351:(0.868959,0.303059)
\figpt 9352:(0.909663,0.306081)
\figpt 9353:(0.871139,0.549342)
\figpt 9361:(0.858731,0.355698)
\figpt 9362:(0.868959,0.303059)
\figpt 9363:(0.942522,0.344667)
\figpt 9371:(0.868959,0.303059)
\figpt 9372:(0.909663,0.306081)
\figpt 9373:(0.871139,0.549342)
\figpt 9381:(0.921718,0.324651)
\figpt 9382:(0.909663,0.306081)
\figpt 9383:(0.959418,0.286981)
\figpt 9391:(0.922549,0.339143)
\figpt 9392:(0.921718,0.324651)
\figpt 9393:(0.944039,0.330641)
\figpt 9401:(0.918627,0.350928)
\figpt 9402:(0.922549,0.339143)
\figpt 9403:(0.936768,0.350420)
\figpt 9411:(0.909909,0.361526)
\figpt 9412:(0.918627,0.350928)
\figpt 9413:(0.929700,0.368923)
\figpt 9421:(0.891806,0.369398)
\figpt 9422:(0.909909,0.361526)
\figpt 9423:(0.916648,0.401773)
\figpt 9431:(0.891806,0.369398)
\figpt 9432:(0.858731,0.355698)
\figpt 9441:(0.828742,0.400152)
\figpt 9442:(0.858731,0.355698)
\figpt 9443:(0.910180,0.422748)
\figpt 9451:(0.858731,0.355698)
\figpt 9452:(0.891806,0.369398)
\figpt 9461:(0.899040,0.387765)
\figpt 9462:(0.891806,0.369398)
\figpt 9463:(0.932264,0.364072)
\figpt 9471:(0.897711,0.401424)
\figpt 9472:(0.899040,0.387765)
\figpt 9473:(0.918265,0.396529)
\figpt 9481:(0.892151,0.412530)
\figpt 9482:(0.897711,0.401424)
\figpt 9483:(0.910180,0.414611)
\figpt 9491:(0.881316,0.422190)
\figpt 9492:(0.892151,0.412530)
\figpt 9493:(0.901335,0.433738)
\figpt 9501:(0.859661,0.426797)
\figpt 9502:(0.881316,0.422190)
\figpt 9503:(0.881337,0.475485)
\figpt 9511:(0.859661,0.426797)
\figpt 9512:(0.828742,0.400152)
\figpt 9513:(1.004432,0.227545)
\figpt 9521:(0.796186,0.489833)
\figpt 9522:(0.769697,0.434009)
\figpt 9523:(0.937786,0.388443)
\figpt 9531:(0.769697,0.434009)
\figpt 9532:(0.828742,0.400152)
\figpt 9533:(0.860942,0.524723)
\figpt 9541:(0.859661,0.426797)
\figpt 9542:(0.828742,0.400152)
\figpt 9543:(1.004432,0.227545)
\figpt 9551:(0.863639,0.450137)
\figpt 9552:(0.859661,0.426797)
\figpt 9553:(0.903235,0.431378)
\figpt 9561:(0.858980,0.467179)
\figpt 9562:(0.863639,0.450137)
\figpt 9563:(0.885561,0.465287)
\figpt 9571:(0.848901,0.480950)
\figpt 9572:(0.858980,0.467179)
\figpt 9573:(0.873143,0.488120)
\figpt 9581:(0.830602,0.491806)
\figpt 9582:(0.848901,0.480950)
\figpt 9583:(0.857336,0.516019)
\figpt 9591:(0.796186,0.489833)
\figpt 9592:(0.830602,0.491806)
\figpt 9593:(0.807083,0.600890)
\figpt 9601:(0.791165,0.529838)
\figpt 9602:(0.796186,0.489833)
\figpt 9603:(0.858126,0.517925)
\figpt 9611:(0.796186,0.489833)
\figpt 9612:(0.830602,0.491806)
\figpt 9613:(0.807083,0.600890)
\figpt 9621:(0.839358,0.508320)
\figpt 9622:(0.830602,0.491806)
\figpt 9623:(0.881337,0.475485)
\figpt 9631:(0.838497,0.519953)
\figpt 9632:(0.839358,0.508320)
\figpt 9633:(0.857114,0.515482)
\figpt 9641:(0.834249,0.528480)
\figpt 9642:(0.838497,0.519953)
\figpt 9643:(0.848080,0.530050)
\figpt 9651:(0.826880,0.535341)
\figpt 9652:(0.834249,0.528480)
\figpt 9653:(0.840287,0.542353)
\figpt 9661:(0.813699,0.539571)
\figpt 9662:(0.826880,0.535341)
\figpt 9663:(0.827967,0.561382)
\figpt 9671:(0.791165,0.529838)
\figpt 9672:(0.813699,0.539571)
\figpt 9673:(0.721675,0.721675)
\figpt 9681:(0.773982,0.558922)
\figpt 9682:(0.791165,0.529838)
\figpt 9683:(0.824013,0.568862)
\figpt 9691:(0.791165,0.529838)
\figpt 9692:(0.813699,0.539571)
\figpt 9693:(0.721675,0.721675)
\figpt 9701:(0.817326,0.552261)
\figpt 9702:(0.813699,0.539571)
\figpt 9703:(0.843533,0.537907)
\figpt 9711:(0.815410,0.560810)
\figpt 9712:(0.817326,0.552261)
\figpt 9713:(0.829029,0.559374)
\figpt 9721:(0.811175,0.567131)
\figpt 9722:(0.815410,0.560810)
\figpt 9723:(0.821901,0.569737)
\figpt 9731:(0.804196,0.572069)
\figpt 9732:(0.811175,0.567131)
\figpt 9733:(0.814883,0.579775)
\figpt 9741:(0.791758,0.573780)
\figpt 9742:(0.804196,0.572069)
\figpt 9743:(0.801506,0.598580)
\figpt 9751:(0.791758,0.573780)
\figpt 9752:(0.773982,0.558922)
\figpt 9753:(1.098684,0.188504)
\figpt 9761:(0.745179,0.580881)
\figpt 9762:(0.773982,0.558922)
\figpt 9763:(0.792284,0.612800)
\figpt 9771:(0.791758,0.573780)
\figpt 9772:(0.773982,0.558922)
\figpt 9773:(1.098684,0.188504)
\figpt 9781:(0.793119,0.586496)
\figpt 9782:(0.791758,0.573780)
\figpt 9783:(0.816757,0.577535)
\figpt 9791:(0.790032,0.594975)
\figpt 9792:(0.793119,0.586496)
\figpt 9793:(0.803725,0.595158)
\figpt 9801:(0.784624,0.601272)
\figpt 9802:(0.790032,0.594975)
\figpt 9803:(0.795929,0.605511)
\figpt 9811:(0.775871,0.605857)
\figpt 9812:(0.784624,0.601272)
\figpt 9813:(0.787220,0.616875)
\figpt 9821:(0.760488,0.605121)
\figpt 9822:(0.775871,0.605857)
\figpt 9823:(0.766356,0.643594)
\figpt 9831:(0.760488,0.605121)
\figpt 9832:(0.745179,0.580881)
\figpt 9833:(0.860942,0.524723)
\figpt 9841:(0.701713,0.637628)
\figpt 9842:(0.696069,0.589564)
\figpt 9843:(0.807083,0.600890)
\figpt 9851:(0.696069,0.589564)
\figpt 9852:(0.745179,0.580881)
\figpt 9853:(0.737846,0.682635)
\figpt 9861:(0.760488,0.605121)
\figpt 9862:(0.745179,0.580881)
\figpt 9863:(0.860942,0.524723)
\figpt 9871:(0.759035,0.621914)
\figpt 9872:(0.760488,0.605121)
\figpt 9873:(0.788322,0.615988)
\figpt 9881:(0.752810,0.633182)
\figpt 9882:(0.759035,0.621914)
\figpt 9883:(0.771706,0.636267)
\figpt 9891:(0.743122,0.641450)
\figpt 9892:(0.752810,0.633182)
\figpt 9893:(0.759479,0.650805)
\figpt 9901:(0.727527,0.646237)
\figpt 9902:(0.743122,0.641450)
\figpt 9903:(0.743237,0.669621)
\figpt 9911:(0.701713,0.637628)
\figpt 9912:(0.727527,0.646237)
\figpt 9913:(0.682635,0.737846)
\figpt 9921:(0.688942,0.668230)
\figpt 9922:(0.701713,0.637628)
\figpt 9923:(0.742070,0.672437)
\figpt 9931:(0.701713,0.637628)
\figpt 9932:(0.727527,0.646237)
\figpt 9933:(0.682635,0.737846)
\figpt 9941:(0.731244,0.660381)
\figpt 9942:(0.727527,0.646237)
\figpt 9943:(0.766356,0.643594)
\figpt 9951:(0.728629,0.669247)
\figpt 9952:(0.731244,0.660381)
\figpt 9953:(0.743564,0.668832)
\figpt 9961:(0.723883,0.675256)
\figpt 9962:(0.728629,0.669247)
\figpt 9963:(0.734466,0.678737)
\figpt 9971:(0.716856,0.679505)
\figpt 9972:(0.723883,0.675256)
\figpt 9973:(0.726412,0.687371)
\figpt 9981:(0.705435,0.680626)
\figpt 9982:(0.716856,0.679505)
\figpt 9983:(0.713227,0.701280)
\figpt 9991:(0.688942,0.668230)
\figpt 9992:(0.705435,0.680626)
\figpt 9993:(0.549342,0.871139)
\figpt 10001:(0.668230,0.688942)
\figpt 10002:(0.688942,0.668230)
\figpt 10003:(0.707785,0.707785)
\figpt 10011:(0.688942,0.668230)
\figpt 10012:(0.705435,0.680626)
\figpt 10013:(0.549342,0.871139)
\figpt 10021:(0.706192,0.691705)
\figpt 10022:(0.705435,0.680626)
\figpt 10023:(0.729363,0.684557)
\figpt 10031:(0.703155,0.698518)
\figpt 10032:(0.706192,0.691705)
\figpt 10033:(0.714663,0.699565)
\figpt 10041:(0.698518,0.703155)
\figpt 10042:(0.703155,0.698518)
\figpt 10043:(0.707139,0.707139)
\figpt 10051:(0.691705,0.706192)
\figpt 10052:(0.698518,0.703155)
\figpt 10053:(0.699565,0.714663)
\figpt 10061:(0.680626,0.705435)
\figpt 10062:(0.691705,0.706192)
\figpt 10063:(0.684557,0.729363)
\figpt 10071:(0.680626,0.705435)
\figpt 10072:(0.668230,0.688942)
\figpt 10073:(0.871139,0.549342)
\figpt 10081:(0.637628,0.701713)
\figpt 10082:(0.668230,0.688942)
\figpt 10083:(0.672437,0.742070)
\figpt 10091:(0.680626,0.705435)
\figpt 10092:(0.668230,0.688942)
\figpt 10093:(0.871139,0.549342)
\figpt 10101:(0.679505,0.716856)
\figpt 10102:(0.680626,0.705435)
\figpt 10103:(0.701280,0.713227)
\figpt 10111:(0.675256,0.723883)
\figpt 10112:(0.679505,0.716856)
\figpt 10113:(0.687371,0.726412)
\figpt 10121:(0.669247,0.728629)
\figpt 10122:(0.675256,0.723883)
\figpt 10123:(0.678737,0.734466)
\figpt 10131:(0.660381,0.731244)
\figpt 10132:(0.669247,0.728629)
\figpt 10133:(0.668832,0.743564)
\figpt 10141:(0.646237,0.727527)
\figpt 10142:(0.660381,0.731244)
\figpt 10143:(0.643594,0.766356)
\figpt 10151:(0.646237,0.727527)
\figpt 10152:(0.637628,0.701713)
\figpt 10153:(0.737846,0.682635)
\figpt 10161:(0.580881,0.745179)
\figpt 10162:(0.589564,0.696069)
\figpt 10163:(0.682635,0.737846)
\figpt 10171:(0.589564,0.696069)
\figpt 10172:(0.637628,0.701713)
\figpt 10173:(0.600890,0.807083)
\figpt 10181:(0.646237,0.727527)
\figpt 10182:(0.637628,0.701713)
\figpt 10183:(0.737846,0.682635)
\figpt 10191:(0.641450,0.743122)
\figpt 10192:(0.646237,0.727527)
\figpt 10193:(0.669621,0.743237)
\figpt 10201:(0.633182,0.752810)
\figpt 10202:(0.641450,0.743122)
\figpt 10203:(0.650805,0.759479)
\figpt 10211:(0.621914,0.759035)
\figpt 10212:(0.633182,0.752810)
\figpt 10213:(0.636267,0.771706)
\figpt 10221:(0.605121,0.760488)
\figpt 10222:(0.621914,0.759035)
\figpt 10223:(0.615988,0.788322)
\figpt 10231:(0.580881,0.745179)
\figpt 10232:(0.605121,0.760488)
\figpt 10233:(0.524723,0.860942)
\figpt 10241:(0.558922,0.773982)
\figpt 10242:(0.580881,0.745179)
\figpt 10243:(0.612800,0.792284)
\figpt 10251:(0.580881,0.745179)
\figpt 10252:(0.605121,0.760488)
\figpt 10253:(0.524723,0.860942)
\figpt 10261:(0.605857,0.775871)
\figpt 10262:(0.605121,0.760488)
\figpt 10263:(0.643594,0.766356)
\figpt 10271:(0.601272,0.784624)
\figpt 10272:(0.605857,0.775871)
\figpt 10273:(0.616875,0.787220)
\figpt 10281:(0.594975,0.790032)
\figpt 10282:(0.601272,0.784624)
\figpt 10283:(0.605511,0.795929)
\figpt 10291:(0.586496,0.793119)
\figpt 10292:(0.594975,0.790032)
\figpt 10293:(0.595158,0.803725)
\figpt 10301:(0.573780,0.791758)
\figpt 10302:(0.586496,0.793119)
\figpt 10303:(0.577535,0.816757)
\figpt 10311:(0.558922,0.773982)
\figpt 10312:(0.573780,0.791758)
\figpt 10313:(0.188504,1.098684)
\figpt 10321:(0.529838,0.791165)
\figpt 10322:(0.558922,0.773982)
\figpt 10323:(0.568862,0.824013)
\figpt 10331:(0.558922,0.773982)
\figpt 10332:(0.573780,0.791758)
\figpt 10333:(0.188504,1.098684)
\figpt 10341:(0.572069,0.804196)
\figpt 10342:(0.573780,0.791758)
\figpt 10343:(0.598580,0.801506)
\figpt 10351:(0.567131,0.811175)
\figpt 10352:(0.572069,0.804196)
\figpt 10353:(0.579775,0.814883)
\figpt 10361:(0.560810,0.815410)
\figpt 10362:(0.567131,0.811175)
\figpt 10363:(0.569737,0.821901)
\figpt 10371:(0.552261,0.817326)
\figpt 10372:(0.560810,0.815410)
\figpt 10373:(0.559374,0.829029)
\figpt 10381:(0.539571,0.813699)
\figpt 10382:(0.552261,0.817326)
\figpt 10383:(0.537907,0.843533)
\figpt 10391:(0.539571,0.813699)
\figpt 10392:(0.529838,0.791165)
\figpt 10393:(0.721675,0.721675)
\figpt 10401:(0.489833,0.796186)
\figpt 10402:(0.529838,0.791165)
\figpt 10403:(0.517925,0.858126)
\figpt 10411:(0.539571,0.813699)
\figpt 10412:(0.529838,0.791165)
\figpt 10413:(0.721675,0.721675)
\figpt 10421:(0.535341,0.826880)
\figpt 10422:(0.539571,0.813699)
\figpt 10423:(0.561382,0.827967)
\figpt 10431:(0.528480,0.834249)
\figpt 10432:(0.535341,0.826880)
\figpt 10433:(0.542353,0.840287)
\figpt 10441:(0.519953,0.838497)
\figpt 10442:(0.528480,0.834249)
\figpt 10443:(0.530050,0.848080)
\figpt 10451:(0.508320,0.839358)
\figpt 10452:(0.519953,0.838497)
\figpt 10453:(0.515482,0.857114)
\figpt 10461:(0.491806,0.830602)
\figpt 10462:(0.508320,0.839358)
\figpt 10463:(0.475485,0.881337)
\figpt 10471:(0.491806,0.830602)
\figpt 10472:(0.489833,0.796186)
\figpt 10473:(0.600890,0.807083)
\figpt 10481:(0.400152,0.828742)
\figpt 10482:(0.434009,0.769697)
\figpt 10483:(0.524723,0.860942)
\figpt 10491:(0.434009,0.769697)
\figpt 10492:(0.489833,0.796186)
\figpt 10493:(0.388443,0.937786)
\figpt 10501:(0.491806,0.830602)
\figpt 10502:(0.489833,0.796186)
\figpt 10503:(0.600890,0.807083)
\figpt 10511:(0.480950,0.848901)
\figpt 10512:(0.491806,0.830602)
\figpt 10513:(0.516019,0.857336)
\figpt 10521:(0.467179,0.858980)
\figpt 10522:(0.480950,0.848901)
\figpt 10523:(0.488120,0.873143)
\figpt 10531:(0.450137,0.863639)
\figpt 10532:(0.467179,0.858980)
\figpt 10533:(0.465287,0.885561)
\figpt 10541:(0.426797,0.859661)
\figpt 10542:(0.450137,0.863639)
\figpt 10543:(0.431378,0.903235)
\figpt 10551:(0.400152,0.828742)
\figpt 10552:(0.426797,0.859661)
\figpt 10553:(0.227545,1.004432)
\figpt 10561:(0.355698,0.858731)
\figpt 10562:(0.400152,0.828742)
\figpt 10563:(0.422748,0.910180)
\figpt 10571:(0.400152,0.828742)
\figpt 10572:(0.426797,0.859661)
\figpt 10573:(0.227545,1.004432)
\figpt 10581:(0.422190,0.881316)
\figpt 10582:(0.426797,0.859661)
\figpt 10583:(0.475485,0.881337)
\figpt 10591:(0.412530,0.892151)
\figpt 10592:(0.422190,0.881316)
\figpt 10593:(0.433738,0.901335)
\figpt 10601:(0.401424,0.897711)
\figpt 10602:(0.412530,0.892151)
\figpt 10603:(0.414611,0.910180)
\figpt 10611:(0.387765,0.899040)
\figpt 10612:(0.401424,0.897711)
\figpt 10613:(0.396529,0.918265)
\figpt 10621:(0.369398,0.891806)
\figpt 10622:(0.387765,0.899040)
\figpt 10623:(0.364072,0.932264)
\figpt 10631:(0.355698,0.858731)
\figpt 10632:(0.369398,0.891806)
\figpt 10641:(0.303059,0.868959)
\figpt 10642:(0.355698,0.858731)
\figpt 10643:(0.344667,0.942522)
\figpt 10651:(0.369398,0.891806)
\figpt 10652:(0.355698,0.858731)
\figpt 10661:(0.361526,0.909909)
\figpt 10662:(0.369398,0.891806)
\figpt 10663:(0.401773,0.916648)
\figpt 10671:(0.350928,0.918627)
\figpt 10672:(0.361526,0.909909)
\figpt 10673:(0.368923,0.929700)
\figpt 10681:(0.339143,0.922549)
\figpt 10682:(0.350928,0.918627)
\figpt 10683:(0.350420,0.936768)
\figpt 10691:(0.324651,0.921718)
\figpt 10692:(0.339143,0.922549)
\figpt 10693:(0.330641,0.944039)
\figpt 10701:(0.306081,0.909663)
\figpt 10702:(0.324651,0.921718)
\figpt 10703:(0.286981,0.959418)
\figpt 10711:(0.306081,0.909663)
\figpt 10712:(0.303059,0.868959)
\figpt 10713:(0.549342,0.871139)
\figpt 10721:(0.216625,0.909353)
\figpt 10722:(0.237367,0.851148)
\figpt 10723:(0.388443,0.937786)
\figpt 10731:(0.237367,0.851148)
\figpt 10732:(0.303059,0.868959)
\figpt 10733:(0.237742,0.979813)
\figpt 10741:(0.306081,0.909663)
\figpt 10742:(0.303059,0.868959)
\figpt 10743:(0.549342,0.871139)
\figpt 10751:(0.292391,0.928980)
\figpt 10752:(0.306081,0.909663)
\figpt 10753:(0.333653,0.943714)
\figpt 10761:(0.277045,0.937736)
\figpt 10762:(0.292391,0.928980)
\figpt 10763:(0.297178,0.955194)
\figpt 10771:(0.260180,0.940347)
\figpt 10772:(0.277045,0.937736)
\figpt 10773:(0.272252,0.962558)
\figpt 10781:(0.239565,0.935084)
\figpt 10782:(0.260180,0.940347)
\figpt 10783:(0.241348,0.971109)
\figpt 10791:(0.216625,0.909353)
\figpt 10792:(0.239565,0.935084)
\figpt 10793:(0.145800,0.995588)
\figpt 10801:(0.184787,0.934090)
\figpt 10802:(0.216625,0.909353)
\figpt 10803:(0.240558,0.973015)
\figpt 10811:(0.216625,0.909353)
\figpt 10812:(0.239565,0.935084)
\figpt 10813:(0.145800,0.995588)
\figpt 10821:(0.234079,0.952952)
\figpt 10822:(0.239565,0.935084)
\figpt 10823:(0.286981,0.959418)
\figpt 10831:(0.225245,0.960570)
\figpt 10832:(0.234079,0.952952)
\figpt 10833:(0.241570,0.970572)
\figpt 10841:(0.216211,0.963594)
\figpt 10842:(0.225245,0.960570)
\figpt 10843:(0.224881,0.974486)
\figpt 10851:(0.206149,0.963235)
\figpt 10852:(0.216211,0.963594)
\figpt 10853:(0.210671,0.977674)
\figpt 10861:(0.193838,0.956906)
\figpt 10862:(0.206149,0.963235)
\figpt 10863:(0.188504,0.982418)
\figpt 10871:(0.184787,0.934090)
\figpt 10872:(0.193838,0.956906)
\figpt 10873:(-0.000000,1.020603)
\figpt 10881:(0.152070,0.942506)
\figpt 10882:(0.184787,0.934090)
\figpt 10883:(0.180419,0.984912)
\figpt 10891:(0.184787,0.934090)
\figpt 10892:(0.193838,0.956906)
\figpt 10893:(0.000000,1.020603)
\figpt 10901:(0.187429,0.968445)
\figpt 10902:(0.193838,0.956906)
\figpt 10903:(0.216110,0.976826)
\figpt 10911:(0.180030,0.973134)
\figpt 10912:(0.187429,0.968445)
\figpt 10913:(0.190675,0.981749)
\figpt 10921:(0.172565,0.974610)
\figpt 10922:(0.180030,0.973134)
\figpt 10923:(0.178307,0.984037)
\figpt 10931:(0.164138,0.973166)
\figpt 10932:(0.172565,0.974610)
\figpt 10933:(0.166247,0.986172)
\figpt 10941:(0.154134,0.965581)
\figpt 10942:(0.164138,0.973166)
\figpt 10943:(0.143490,0.990010)
\figpt 10951:(0.154134,0.965581)
\figpt 10952:(0.152070,0.942506)
\figpt 10953:(0.643594,0.910180)
\figpt 10961:(0.116176,0.937666)
\figpt 10962:(0.152070,0.942506)
\figpt 10963:(0.126915,0.993544)
\figpt 10971:(0.154134,0.965581)
\figpt 10972:(0.152070,0.942506)
\figpt 10973:(0.643594,0.910180)
\figpt 10981:(0.146105,0.975535)
\figpt 10982:(0.154134,0.965581)
\figpt 10983:(0.169156,0.985913)
\figpt 10991:(0.137927,0.979348)
\figpt 10992:(0.146105,0.975535)
\figpt 10993:(0.147479,0.989160)
\figpt 11001:(0.129649,0.979976)
\figpt 11002:(0.137927,0.979348)
\figpt 11003:(0.134646,0.990967)
\figpt 11011:(0.120218,0.977030)
\figpt 11012:(0.129649,0.979976)
\figpt 11013:(0.120452,0.992845)
\figpt 11021:(0.109861,0.965631)
\figpt 11022:(0.120218,0.977030)
\figpt 11023:(0.086805,0.996985)
\figpt 11031:(0.109861,0.965631)
\figpt 11032:(0.116176,0.937666)
\figpt 11033:(0.237742,0.979813)
\figpt 11041:(0.045315,0.947058)
\figpt 11042:(0.075311,0.909079)
\figpt 11043:(0.145800,0.995588)
\figpt 11051:(0.075311,0.909079)
\figpt 11052:(0.116176,0.937666)
\figpt 11053:(0.039041,1.004432)
\figpt 11061:(0.109861,0.965631)
\figpt 11062:(0.116176,0.937666)
\figpt 11063:(0.237742,0.979813)
\figpt 11071:(0.096959,0.976479)
\figpt 11072:(0.109861,0.965631)
\figpt 11073:(0.121858,0.992997)
\figpt 11081:(0.084590,0.980045)
\figpt 11082:(0.096959,0.976479)
\figpt 11083:(0.095770,0.995588)
\figpt 11091:(0.071893,0.979041)
\figpt 11092:(0.084590,0.980045)
\figpt 11093:(0.076844,0.997221)
\figpt 11101:(0.057481,0.971398)
\figpt 11102:(0.071893,0.979041)
\figpt 11103:(0.052054,0.999042)
\figpt 11111:(0.045315,0.947058)
\figpt 11112:(0.057481,0.971398)
\figpt 11113:(-0.039041,1.004432)
\figpt 11121:(0.014645,0.959665)
\figpt 11122:(0.045315,0.947058)
\figpt 11123:(0.049238,1.000208)
\figpt 11131:(0.045315,0.947058)
\figpt 11132:(0.057481,0.971398)
\figpt 11133:(-0.039041,1.004432)
\figpt 11141:(0.050108,0.984027)
\figpt 11142:(0.057481,0.971398)
\figpt 11143:(0.086805,0.996985)
\figpt 11151:(0.041990,0.988448)
\figpt 11152:(0.050108,0.984027)
\figpt 11153:(0.052843,0.998715)
\figpt 11161:(0.034385,0.989340)
\figpt 11162:(0.041990,0.988448)
\figpt 11163:(0.039406,0.999285)
\figpt 11171:(0.026411,0.987376)
\figpt 11172:(0.034385,0.989340)
\figpt 11173:(0.027606,0.999696)
\figpt 11181:(0.017542,0.980093)
\figpt 11182:(0.026411,0.987376)
\figpt 11183:(0.008448,1.000208)
\figpt 11191:(0.014645,0.959665)
\figpt 11192:(0.017542,0.980093)
\figpt 11193:(-0.227545,1.004432)
\figpt 11201:(-0.014645,0.959665)
\figpt 11202:(0.014645,0.959665)
\figpt 11203:(0.000000,1.000959)
\figpt 11211:(0.014645,0.959665)
\figpt 11212:(0.017542,0.980093)
\figpt 11213:(-0.227545,1.004432)
\figpt 11221:(0.010243,0.988462)
\figpt 11222:(0.017542,0.980093)
\figpt 11223:(0.031683,0.999792)
\figpt 11231:(0.003278,0.991132)
\figpt 11232:(0.010243,0.988462)
\figpt 11233:(0.010676,1.000010)
\figpt 11241:(-0.003278,0.991132)
\figpt 11242:(0.003278,0.991132)
\figpt 11243:(-0.000000,1.000045)
\figpt 11251:(-0.010243,0.988462)
\figpt 11252:(-0.003278,0.991132)
\figpt 11253:(-0.010676,1.000010)
\figpt 11261:(-0.017542,0.980093)
\figpt 11262:(-0.010243,0.988462)
\figpt 11263:(-0.031683,0.999792)
\figpt 11271:(-0.017542,0.980093)
\figpt 11272:(-0.014645,0.959665)
\figpt 11273:(0.227545,1.004432)
\figpt 11281:(-0.045315,0.947058)
\figpt 11282:(-0.014645,0.959665)
\figpt 11283:(-0.049238,1.000208)
\figpt 11291:(-0.017542,0.980093)
\figpt 11292:(-0.014645,0.959665)
\figpt 11293:(0.227545,1.004432)
\figpt 11301:(-0.026411,0.987376)
\figpt 11302:(-0.017542,0.980093)
\figpt 11303:(-0.008448,1.000208)
\figpt 11311:(-0.034385,0.989340)
\figpt 11312:(-0.026411,0.987376)
\figpt 11313:(-0.027606,0.999696)
\figpt 11321:(-0.041990,0.988448)
\figpt 11322:(-0.034385,0.989340)
\figpt 11323:(-0.039406,0.999285)
\figpt 11331:(-0.050108,0.984027)
\figpt 11332:(-0.041990,0.988448)
\figpt 11333:(-0.052843,0.998715)
\figpt 11341:(-0.057481,0.971398)
\figpt 11342:(-0.050108,0.984027)
\figpt 11343:(-0.086805,0.996985)
\figpt 11351:(-0.057481,0.971398)
\figpt 11352:(-0.045315,0.947058)
\figpt 11353:(0.039041,1.004432)
\figpt 11361:(-0.116176,0.937666)
\figpt 11362:(-0.075311,0.909079)
\figpt 11363:(-0.039041,1.004432)
\figpt 11371:(-0.075311,0.909079)
\figpt 11372:(-0.045315,0.947058)
\figpt 11373:(-0.145800,0.995588)
\figpt 11381:(-0.057481,0.971398)
\figpt 11382:(-0.045315,0.947058)
\figpt 11383:(0.039041,1.004432)
\figpt 11391:(-0.071893,0.979041)
\figpt 11392:(-0.057481,0.971398)
\figpt 11393:(-0.052054,0.999042)
\figpt 11401:(-0.084590,0.980045)
\figpt 11402:(-0.071893,0.979041)
\figpt 11403:(-0.076844,0.997221)
\figpt 11411:(-0.096959,0.976479)
\figpt 11412:(-0.084590,0.980045)
\figpt 11413:(-0.095770,0.995588)
\figpt 11421:(-0.109861,0.965631)
\figpt 11422:(-0.096959,0.976479)
\figpt 11423:(-0.121858,0.992997)
\figpt 11431:(-0.116176,0.937666)
\figpt 11432:(-0.109861,0.965631)
\figpt 11433:(-0.237742,0.979813)
\figpt 11441:(-0.152070,0.942506)
\figpt 11442:(-0.116176,0.937666)
\figpt 11443:(-0.126915,0.993544)
\figpt 11451:(-0.116176,0.937666)
\figpt 11452:(-0.109861,0.965631)
\figpt 11453:(-0.237742,0.979813)
\figpt 11461:(-0.120218,0.977030)
\figpt 11462:(-0.109861,0.965631)
\figpt 11463:(-0.086805,0.996985)
\figpt 11471:(-0.129649,0.979976)
\figpt 11472:(-0.120218,0.977030)
\figpt 11473:(-0.120452,0.992845)
\figpt 11481:(-0.137927,0.979348)
\figpt 11482:(-0.129649,0.979976)
\figpt 11483:(-0.134646,0.990967)
\figpt 11491:(-0.146105,0.975535)
\figpt 11492:(-0.137927,0.979348)
\figpt 11493:(-0.147479,0.989160)
\figpt 11501:(-0.154134,0.965581)
\figpt 11502:(-0.146105,0.975535)
\figpt 11503:(-0.169156,0.985913)
\figpt 11511:(-0.152070,0.942506)
\figpt 11512:(-0.154134,0.965581)
\figpt 11513:(-0.643594,0.910180)
\figpt 11521:(-0.184787,0.934090)
\figpt 11522:(-0.152070,0.942506)
\figpt 11523:(-0.180419,0.984912)
\figpt 11531:(-0.152070,0.942506)
\figpt 11532:(-0.154134,0.965581)
\figpt 11533:(-0.643594,0.910180)
\figpt 11541:(-0.164138,0.973166)
\figpt 11542:(-0.154134,0.965581)
\figpt 11543:(-0.143490,0.990010)
\figpt 11551:(-0.172565,0.974610)
\figpt 11552:(-0.164138,0.973166)
\figpt 11553:(-0.166247,0.986172)
\figpt 11561:(-0.180030,0.973134)
\figpt 11562:(-0.172565,0.974610)
\figpt 11563:(-0.178307,0.984037)
\figpt 11571:(-0.187429,0.968445)
\figpt 11572:(-0.180030,0.973134)
\figpt 11573:(-0.190675,0.981749)
\figpt 11581:(-0.193838,0.956906)
\figpt 11582:(-0.187429,0.968445)
\figpt 11583:(-0.216110,0.976826)
\figpt 11591:(-0.193838,0.956906)
\figpt 11592:(-0.184787,0.934090)
\figpt 11593:(-0.000000,1.020603)
\figpt 11601:(-0.216625,0.909353)
\figpt 11602:(-0.184787,0.934090)
\figpt 11603:(-0.240558,0.973015)
\figpt 11611:(-0.193838,0.956906)
\figpt 11612:(-0.184787,0.934090)
\figpt 11613:(0.000000,1.020603)
\figpt 11621:(-0.206149,0.963235)
\figpt 11622:(-0.193838,0.956906)
\figpt 11623:(-0.188504,0.982418)
\figpt 11631:(-0.216211,0.963594)
\figpt 11632:(-0.206149,0.963235)
\figpt 11633:(-0.210671,0.977674)
\figpt 11641:(-0.225245,0.960570)
\figpt 11642:(-0.216211,0.963594)
\figpt 11643:(-0.224881,0.974486)
\figpt 11651:(-0.234079,0.952952)
\figpt 11652:(-0.225245,0.960570)
\figpt 11653:(-0.241570,0.970572)
\figpt 11661:(-0.239565,0.935084)
\figpt 11662:(-0.234079,0.952952)
\figpt 11663:(-0.286981,0.959418)
\figpt 11671:(-0.239565,0.935084)
\figpt 11672:(-0.216625,0.909353)
\figpt 11673:(-0.145800,0.995588)
\figpt 11681:(-0.303059,0.868959)
\figpt 11682:(-0.237367,0.851148)
\figpt 11683:(-0.237742,0.979813)
\figpt 11691:(-0.237367,0.851148)
\figpt 11692:(-0.216625,0.909353)
\figpt 11693:(-0.388443,0.937786)
\figpt 11701:(-0.239565,0.935084)
\figpt 11702:(-0.216625,0.909353)
\figpt 11703:(-0.145800,0.995588)
\figpt 11711:(-0.260180,0.940347)
\figpt 11712:(-0.239565,0.935084)
\figpt 11713:(-0.241348,0.971109)
\figpt 11721:(-0.277045,0.937736)
\figpt 11722:(-0.260180,0.940347)
\figpt 11723:(-0.272252,0.962558)
\figpt 11731:(-0.292391,0.928980)
\figpt 11732:(-0.277045,0.937736)
\figpt 11733:(-0.297178,0.955194)
\figpt 11741:(-0.306081,0.909663)
\figpt 11742:(-0.292391,0.928980)
\figpt 11743:(-0.333653,0.943714)
\figpt 11751:(-0.303059,0.868959)
\figpt 11752:(-0.306081,0.909663)
\figpt 11753:(-0.549342,0.871139)
\figpt 11761:(-0.355698,0.858731)
\figpt 11762:(-0.303059,0.868959)
\figpt 11763:(-0.344667,0.942522)
\figpt 11771:(-0.303059,0.868959)
\figpt 11772:(-0.306081,0.909663)
\figpt 11773:(-0.549342,0.871139)
\figpt 11781:(-0.324651,0.921718)
\figpt 11782:(-0.306081,0.909663)
\figpt 11783:(-0.286981,0.959418)
\figpt 11791:(-0.339143,0.922549)
\figpt 11792:(-0.324651,0.921718)
\figpt 11793:(-0.330641,0.944039)
\figpt 11801:(-0.350928,0.918627)
\figpt 11802:(-0.339143,0.922549)
\figpt 11803:(-0.350420,0.936768)
\figpt 11811:(-0.361526,0.909909)
\figpt 11812:(-0.350928,0.918627)
\figpt 11813:(-0.368923,0.929700)
\figpt 11821:(-0.369398,0.891806)
\figpt 11822:(-0.361526,0.909909)
\figpt 11823:(-0.401773,0.916648)
\figpt 11831:(-0.355698,0.858731)
\figpt 11832:(-0.369398,0.891806)
\figpt 11841:(-0.400152,0.828742)
\figpt 11842:(-0.355698,0.858731)
\figpt 11843:(-0.422748,0.910180)
\figpt 11851:(-0.369398,0.891806)
\figpt 11852:(-0.355698,0.858731)
\figpt 11861:(-0.387765,0.899040)
\figpt 11862:(-0.369398,0.891806)
\figpt 11863:(-0.364072,0.932264)
\figpt 11871:(-0.401424,0.897711)
\figpt 11872:(-0.387765,0.899040)
\figpt 11873:(-0.396529,0.918265)
\figpt 11881:(-0.412530,0.892151)
\figpt 11882:(-0.401424,0.897711)
\figpt 11883:(-0.414611,0.910180)
\figpt 11891:(-0.422190,0.881316)
\figpt 11892:(-0.412530,0.892151)
\figpt 11893:(-0.433738,0.901335)
\figpt 11901:(-0.426797,0.859661)
\figpt 11902:(-0.422190,0.881316)
\figpt 11903:(-0.475485,0.881337)
\figpt 11911:(-0.426797,0.859661)
\figpt 11912:(-0.400152,0.828742)
\figpt 11913:(-0.227545,1.004432)
\figpt 11921:(-0.489833,0.796186)
\figpt 11922:(-0.434009,0.769697)
\figpt 11923:(-0.388443,0.937786)
\figpt 11931:(-0.434009,0.769697)
\figpt 11932:(-0.400152,0.828742)
\figpt 11933:(-0.524723,0.860942)
\figpt 11941:(-0.426797,0.859661)
\figpt 11942:(-0.400152,0.828742)
\figpt 11943:(-0.227545,1.004432)
\figpt 11951:(-0.450137,0.863639)
\figpt 11952:(-0.426797,0.859661)
\figpt 11953:(-0.431378,0.903235)
\figpt 11961:(-0.467179,0.858980)
\figpt 11962:(-0.450137,0.863639)
\figpt 11963:(-0.465287,0.885561)
\figpt 11971:(-0.480950,0.848901)
\figpt 11972:(-0.467179,0.858980)
\figpt 11973:(-0.488120,0.873143)
\figpt 11981:(-0.491806,0.830602)
\figpt 11982:(-0.480950,0.848901)
\figpt 11983:(-0.516019,0.857336)
\figpt 11991:(-0.489833,0.796186)
\figpt 11992:(-0.491806,0.830602)
\figpt 11993:(-0.600890,0.807083)
\figpt 12001:(-0.529838,0.791165)
\figpt 12002:(-0.489833,0.796186)
\figpt 12003:(-0.517925,0.858126)
\figpt 12011:(-0.489833,0.796186)
\figpt 12012:(-0.491806,0.830602)
\figpt 12013:(-0.600890,0.807083)
\figpt 12021:(-0.508320,0.839358)
\figpt 12022:(-0.491806,0.830602)
\figpt 12023:(-0.475485,0.881337)
\figpt 12031:(-0.519953,0.838497)
\figpt 12032:(-0.508320,0.839358)
\figpt 12033:(-0.515482,0.857114)
\figpt 12041:(-0.528480,0.834249)
\figpt 12042:(-0.519953,0.838497)
\figpt 12043:(-0.530050,0.848080)
\figpt 12051:(-0.535341,0.826880)
\figpt 12052:(-0.528480,0.834249)
\figpt 12053:(-0.542353,0.840287)
\figpt 12061:(-0.539571,0.813699)
\figpt 12062:(-0.535341,0.826880)
\figpt 12063:(-0.561382,0.827967)
\figpt 12071:(-0.529838,0.791165)
\figpt 12072:(-0.539571,0.813699)
\figpt 12073:(-0.721675,0.721675)
\figpt 12081:(-0.558922,0.773982)
\figpt 12082:(-0.529838,0.791165)
\figpt 12083:(-0.568862,0.824013)
\figpt 12091:(-0.529838,0.791165)
\figpt 12092:(-0.539571,0.813699)
\figpt 12093:(-0.721675,0.721675)
\figpt 12101:(-0.552261,0.817326)
\figpt 12102:(-0.539571,0.813699)
\figpt 12103:(-0.537907,0.843533)
\figpt 12111:(-0.560810,0.815410)
\figpt 12112:(-0.552261,0.817326)
\figpt 12113:(-0.559374,0.829029)
\figpt 12121:(-0.567131,0.811175)
\figpt 12122:(-0.560810,0.815410)
\figpt 12123:(-0.569737,0.821901)
\figpt 12131:(-0.572069,0.804196)
\figpt 12132:(-0.567131,0.811175)
\figpt 12133:(-0.579775,0.814883)
\figpt 12141:(-0.573780,0.791758)
\figpt 12142:(-0.572069,0.804196)
\figpt 12143:(-0.598580,0.801506)
\figpt 12151:(-0.573780,0.791758)
\figpt 12152:(-0.558922,0.773982)
\figpt 12153:(-0.188504,1.098684)
\figpt 12161:(-0.580881,0.745179)
\figpt 12162:(-0.558922,0.773982)
\figpt 12163:(-0.612800,0.792284)
\figpt 12171:(-0.573780,0.791758)
\figpt 12172:(-0.558922,0.773982)
\figpt 12173:(-0.188504,1.098684)
\figpt 12181:(-0.586496,0.793119)
\figpt 12182:(-0.573780,0.791758)
\figpt 12183:(-0.577535,0.816757)
\figpt 12191:(-0.594975,0.790032)
\figpt 12192:(-0.586496,0.793119)
\figpt 12193:(-0.595158,0.803725)
\figpt 12201:(-0.601272,0.784624)
\figpt 12202:(-0.594975,0.790032)
\figpt 12203:(-0.605511,0.795929)
\figpt 12211:(-0.605857,0.775871)
\figpt 12212:(-0.601272,0.784624)
\figpt 12213:(-0.616875,0.787220)
\figpt 12221:(-0.605121,0.760488)
\figpt 12222:(-0.605857,0.775871)
\figpt 12223:(-0.643594,0.766356)
\figpt 12231:(-0.605121,0.760488)
\figpt 12232:(-0.580881,0.745179)
\figpt 12233:(-0.524723,0.860942)
\figpt 12241:(-0.637628,0.701713)
\figpt 12242:(-0.589564,0.696069)
\figpt 12243:(-0.600890,0.807083)
\figpt 12251:(-0.589564,0.696069)
\figpt 12252:(-0.580881,0.745179)
\figpt 12253:(-0.682635,0.737846)
\figpt 12261:(-0.605121,0.760488)
\figpt 12262:(-0.580881,0.745179)
\figpt 12263:(-0.524723,0.860942)
\figpt 12271:(-0.621914,0.759035)
\figpt 12272:(-0.605121,0.760488)
\figpt 12273:(-0.615988,0.788322)
\figpt 12281:(-0.633182,0.752810)
\figpt 12282:(-0.621914,0.759035)
\figpt 12283:(-0.636267,0.771706)
\figpt 12291:(-0.641450,0.743122)
\figpt 12292:(-0.633182,0.752810)
\figpt 12293:(-0.650805,0.759479)
\figpt 12301:(-0.646237,0.727527)
\figpt 12302:(-0.641450,0.743122)
\figpt 12303:(-0.669621,0.743237)
\figpt 12311:(-0.637628,0.701713)
\figpt 12312:(-0.646237,0.727527)
\figpt 12313:(-0.737846,0.682635)
\figpt 12321:(-0.668230,0.688942)
\figpt 12322:(-0.637628,0.701713)
\figpt 12323:(-0.672437,0.742070)
\figpt 12331:(-0.637628,0.701713)
\figpt 12332:(-0.646237,0.727527)
\figpt 12333:(-0.737846,0.682635)
\figpt 12341:(-0.660381,0.731244)
\figpt 12342:(-0.646237,0.727527)
\figpt 12343:(-0.643594,0.766356)
\figpt 12351:(-0.669247,0.728629)
\figpt 12352:(-0.660381,0.731244)
\figpt 12353:(-0.668832,0.743564)
\figpt 12361:(-0.675256,0.723883)
\figpt 12362:(-0.669247,0.728629)
\figpt 12363:(-0.678737,0.734466)
\figpt 12371:(-0.679505,0.716856)
\figpt 12372:(-0.675256,0.723883)
\figpt 12373:(-0.687371,0.726412)
\figpt 12381:(-0.680626,0.705435)
\figpt 12382:(-0.679505,0.716856)
\figpt 12383:(-0.701280,0.713227)
\figpt 12391:(-0.668230,0.688942)
\figpt 12392:(-0.680626,0.705435)
\figpt 12393:(-0.871139,0.549342)
\figpt 12401:(-0.688942,0.668230)
\figpt 12402:(-0.668230,0.688942)
\figpt 12403:(-0.707785,0.707785)
\figpt 12411:(-0.668230,0.688942)
\figpt 12412:(-0.680626,0.705435)
\figpt 12413:(-0.871139,0.549342)
\figpt 12421:(-0.691705,0.706192)
\figpt 12422:(-0.680626,0.705435)
\figpt 12423:(-0.684557,0.729363)
\figpt 12431:(-0.698518,0.703155)
\figpt 12432:(-0.691705,0.706192)
\figpt 12433:(-0.699565,0.714663)
\figpt 12441:(-0.703155,0.698518)
\figpt 12442:(-0.698518,0.703155)
\figpt 12443:(-0.707139,0.707139)
\figpt 12451:(-0.706192,0.691705)
\figpt 12452:(-0.703155,0.698518)
\figpt 12453:(-0.714663,0.699565)
\figpt 12461:(-0.705435,0.680626)
\figpt 12462:(-0.706192,0.691705)
\figpt 12463:(-0.729363,0.684557)
\figpt 12471:(-0.705435,0.680626)
\figpt 12472:(-0.688942,0.668230)
\figpt 12473:(-0.549342,0.871139)
\figpt 12481:(-0.701713,0.637628)
\figpt 12482:(-0.688942,0.668230)
\figpt 12483:(-0.742070,0.672437)
\figpt 12491:(-0.705435,0.680626)
\figpt 12492:(-0.688942,0.668230)
\figpt 12493:(-0.549342,0.871139)
\figpt 12501:(-0.716856,0.679505)
\figpt 12502:(-0.705435,0.680626)
\figpt 12503:(-0.713227,0.701280)
\figpt 12511:(-0.723883,0.675256)
\figpt 12512:(-0.716856,0.679505)
\figpt 12513:(-0.726412,0.687371)
\figpt 12521:(-0.728629,0.669247)
\figpt 12522:(-0.723883,0.675256)
\figpt 12523:(-0.734466,0.678737)
\figpt 12531:(-0.731244,0.660381)
\figpt 12532:(-0.728629,0.669247)
\figpt 12533:(-0.743564,0.668832)
\figpt 12541:(-0.727527,0.646237)
\figpt 12542:(-0.731244,0.660381)
\figpt 12543:(-0.766356,0.643594)
\figpt 12551:(-0.727527,0.646237)
\figpt 12552:(-0.701713,0.637628)
\figpt 12553:(-0.682635,0.737846)
\figpt 12561:(-0.745179,0.580881)
\figpt 12562:(-0.696069,0.589564)
\figpt 12563:(-0.737846,0.682635)
\figpt 12571:(-0.696069,0.589564)
\figpt 12572:(-0.701713,0.637628)
\figpt 12573:(-0.807083,0.600890)
\figpt 12581:(-0.727527,0.646237)
\figpt 12582:(-0.701713,0.637628)
\figpt 12583:(-0.682635,0.737846)
\figpt 12591:(-0.743122,0.641450)
\figpt 12592:(-0.727527,0.646237)
\figpt 12593:(-0.743237,0.669621)
\figpt 12601:(-0.752810,0.633182)
\figpt 12602:(-0.743122,0.641450)
\figpt 12603:(-0.759479,0.650805)
\figpt 12611:(-0.759035,0.621914)
\figpt 12612:(-0.752810,0.633182)
\figpt 12613:(-0.771706,0.636267)
\figpt 12621:(-0.760488,0.605121)
\figpt 12622:(-0.759035,0.621914)
\figpt 12623:(-0.788322,0.615988)
\figpt 12631:(-0.745179,0.580881)
\figpt 12632:(-0.760488,0.605121)
\figpt 12633:(-0.860942,0.524723)
\figpt 12641:(-0.773982,0.558922)
\figpt 12642:(-0.745179,0.580881)
\figpt 12643:(-0.792284,0.612800)
\figpt 12651:(-0.745179,0.580881)
\figpt 12652:(-0.760488,0.605121)
\figpt 12653:(-0.860942,0.524723)
\figpt 12661:(-0.775871,0.605857)
\figpt 12662:(-0.760488,0.605121)
\figpt 12663:(-0.766356,0.643594)
\figpt 12671:(-0.784624,0.601272)
\figpt 12672:(-0.775871,0.605857)
\figpt 12673:(-0.787220,0.616875)
\figpt 12681:(-0.790032,0.594975)
\figpt 12682:(-0.784624,0.601272)
\figpt 12683:(-0.795929,0.605511)
\figpt 12691:(-0.793119,0.586496)
\figpt 12692:(-0.790032,0.594975)
\figpt 12693:(-0.803725,0.595158)
\figpt 12701:(-0.791758,0.573780)
\figpt 12702:(-0.793119,0.586496)
\figpt 12703:(-0.816757,0.577535)
\figpt 12711:(-0.773982,0.558922)
\figpt 12712:(-0.791758,0.573780)
\figpt 12713:(-1.098684,0.188504)
\figpt 12721:(-0.791165,0.529838)
\figpt 12722:(-0.773982,0.558922)
\figpt 12723:(-0.824013,0.568862)
\figpt 12731:(-0.773982,0.558922)
\figpt 12732:(-0.791758,0.573780)
\figpt 12733:(-1.098684,0.188504)
\figpt 12741:(-0.804196,0.572069)
\figpt 12742:(-0.791758,0.573780)
\figpt 12743:(-0.801506,0.598580)
\figpt 12751:(-0.811175,0.567131)
\figpt 12752:(-0.804196,0.572069)
\figpt 12753:(-0.814883,0.579775)
\figpt 12761:(-0.815410,0.560810)
\figpt 12762:(-0.811175,0.567131)
\figpt 12763:(-0.821901,0.569737)
\figpt 12771:(-0.817326,0.552261)
\figpt 12772:(-0.815410,0.560810)
\figpt 12773:(-0.829029,0.559374)
\figpt 12781:(-0.813699,0.539571)
\figpt 12782:(-0.817326,0.552261)
\figpt 12783:(-0.843533,0.537907)
\figpt 12791:(-0.813699,0.539571)
\figpt 12792:(-0.791165,0.529838)
\figpt 12793:(-0.721675,0.721675)
\figpt 12801:(-0.796186,0.489833)
\figpt 12802:(-0.791165,0.529838)
\figpt 12803:(-0.858126,0.517925)
\figpt 12811:(-0.813699,0.539571)
\figpt 12812:(-0.791165,0.529838)
\figpt 12813:(-0.721675,0.721675)
\figpt 12821:(-0.826880,0.535341)
\figpt 12822:(-0.813699,0.539571)
\figpt 12823:(-0.827967,0.561382)
\figpt 12831:(-0.834249,0.528480)
\figpt 12832:(-0.826880,0.535341)
\figpt 12833:(-0.840287,0.542353)
\figpt 12841:(-0.838497,0.519953)
\figpt 12842:(-0.834249,0.528480)
\figpt 12843:(-0.848080,0.530050)
\figpt 12851:(-0.839358,0.508320)
\figpt 12852:(-0.838497,0.519953)
\figpt 12853:(-0.857114,0.515482)
\figpt 12861:(-0.830602,0.491806)
\figpt 12862:(-0.839358,0.508320)
\figpt 12863:(-0.881337,0.475485)
\figpt 12871:(-0.830602,0.491806)
\figpt 12872:(-0.796186,0.489833)
\figpt 12873:(-0.807083,0.600890)


==> fig1-b.tex <==
%\input{/Users/Moriceau/Documents/fig4tex.tex}
\newbox\figBoxD
\newbox\figBoxE
\newbox\figBoxF
\newbox\figBoxG
\def\RayonBulle{0.09}
% 1. Definition of characteristic points
\figinit{1cm}
\figpt 0:(0,0)

\input{fig1-0pt.tex}

\figpt 4:(-0.476118,-0.45531)
\figpt 5:(0,-0.53531)
\figpt 6:(0.476118,-0.45531)
\figpt 7:(0.536118,-0.000588)
%\figpt 8:(0.35,0.4665625)
\figpt 8:(0,0.57531)
\figpt 14:(0,0)
\figpt 15:(1,0)
\figpt 16:(0.5,0)
\figpt 17:(1.2,-1.2)
\figpt 18:(-0.2,-1.2)
% 2. Creation of the graphical file
\psbeginfig{}

\input{fig1-0dr.tex}

\pscirc 0 (0.986625)
\psset(fillmode=yes)
\pscirc 4(\RayonBulle)
\pscirc 5(\RayonBulle)
\pscirc 6(\RayonBulle)
\pscirc 7(\RayonBulle)
\pscirc 8(\RayonBulle)
\psendfig
% 3. Writing text on the figure
\figvisu{\figBoxA}{}{}
% 2. Creation of the graphical file
\psbeginfig{}

\input{fig1-0dr.tex}

\pscirc 0 (0.986625)
\psset(fillmode=yes)
\figpt 5:(0,-0.59531)
\figpt 6:(0.406118,-0.40531)
\pscirc 5(\RayonBulle)
\pscirc 6(\RayonBulle)
%\pscirc 7(\RayonBulle)
\psendfig
% 3. Writing text on the figure
\figvisu{\figBoxB}{}{}
% 2. Creation of the graphical file
\psbeginfig{}

\input{fig1-0dr.tex}

\pscirc 0 (0.986625)
\psset(fillmode=yes)
\pscirc 6(\RayonBulle)
\psendfig
% 3. Writing text on the figure
\figvisu{\figBoxC}{}{}
% 2. Creation of the graphical file
\psbeginfig{}

\input{fig1-0dr.tex}

\pscirc 0 (0.986625)
\psendfig
% 3. Writing text on the figure
\figvisu{\figBoxD}{}{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%        arrows
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 2. Creation of the graphical file
\psbeginfig{}
\psarrow [14,15]
\psendfig
% 3. Writing text on the figure 
\figvisu{\figBoxE}{}{\figwriten 16:$\tau$(0.2) \figwriten 17:$\ $(0.2)  \figwriten 18:$\ $(0.2)}
% 2. Creation of the graphical file
\psbeginfig{}
\psarrow [14,15]
\psendfig
% 3. Writing text on the figure 
\figvisu{\figBoxF}{}{\figwriten 16:$\tau$(0.2) \figwriten 17:$\ $(0.2)  \figwriten 18:$\ $(0.2)}
% 2. Creation of the graphical file
\psbeginfig{}
\psarrow [14,15]
\psendfig
% 3. Writing text on the figure 
\figvisu{\figBoxG}{}{\figwriten 16:$\tau$(0.2) \figwriten 17:$\ $(0.2)  \figwriten 18:$\ $(0.2)}
%\centerline{\box\figBoxA\box\figBoxE\box\figBoxB\box\figBoxF\box\figBoxC\box\figBoxG\box\figBoxD}
\centerline{\box\figBoxA\box\figBoxE\box\figBoxB\box\figBoxF\box\figBoxD}

